Scalable Multi-domain Trust Infrastructures for Segmented Networks

Within a trust infrastructure, a private key is often used to digitally sign a transaction, which can be verified with an associated public key. Using PKI (Public Key Infrastructure), a trusted entity can produce a digital signature, verifying the authenticity of the public key. However, what happens when external entities are not trusted to verify the public key or in cases where there is no Internet connection within an isolated or autonomously acting collection of devices? For this, a trusted entity can be elected to generate a key pair and then split the private key amongst trusted devices. Each node can then sign part of the transaction using their split of the shared secret. The aggregated signature can then define agreement on a consensus within the infrastructure. Unfortunately, this process has two significant problems. The first is when no trusted node can act as a dealer of the shares. The second is the difficulty of scaling the digital signature scheme. This paper outlines a method of creating a leaderless approach to defining trust domains to overcome weaknesses in the scaling of the elliptic curve digital signature algorithm. Instead, it proposes the usage of the Edwards curve digital signature algorithm for the definition of multiple trust zones. The paper shows that the computational overhead of the distributed key generation phase increases with the number of nodes in the trust domain but that the distributed signing has a relatively constant computational overhead.

==> coding.tex <==

\definecolor{lightgray}{rgb}{.9,.9,.9}
\definecolor{darkgray}{rgb}{.4,.4,.4}
\definecolor{purple}{rgb}{0.65, 0.12, 0.82}

\lstdefinelanguage{script}{
  keywords={},
  keywordstyle=\color{blue}\bfseries,
  ndkeywordstyle=\color{darkgray}\bfseries,
  identifierstyle=\color{black},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{red}\ttfamily,
  sensitive=true,
  breaklines=true,
  escapechar=\$
}

%Javascript styling. Source: https://tex.stackexchange.com/a/89576
\lstdefinelanguage{javascript}{
  keywords={do, if, in, for, let, new, try, var, case, else, enum, eval, null, this, true, void, with, await, break, catch, class, const, false, super, throw, while, yield, delete, export, import, public, return, static, switch, typeof, default, extends, finally, package, private, continue, debugger, function, arguments, interface, protected, implements, instanceof},
  keywordstyle=\color{blue}\bfseries,
  ndkeywords={class, export, boolean, throw, implements, import, this},
  ndkeywordstyle=\color{darkgray}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  commentstyle=\color{purple}\ttfamily,
  stringstyle=\color{red}\ttfamily,
  morestring=[b]',
  morestring=[b]",
  breaklines=true,
  escapechar=\$
}
\lstdefinelanguage{json}{
  keywords={type, data, blockSizes},
  keywordstyle=\color{purple}\bfseries,
  identifierstyle=\color{black},
  sensitive=false,
  comment=[l]{//},
  morecomment=[s]{/*}{*/},
  stringstyle=\color{red}\ttfamily,
  morestring=[b]',
  morestring=[b]",
  breaklines=true,
}

\lstset{ %Note: remove this command if we want to get rid of grey boxes in code listings. 
   language=JavaScript,
   backgroundcolor=\color{lightgray},
   extendedchars=true,
   basicstyle=\footnotesize\ttfamily,
   showstringspaces=false,
   showspaces=false,
   numbers=left,
   numberstyle=\footnotesize,
   numbersep=9pt,
   tabsize=2,
   breaklines=true,
   showtabs=false,
   captionpos=b
}


==> elsarticle.tex <==
%%
%% This is file `elsarticle.cls',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% elsarticle.dtx  (with options: `class')
%% 
%% Copyright 2007-2019 Elsevier Ltd
%% 
%% This file is part of the 'Elsarticle Bundle'.
%% -------------------------------------------
%% 
%% It may be distributed under the conditions of the LaTeX Project Public
%% License, either version 1.2 of this license or (at your option) any
%% later version.  The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX
%% version 1999/12/01 or later.
%% 
%% The list of all files belonging to the 'Elsarticle Bundle' is
%% given in the file `manifest.txt'.
%% 
%%
%%
%%
 \def\RCSfile{elsarticle}%
 \def\RCSversion{3.1}%
 \def\RCSdate{2019/01/14}%
 \def\@shortjnl{\relax}
 \def\@journal{Elsevier Ltd}
 \def\@company{Elsevier Ltd}
 \def\@issn{000-0000}
 \def\@shortjid{elsarticle}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{\@shortjid}[\RCSdate, \RCSversion: \@journal]
\def\ABD{\AtBeginDocument}
\newif\ifpreprint \preprintfalse
\newif\ifnonatbib \nonatbibfalse
\newif\iflongmktitle \longmktitlefalse
\newif\ifnopreprintline \nopreprintlinefalse
\newif\ifdoubleblind \doubleblindfalse

\def\@blstr{1}
\newdimen\@bls
\@bls=\baselineskip

\def\@finalWarning{%
  *****************************************************\MessageBreak
   This document is typeset in the CRC style which\MessageBreak
   is not suitable for submission.\MessageBreak
   \MessageBreak
   Please typeset again using 'preprint' option\MessageBreak
   for creating PDF suitable for submission.\MessageBreak
  ******************************************************\MessageBreak
}

\DeclareOption{preprint}{\global\preprinttrue
  \gdef\@blstr{1}\xdef\jtype{0}%
   \AtBeginDocument{\@twosidefalse\@mparswitchfalse}}
\DeclareOption{nopreprintline}{\global\nopreprintlinetrue}
\DeclareOption{final}{\gdef\@blstr{1}\global\preprintfalse}
\DeclareOption{review}{\global\preprinttrue\gdef\@blstr{1.5}}
\DeclareOption{authoryear}{\xdef\@biboptions{round,authoryear}}
\DeclareOption{number}{\xdef\@biboptions{numbers}}
\DeclareOption{numbers}{\xdef\@biboptions{numbers}}
\DeclareOption{nonatbib}{\global\nonatbibtrue}
\DeclareOption{longtitle}{\global\longmktitletrue}
\DeclareOption{5p}{\xdef\jtype{5}\global\preprintfalse
  \ExecuteOptions{twocolumn}}
  \def\jtype{0}
\DeclareOption{3p}{\xdef\jtype{3}\global\preprintfalse}
\DeclareOption{1p}{\xdef\jtype{1}\global\preprintfalse
  \AtBeginDocument{\@twocolumnfalse}}
\DeclareOption{times}{\IfFileExists{txfonts.sty}%
  {\AtEndOfClass{\RequirePackage{txfonts}%
  \gdef\ttdefault{cmtt}%
   \let\iint\relax
  \let\iiint\relax
  \let\iiiint\relax
  \let\idotsint\relax
  \let\openbox\relax}}{\AtEndOfClass{\RequirePackage{times}}}}

\DeclareOption{endfloat}{\IfFileExists{endfloat.sty}
   {\AtEndOfClass{\RequirePackage[markers]{endfloat}}}{}}
\DeclareOption{endfloats}{\IfFileExists{endfloat.sty}
   {\AtEndOfClass{\RequirePackage[markers]{endfloat}}}{}}
\DeclareOption{numafflabel}
   {\AtBeginDocument{\def\theaffn{\arabic{affn}}}} %*%
\DeclareOption{lefttitle}
   {\AtBeginDocument{\def\elsarticletitlealign{flushleft}}} %*%
\DeclareOption{centertitle}
   {\AtBeginDocument{\def\elsarticletitlealign{center}}} %*%
\DeclareOption{reversenotenum}
   {\AtBeginDocument{\def\theaffn{\arabic{affn}}
    \def\thefnote{\alph{fnote}}}}
\DeclareOption{doubleblind}{\doubleblindtrue}

\ExecuteOptions{a4paper,10pt,oneside,onecolumn,number,preprint,centertitle}
\DeclareOption*{\PassOptionsToClass{\CurrentOption}{article}}
\ProcessOptions
\LoadClass{article}
\RequirePackage{graphicx}
\let\comma\@empty
\let\tnotesep\@empty
\let\@title\@empty

\def\useelstitle{}

\def\title#1{\g@addto@macro\@title{#1%
       \global\let\tnoteref\@gobble}%
       \g@addto@macro\useelstitle{#1}}

\def\elsLabel#1{\@bsphack\protected@write\@auxout{}%
         {\string\Newlabel{#1}{\@currentlabel}}\@esphack}
\def\Newlabel#1#2{\expandafter\xdef\csname X@#1\endcsname{#2}}

\def\elsRef#1{\@ifundefined{X@#1}{0}{\csname X@#1\endcsname}}

\let\@tnotemark\@empty

\ifdoubleblind
  \def\tnotemark[#1]{}
\else
  \def\tnotemark[#1]{\@for\mytmark:=#1\do{%
        \expandafter\ifcase\elsRef{\mytmark}\or$^{\star}$\or
       $^{,\star\star}$\fi
    }%
}
\fi

\def\tnoteref#1{\tnotemark[{#1}]}
\let\@tnotes\@empty
\newcounter{tnote}
\def\tnotetext[#1]#2{\g@addto@macro\@tnotes{%
  \stepcounter{tnote}\elsLabel{#1}%
    \def\thefootnote{\ifcase\c@tnote\or$\star$\or$\star\star$\fi}%
    \footnotetext{#2}}}

\let\@nonumnotes\@empty
\def\nonumnote#1{\g@addto@macro\@nonumnotes{%
     \let\thefootnote\relax\footnotetext{#1}}}

\newcounter{fnote}
\def\thefnote{\arabic{fnote}}
\def\fnmark[#1]{\let\comma\@empty
    \def\@fnmark{\@for\@@fnmark:=#1\do{%
    \edef\fnotenum{\@ifundefined{X@\@@fnmark}{1}{\elsRef{\@@fnmark}}}%
  \unskip\comma\fnotenum\let\comma,}}%
}

\def\fnref#1{\fnmark[#1]}

\let\@fnotes\@empty\let\@fnmark\@empty
\def\fntext[#1]#2{\g@addto@macro\@fnotes{%
   \refstepcounter{fnote}\elsLabel{#1}%
   \def\thefootnote{\c@fnote}%
   \global\setcounter{footnote}{\c@fnote}%
   \footnotetext{#2}}}

\def\cormark[#1]{\edef\cnotenum{\elsRef{#1}}%
    \unskip\textsuperscript{\sep\ifcase\cnotenum\or
       $\ast$\or$\ast\ast$\fi\hspace{-1pt}}\let\sep=,}

\let\@cormark\@empty
\let\@cornotes\@empty
\newcounter{cnote}
\def\cortext[#1]#2{\g@addto@macro\@cornotes{%
    \refstepcounter{cnote}\elsLabel{#1}%
    \def\thefootnote{\ifcase\thecnote\or$\ast$\or
    $\ast\ast$\fi}%
    \footnotetext{#2}}}

\let\@corref\@empty
\def\corref#1{\edef\cnotenum{\elsRef{#1}}%
    \edef\@corref{\ifcase\cnotenum\or
         $\ast$\or$\ast\ast$\fi\hskip-1pt}}

\def\resetTitleCounters{\c@cnote=0
   \c@fnote=0 \c@tnote=0 \c@footnote=0}

\let\eadsep\@empty
\def\@elseads{}
\let\@elsuads\@empty
\let\@cormark\@empty
\def\hashchar{\expandafter\@gobble\string\~}
\def\underscorechar{\expandafter\@gobble\string\_}
\def\lbracechar{\expandafter\@gobble\string\{}
\def\rbracechar{\expandafter\@gobble\string\}}

\gdef\ead{\@ifnextchar[{\@uad}{\@ead}}
\gdef\@ead#1{\bgroup
   \def\_{\underscorechar}%
   \def\{{\lbracechar}%
   \def~{\hashchar}%
   \def\}{\rbracechar}%
   \edef\tmp{\the\@eadauthor}%
   \immediate\write\@auxout{\string\emailauthor
     {#1}{\expandafter\strip@prefix\meaning\tmp}}%
   \egroup
}
\newcounter{ead}
\gdef\emailauthor#1#2{\stepcounter{ead}%
     \g@addto@macro\@elseads{\raggedright%
      \let\corref\@gobble\def\@@tmp{#1}%
      \eadsep{\ttfamily\expandafter\strip@prefix\meaning\@@tmp}
      (#2)\def\eadsep{\unskip,\space}}%
}
\gdef\@uad[#1]#2{\bgroup
   \def~{\hashchar}%
   \def\_{\underscorechar}%
   \def~{\hashchar}%
   \def\}{\rbracechar}%
   \edef\tmp{\the\@eadauthor}
   \immediate\write\@auxout{\string\urlauthor
     {#2}{\expandafter\strip@prefix\meaning\tmp}}%
  \egroup
}
\gdef\urlauthor#1#2{\g@addto@macro\@elsuads{\let\corref\@gobble%
     \def\@@tmp{#1}\raggedright\eadsep
     {\ttfamily\expandafter\strip@prefix\meaning\@@tmp}\space(#2)%
     \def\eadsep{\unskip,\space}}%
}

\def\elsauthors{}
\def\useauthors{}

\def\pprinttitle{}
\let\authorsep\@empty
\let\sep\@empty
\newcounter{author}
\def\author{\@ifnextchar[{\@@author}{\@author}}

\newtoks\@eadauthor
\def\@@author[#1]#2{\g@addto@macro\elsauthors{%
    \def\baselinestretch{1}%
    \authorsep#2\unskip\textsuperscript{%#1%
      \@for\@@affmark:=#1\do{%
       \edef\affnum{\@ifundefined{X@\@@affmark}{1}{\elsRef{\@@affmark}}}%
     \unskip\sep\affnum\let\sep=,}%
      \ifx\@fnmark\@empty\else\unskip\sep\@fnmark\let\sep=,\fi
      \ifx\@corref\@empty\else\unskip\sep\@corref\let\sep=,\fi
      }%
    \def\authorsep{\unskip,\space}%
    \global\let\sep\@empty\global\let\@corref\@empty
    \global\let\@fnmark\@empty}%
    \@eadauthor={#2}%
    \g@addto@macro\useauthors{#2; }%
}

\def\@author#1{\g@addto@macro\elsauthors{\normalsize%
    \def\baselinestretch{1}%
    \upshape\authorsep#1\unskip\textsuperscript{%
      \ifx\@fnmark\@empty\else\unskip\sep\@fnmark\let\sep=,\fi
      \ifx\@corref\@empty\else\unskip\sep\@corref\let\sep=,\fi
      }%
    \def\authorsep{\unskip,\space}%
    \global\let\@fnmark\@empty
    \global\let\@corref\@empty    \global\let\sep\@empty}%
    \@eadauthor={#1}%
    \g@addto@macro\useauthors{#1; }%
}

\AtBeginDocument{%
  \@ifpackageloaded{hyperref}{%
    \expandafter\gdef\csname Hy@title\endcsname{\useelstitle}%
    \expandafter\gdef\csname Hy@author\endcsname{\useauthors}%
   }{}
}

\def\elsaddress{}
\def\addsep{\par\vskip6pt}
\def\address{\@ifnextchar[{\@@address}{\@address}}

\def\@alph#1{%
  \ifcase#1\or a\or b\or c\or d\or e\or f\or g\or h\or i\or j\or k\or
  l\or m\or n\or o\or p\or q\or r\or s\or t\or u\or v\or w\or x\or
  y\or z%
  \or aa\or ab\or ac\or ad\or ae\or af\or ag\or ah\or ai\or aj\or
  ak\or al\or am\or an\or ao\or ap\or aq\or ar\or as\or at\or au\or
  av\or aw\or ax\or ay\or az%
  \or ba\or bb\or bc\or bd\or be\or bf\or bg\or bh\or bi\or bj\or
  bk\or bl\or bm\or bn\or bo\or bp\or bq\or br\or bs\or bt\or bu\or
  bv\or bw\or bx\or by\or bz%
  \or ca\or cb\or cc\or cd\or ce\or cf\or cg\or ch\or ci\or cj\or
  ck\or cl\or cm\or cn\or co\or cp\or cq\or cr\or cs\or ct\or cu\or
  cv\or cw\or cx\or cy\or cz%
  \or da\or db\or dc\or dd\or de\or df\or dg\or dh\or di\or dj\or
  dk\or dl\or dm\or dn\or do\or dp\or dq\or dr\or ds\or dt\or du\or
  dv\or dw\or dx\or dy\or dz%
  \or ea\or eb\or ec\or ed\or ee\or ef\or eg\or eh\or ei\or ej\or
  ek\or el\or em\or en\or eo\or ep\or eq\or er\or es\or et\or eu\or
  ev\or ew\or ex\or ey\or ez%
  \or fa\or fb\or fc\or fd\or fe\or ff\or fg\or fh\or fi\or fj\or
  fk\or fl\or fm\or fn\or fo\or fp\or fq\or fr\or fs\or ft\or fu\or
  fv\or fw\or fx\or fy\or fz%
  \or ga\or gb\or gc\or gd\or ge\or gf\or gg\or gh\or gi\or gj\or
  gk\or gl\or gm\or gn\or go\or gp\or gq\or gr\or gs\or gt\or gu\or
  gv\or gw\or gx\or gy\or gz%
  \else\@ctrerr\fi}

\newcounter{affn}
\renewcommand\theaffn{\alph{affn}}

\long\def\@@address[#1]#2{\g@addto@macro\elsaddress{%
    \def\baselinestretch{1}%
     \refstepcounter{affn}
     \xdef\@currentlabel{\theaffn}
     \elsLabel{#1}%
    \textsuperscript{\theaffn}#2\par}}

\long\def\@address#1{\g@addto@macro\elsauthors{%
    \def\baselinestretch{1}%
    \addsep\footnotesize\itshape#1\def\addsep{\par\vskip6pt}%
    \def\authorsep{\par\vskip8pt}}}

\newbox\absbox
\let\@elsarticleabstitle\@empty %*%
\def\abstracttitle#1{\gdef\@elsarticleabstitle{#1}} %*%
\abstracttitle{Abstract} %*%
\renewenvironment{abstract}{\global\setbox\absbox=\vbox\bgroup
  \hsize=\textwidth\def\baselinestretch{1}%
  \noindent\unskip\textbf{\@elsarticleabstitle} %*%
 \par\medskip\noindent\unskip\ignorespaces}
 {\egroup}

\newbox\keybox
\let\@elsarticlekwdtitle\@empty %*%
\def\keywordtitle#1{\gdef\@elsarticlekwdtitle{#1}} %*%
\def\keywordtitlesep#1{\gdef\@elsarticlekeywordtitlesep{#1}} %*%
\keywordtitle{Keywords} %*%
\keywordtitlesep{:\ }
\def\keyword{%
  \def\sep{\unskip, }%
 \def\MSC{\@ifnextchar[{\@MSC}{\@MSC[2000]}}
  \def\@MSC[##1]{\par\leavevmode\hbox {\it ##1~MSC:\space}}%
  \def\PACS{\par\leavevmode\hbox {\it PACS:\space}}%
  \def\JEL{\par\leavevmode\hbox {\it JEL:\space}}%
  \global\setbox\keybox=\vbox\bgroup\hsize=\textwidth
  \normalsize\normalfont\def\baselinestretch{1}
  \parskip\z@
  \noindent\textit{\@elsarticlekwdtitle\@elsarticlekeywordtitlesep}
  \raggedright                         % Keywords are not justified.
  \ignorespaces}
\def\endkeyword{\par \egroup}

\newdimen\Columnwidth
\Columnwidth=\columnwidth

\def\printFirstPageNotes{%
  \iflongmktitle
    \let\columnwidth=\textwidth
  \fi
\ifdoubleblind
\else
  \ifx\@tnotes\@empty\else\@tnotes\fi
  \ifx\@nonumnotes\@empty\else\@nonumnotes\fi
  \ifx\@cornotes\@empty\else\@cornotes\fi
  \ifx\@elseads\@empty\relax\else
   \let\thefootnote\relax
   \footnotetext{\ifnum\theead=1\relax
      \textit{Email address:\space}\else
      \textit{Email addresses:\space}\fi
     \@elseads}\fi
  \ifx\@elsuads\@empty\relax\else
   \let\thefootnote\relax
   \footnotetext{\textit{URL:\space}%
     \@elsuads}\fi
\fi
  \ifx\@fnotes\@empty\else\@fnotes\fi
  \iflongmktitle\if@twocolumn
   \let\columnwidth=\Columnwidth\fi\fi
}

%% Pushing text to begin on newpage %*%
\def\newpage@after@title{title}
\def\newpage@after@author{author}
\def\newpage@after@abstract{abstract}
\def\newpageafter#1%
    {\gdef\@elsarticlenewpageafter{#1}}

\long\def\pprintMaketitle{\clearpage
  \iflongmktitle\if@twocolumn\let\columnwidth=\textwidth\fi\fi
  \resetTitleCounters
  \def\baselinestretch{1}%
  \printFirstPageNotes
  \begin{\elsarticletitlealign}%
 \thispagestyle{pprintTitle}%
   \def\baselinestretch{1}%
    \Large\@title\par\vskip18pt%
    \ifx\@elsarticlenewpageafter\newpage@after@title% %*%
      \newpage
    \fi%
    \ifdoubleblind
      \vspace*{2pc}
    \else
      \normalsize\elsauthors\par\vskip10pt
      \footnotesize\itshape\elsaddress\par\vskip36pt
    \fi
    \ifx\@elsarticlenewpageafter\newpage@after@author% %*%
      \newpage
    \fi%
    \hrule\vskip12pt
    \ifvoid\absbox\else\unvbox\absbox\par\vskip10pt\fi
    \ifvoid\keybox\else\unvbox\keybox\par\vskip10pt\fi
    \hrule\vskip12pt
    \ifx\@elsarticlenewpageafter\newpage@after@abstract% %*%
      \newpage
    \fi%
    \end{\elsarticletitlealign}%
    \gdef\thefootnote{\arabic{footnote}}%
  }

\def\printWarning{%
     \mbox{}\par\vfill\par\bgroup
     \fboxsep12pt\fboxrule1pt
     \hspace*{.18\textwidth}
     \fcolorbox{gray50}{gray10}{\box\warnbox}
     \egroup\par\vfill\thispagestyle{empty}
     \setcounter{page}{0}
     \clearpage}

\long\def\finalMaketitle{%
  \resetTitleCounters
  \def\baselinestretch{1}%
   \MaketitleBox
   \thispagestyle{pprintTitle}%
  \gdef\thefootnote{\arabic{footnote}}%
  }

\long\def\MaketitleBox{%
  \resetTitleCounters
  \def\baselinestretch{1}%
  \begin{\elsarticletitlealign}%
   \def\baselinestretch{1}%
    \Large\@title\par\vskip18pt
  \ifdoubleblind
    \vspace*{2pc}
  \else
    \normalsize\elsauthors\par\vskip10pt
    \footnotesize\itshape\elsaddress\par\vskip36pt
  \fi
    \hrule\vskip12pt
    \ifvoid\absbox\else\unvbox\absbox\par\vskip10pt\fi
    \ifvoid\keybox\else\unvbox\keybox\par\vskip10pt\fi
    \hrule\vskip12pt
    \end{\elsarticletitlealign}%
}

\def\FNtext#1{\par\bgroup\footnotesize#1\egroup}
\newdimen\space@left
\def\alarm#1{\typeout{******************************}%
             \typeout{#1}%
             \typeout{******************************}%
}

\def\titlespancalculator#1#2#3#4{%
  % break count
  \@tempcnta=#4\relax%
  % pagebreakcount increment
  \advance\@tempcnta by 1\relax%
  % title page height
  \@tempdima=#1\relax%
  % Page height - title page notes height (only for first break)
  % Page height - textheight (for remaining breaks)
  % Page height - title page notes height
  \@tempdimb=#2\relax%
  % Remaining title page height
  \advance\@tempdima -\the\@tempdimb%
  % Checks if remaining title page
  % height less than textheight
  \ifdim\the\@tempdima>#3\relax%
     \titlespancalculator%
      {\the\@tempdima}{#3}{#3}{\the\@tempcnta}%Break again
  \else%
  % Save break count and exit.
     \xdef\savetitlepagespan{\the\@tempcnta}%
  \fi%
}%

\long\def\myfor#1#2#3{%
  \@tempcnta=#1\relax%
  \ifnum#1<#2\relax%
    \advance\@tempcnta by 1\relax%
    #3%
    \myfor{\the\@tempcnta}{#2}{#3}%
  \fi}

\long\def\getSpaceLeft{%\global\@twocolumnfalse%
   \global\setbox0=\vbox{\hsize=\textwidth\MaketitleBox}%
   \global\setbox1=\vbox{\hsize=\textwidth
    \let\footnotetext\FNtext
    \printFirstPageNotes}%
    \xdef\noteheight{\the\ht1}%
    \xdef\titleheight{\the\ht0}%
    \@tempdima=\vsize
    \advance\@tempdima-\noteheight
    \advance\@tempdima-1\baselineskip
    \xdef\savefpageheight{\the\@tempdima}%
    \setbox2=\vbox{\titlespancalculator{\titleheight}%
       {\savefpageheight}{\textheight}{0}}%
}

  \skip\footins=24pt

\newbox\els@boxa
\newbox\els@boxb

\ifpreprint
  \def\maketitle{\pprintMaketitle}
  \else
   \ifnum\jtype=1
    \def\maketitle{%
      \iflongmktitle\getSpaceLeft
        \ifdim\noteheight>0pt%
    \advance\@tempdima-1.35\baselineskip
        \fi%
       \global\setbox\els@boxa=\vsplit0 to \@tempdima
       \box\els@boxa\par\resetTitleCounters
       \thispagestyle{pprintTitle}%
       \printFirstPageNotes
       \ifnum\savetitlepagespan>1\relax%
       \myfor{2}{\savetitlepagespan}{%
       \global\setbox\els@boxb=\vsplit0 to \textheight%\@tempdima
       \box\els@boxb}
       \else%
       \fi%
       \box0%
      \else
       \finalMaketitle\printFirstPageNotes
      \fi
    \gdef\thefootnote{\arabic{footnote}}}%
  \else
 \ifnum\jtype=5
    \def\maketitle{%
      \iflongmktitle\getSpaceLeft
        \ifdim\noteheight>0pt%
    \advance\@tempdima-1.35\baselineskip
        \fi%
       \global\setbox\els@boxa=\vsplit0 to \@tempdima
       \box\els@boxa\par\resetTitleCounters
       \thispagestyle{pprintTitle}%
       \printFirstPageNotes
       \ifnum\savetitlepagespan>1\relax%
       \myfor{2}{\savetitlepagespan}{%
       \global\setbox\els@boxb=\vsplit0 to \textheight%\@tempdima
       \twocolumn[\box\els@boxb]}
       \else%
       \fi%
       \twocolumn[\box0]%\printFirstPageNotes
      \else
       \twocolumn[\finalMaketitle]\printFirstPageNotes
     \fi
     \gdef\thefootnote{\arabic{footnote}}}
  \else
  \if@twocolumn
    \def\maketitle{%
        \iflongmktitle\getSpaceLeft
          \ifdim\noteheight>0pt%
    \advance\@tempdima-1.35\baselineskip
        \fi%
       \global\setbox\els@boxa=\vsplit0 to \@tempdima
       \box\els@boxa\par\resetTitleCounters
       \thispagestyle{pprintTitle}%
       \printFirstPageNotes
       \ifnum\savetitlepagespan>1\relax%
       \myfor{2}{\savetitlepagespan}{%
       \global\setbox\els@boxb=\vsplit0 to \textheight%\@tempdima
       \twocolumn[\box\els@boxb]}
       \else%
       \fi%
       \twocolumn[\box0]%
      \else
       \twocolumn[\finalMaketitle]\printFirstPageNotes
      \fi
     \gdef\thefootnote{\arabic{footnote}}}%
   \else
    \def\maketitle{%
      \iflongmktitle\getSpaceLeft
        \ifdim\noteheight>0pt%
    \advance\@tempdima-1.35\baselineskip
        \fi%
       \global\setbox\els@boxa=\vsplit0 to \@tempdima
       \box\els@boxa\par\resetTitleCounters
       \thispagestyle{pprintTitle}%
       \printFirstPageNotes
       \ifnum\savetitlepagespan>1\relax%
       \myfor{2}{\savetitlepagespan}{%
       \global\setbox\els@boxb=\vsplit0 to \textheight%\@tempdima
       \box\els@boxb}
       \else%
       \fi%
       \box0%
     \else
       \finalMaketitle\printFirstPageNotes
      \fi
    \gdef\thefootnote{\arabic{footnote}}}%
   \fi
  \fi
 \fi
\fi

\let\@elsarticlemyfooter\@empty
\let\@elsarticlemyfooteralign\@empty
\def\@elsarticlemyfooteralignleft{L}
\def\@elsarticlemyfooteralignright{R}
\def\@elsarticlemyfooteraligncenter{C}

\def\myfooter[#1]#2 %*%
      {\gdef\@elsarticlemyfooteralign{#1}
       \gdef\@elsarticlemyfooter{#2}}

\def\myfooterfont#1{\gdef\@myfooterfont{#1}}
\myfooterfont{\footnotesize\itshape}
\def\ps@pprintTitle{%
     \let\@oddhead\@empty
     \let\@evenhead\@empty
     \def\@oddfoot
       {\hbox to \textwidth%
        {\ifnopreprintline\relax\else
        \@myfooterfont%
         \ifx\@elsarticlemyfooteralign\@elsarticlemyfooteraligncenter%
           \hfil\@elsarticlemyfooter\hfil%
         \else%
         \ifx\@elsarticlemyfooteralign\@elsarticlemyfooteralignleft%
           \@elsarticlemyfooter\hfill{}%
         \else%
         \ifx\@elsarticlemyfooteralign\@elsarticlemyfooteralignright%
           {}\hfill\@elsarticlemyfooter%
         \else%
               Preprint submitted to \ifx\@journal\@empty%
                 Elsevier%
            \else\@journal\fi\hfill\@date\fi%
         \fi%
         \fi%
         \fi%
         }
       }%
     \let\@evenfoot\@oddfoot}
\def\@seccntDot{.}
\def\@seccntformat#1{\csname the#1\endcsname\@seccntDot\hskip 0.5em}

\renewcommand\section{\@startsection {section}{1}{\z@}%
           {18\p@ \@plus 6\p@ \@minus 3\p@}%
           {9\p@ \@plus 6\p@ \@minus 3\p@}%
           {\normalsize\bfseries\boldmath}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
           {12\p@ \@plus 6\p@ \@minus 3\p@}%
           {3\p@ \@plus 6\p@ \@minus 3\p@}%
           {\normalfont\normalsize\itshape}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
           {12\p@ \@plus 6\p@ \@minus 3\p@}%
           {\p@}%
           {\normalfont\normalsize\itshape}}

\def\paragraph{\secdef{\els@aparagraph}{\els@bparagraph}}
\def\els@aparagraph[#1]#2{\elsparagraph[#1]{#2.}}
\def\els@bparagraph#1{\elsparagraph*{#1.}}

\newcommand\elsparagraph{\@startsection{paragraph}{4}{0\z@}%
           {10\p@ \@plus 6\p@ \@minus 3\p@}%
           {-6\p@}%
           {\normalfont\itshape}}
\newdimen\leftMargin
\leftMargin=2em
\newtoks\@enLab  %\newtoks\@enfont
\def\@enQmark{?}
\def\@enLabel#1#2{%
  \edef\@enThe{\noexpand#1{\@enumctr}}%
  \@enLab\expandafter{\the\@enLab\csname the\@enumctr\endcsname}%
  \@enloop}
\def\@enSpace{\afterassignment\@enSp@ce\let\@tempa= }
\def\@enSp@ce{\@enLab\expandafter{\the\@enLab\space}\@enloop}
\def\@enGroup#1{\@enLab\expandafter{\the\@enLab{#1}}\@enloop}
\def\@enOther#1{\@enLab\expandafter{\the\@enLab#1}\@enloop}
\def\@enloop{\futurelet\@entemp\@enloop@}
\def\@enloop@{%
  \ifx A\@entemp         \def\@tempa{\@enLabel\Alph  }\else
  \ifx a\@entemp         \def\@tempa{\@enLabel\alph  }\else
  \ifx i\@entemp         \def\@tempa{\@enLabel\roman }\else
  \ifx I\@entemp         \def\@tempa{\@enLabel\Roman }\else
  \ifx 1\@entemp         \def\@tempa{\@enLabel\arabic}\else
  \ifx \@sptoken\@entemp \let\@tempa\@enSpace         \else
  \ifx \bgroup\@entemp   \let\@tempa\@enGroup         \else
  \ifx \@enum@\@entemp   \let\@tempa\@gobble          \else
                         \let\@tempa\@enOther
             \fi\fi\fi\fi\fi\fi\fi\fi
  \@tempa}
\newlength{\@sep} \newlength{\@@sep}
\setlength{\@sep}{.5\baselineskip plus.2\baselineskip
            minus.2\baselineskip}
\setlength{\@@sep}{.1\baselineskip plus.01\baselineskip
            minus.05\baselineskip}
\providecommand{\sfbc}{\rmfamily\upshape}
\providecommand{\sfn}{\rmfamily\upshape}
\def\@enfont{\ifnum \@enumdepth >1\let\@nxt\sfn \else\let\@nxt\sfbc \fi\@nxt}
\def\enumerate{%
   \ifnum \@enumdepth >3 \@toodeep\else
      \advance\@enumdepth \@ne
      \edef\@enumctr{enum\romannumeral\the\@enumdepth}\fi
   \@ifnextchar[{\@@enum@}{\@enum@}}
\def\@@enum@[#1]{%
  \@enLab{}\let\@enThe\@enQmark
  \@enloop#1\@enum@
  \ifx\@enThe\@enQmark\@warning{The counter will not be printed.%
   ^^J\space\@spaces\@spaces\@spaces The label is: \the\@enLab}\fi
  \expandafter\edef\csname label\@enumctr\endcsname{\the\@enLab}%
  \expandafter\let\csname the\@enumctr\endcsname\@enThe
  \csname c@\@enumctr\endcsname7
  \expandafter\settowidth
            \csname leftmargin\romannumeral\@enumdepth\endcsname
            {\the\@enLab\hskip\labelsep}%
  \@enum@}
\def\@enum@{\list{{\@enfont\csname label\@enumctr\endcsname}}%
           {\usecounter{\@enumctr}\def\makelabel##1{\hss\llap{##1}}%
     \ifnum \@enumdepth>1\setlength{\topsep}{\@@sep}\else
           \setlength{\topsep}{\@sep}\fi
     \ifnum \@enumdepth>1\setlength{\itemsep}{0pt plus1pt minus1pt}%
      \else \setlength{\itemsep}{\@@sep}\fi
     %\setlength\leftmargin{\leftMargin}%%%{1.8em}
     \setlength{\parsep}{0pt plus1pt minus1pt}%
     \setlength{\parskip}{0pt plus1pt minus1pt}
                   }}

\def\endenumerate{\par\ifnum \@enumdepth >1\addvspace{\@@sep}\else
           \addvspace{\@sep}\fi \endlist}

\def\sitem{\@noitemargtrue\@item[\@itemlabel *]}

\def\itemize{\@ifnextchar[{\@Itemize}{\@Itemize[]}}

\def\@Itemize[#1]{\def\next{#1}%
  \ifnum \@itemdepth >\thr@@\@toodeep\else
   \advance\@itemdepth\@ne
  \ifx\next\@empty\else\expandafter\def\csname
   labelitem\romannumeral\the\@itemdepth\endcsname{#1}\fi%
  \edef\@itemitem{labelitem\romannumeral\the\@itemdepth}%
  \expandafter\list\csname\@itemitem\endcsname
  {\def\makelabel##1{\hss\llap{##1}}}%
 \fi}
\def\newdefinition#1{%
  \@ifnextchar[{\@odfn{#1}}{\@ndfn{#1}}}%]
\def\@ndfn#1#2{%
  \@ifnextchar[{\@xndfn{#1}{#2}}{\@yndfn{#1}{#2}}}
\def\@xndfn#1#2[#3]{%
  \expandafter\@ifdefinable\csname #1\endcsname
    {\@definecounter{#1}\@newctr{#1}[#3]%
     \expandafter\xdef\csname the#1\endcsname{%
       \expandafter\noexpand\csname the#3\endcsname \@dfncountersep
          \@dfncounter{#1}}%
     \global\@namedef{#1}{\@dfn{#1}{#2}}%
     \global\@namedef{end#1}{\@enddefinition}}}
\def\@yndfn#1#2{%
  \expandafter\@ifdefinable\csname #1\endcsname
    {\@definecounter{#1}%
     \expandafter\xdef\csname the#1\endcsname{\@dfncounter{#1}}%
     \global\@namedef{#1}{\@dfn{#1}{#2}}%
     \global\@namedef{end#1}{\@enddefinition}}}
\def\@odfn#1[#2]#3{%
  \@ifundefined{c@#2}{\@nocounterr{#2}}%
    {\expandafter\@ifdefinable\csname #1\endcsname
    {\global\@namedef{the#1}{\@nameuse{the#2}}
  \global\@namedef{#1}{\@dfn{#2}{#3}}%
  \global\@namedef{end#1}{\@enddefinition}}}}
\def\@dfn#1#2{%
  \refstepcounter{#1}%
  \@ifnextchar[{\@ydfn{#1}{#2}}{\@xdfn{#1}{#2}}}
\def\@xdfn#1#2{%
  \@begindefinition{#2}{\csname the#1\endcsname}\ignorespaces}
\def\@ydfn#1#2[#3]{%
  \@opargbegindefinition{#2}{\csname the#1\endcsname}{#3}\ignorespaces}
\def\@dfncounter#1{\noexpand\arabic{#1}}
\def\@dfncountersep{.}
\def\@begindefinition#1#2{\trivlist
   \item[\hskip\labelsep{\bfseries #1\ #2.}]\upshape}
\def\@opargbegindefinition#1#2#3{\trivlist
      \item[\hskip\labelsep{\bfseries #1\ #2\ (#3).}]\upshape}
\def\@enddefinition{\endtrivlist}

\def\@begintheorem#1#2{\trivlist
  \let\baselinestretch\@blstr
   \item[\hskip \labelsep{\bfseries #1\ #2.}]\itshape}
\def\@opargbegintheorem#1#2#3{\trivlist
  \let\baselinestretch\@blstr
      \item[\hskip \labelsep{\bfseries #1\ #2\ (#3).}]\itshape}

\def\newproof#1{%
  \@ifnextchar[{\@oprf{#1}}{\@nprf{#1}}}
\def\@nprf#1#2{%
  \@ifnextchar[{\@xnprf{#1}{#2}}{\@ynprf{#1}{#2}}}
\def\@xnprf#1#2[#3]{%
  \expandafter\@ifdefinable\csname #1\endcsname
    {\@definecounter{#1}\@newctr{#1}[#3]%
     \expandafter\xdef\csname the#1\endcsname{%
       \expandafter\noexpand\csname the#3\endcsname \@prfcountersep
          \@prfcounter{#1}}%
     \global\@namedef{#1}{\@prf{#1}{#2}}%
     \global\@namedef{end#1}{\@endproof}}}
\def\@ynprf#1#2{%
  \expandafter\@ifdefinable\csname #1\endcsname
    {\@definecounter{#1}%
     \expandafter\xdef\csname the#1\endcsname{\@prfcounter{#1}}%
     \global\@namedef{#1}{\@prf{#1}{#2}}%
     \global\@namedef{end#1}{\@endproof}}}
\def\@oprf#1[#2]#3{%
  \@ifundefined{c@#2}{\@nocounterr{#2}}%
    {\expandafter\@ifdefinable\csname #1\endcsname
    {\global\@namedef{the#1}{\@nameuse{the#2}}%
  \global\@namedef{#1}{\@prf{#2}{#3}}%
  \global\@namedef{end#1}{\@endproof}}}}
\def\@prf#1#2{%
  \refstepcounter{#1}%
  \@ifnextchar[{\@yprf{#1}{#2}}{\@xprf{#1}{#2}}}
\def\@xprf#1#2{%
  \@beginproof{#2}{\csname the#1\endcsname}\ignorespaces}
\def\@yprf#1#2[#3]{%
  \@opargbeginproof{#2}{\csname the#1\endcsname}{#3}\ignorespaces}
\def\@prfcounter#1{\noexpand\arabic{#1}}
\def\@prfcountersep{.}
\def\@beginproof#1#2{\trivlist\let\baselinestretch\@blstr
   \item[\hskip \labelsep{\scshape #1.}]\rmfamily}
\def\@opargbeginproof#1#2#3{\trivlist\let\baselinestretch\@blstr
      \item[\hskip \labelsep{\scshape #1\ (#3).}]\rmfamily}
\def\@endproof{\endtrivlist}
\newcommand*{\qed}{\hbox{}\hfill$\Box$}

\@ifundefined{@biboptions}{\xdef\@biboptions{numbers}}{}
\InputIfFileExists{\jobname.spl}{}{}
\ifnonatbib\relax\else
  \RequirePackage[\@biboptions]{natbib}
\fi
\newwrite\splwrite
\immediate\openout\splwrite=\jobname.spl
\def\biboptions#1{\def\next{#1}\immediate\write\splwrite{%
   \string\g@addto@macro\string\@biboptions{%
    ,\expandafter\strip@prefix\meaning\next}}}

\let\baselinestretch=\@blstr
\ifnum\jtype=1
 \RequirePackage{geometry}
 \geometry{twoside,
  paperwidth=210mm,
  paperheight=297mm,
  textheight=562pt,
  textwidth=384pt,
  centering,
  headheight=50pt,
  headsep=12pt,
  footskip=12pt,
  footnotesep=24pt plus 2pt minus 12pt,
 }
 \global\let\bibfont=\footnotesize
 \global\bibsep=0pt
 \if@twocolumn\global\@twocolumnfalse\fi
\else\ifnum\jtype=3
 \RequirePackage{geometry}
 \geometry{twoside,
  paperwidth=210mm,
  paperheight=297mm,
  textheight=622pt,
  textwidth=468pt,
  centering,
  headheight=50pt,
  headsep=12pt,
  footskip=18pt,
  footnotesep=24pt plus 2pt minus 12pt,
  columnsep=2pc
 }
 \global\let\bibfont=\footnotesize
 \global\bibsep=0pt
 \if@twocolumn\input{fleqn.clo}\fi
\else\ifnum\jtype=5
 \RequirePackage{geometry}
 \geometry{twoside,
  paperwidth=210mm,
  paperheight=297mm,
  textheight=682pt,
  textwidth=522pt,
  centering,
 headheight=50pt,
  headsep=12pt,
  footskip=18pt,
  footnotesep=24pt plus 2pt minus 12pt,
  columnsep=18pt
 }%
 \global\let\bibfont=\footnotesize
 \global\bibsep=0pt
 \input{fleqn.clo}
 \global\@twocolumntrue
%%
%% End of option '5p'
%%
\fi\fi\fi
\def\journal#1{\gdef\@journal{#1}}
 \let\@journal\@empty
\newenvironment{frontmatter}{}{\maketitle}

\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip\footnotesize
  \sbox\@tempboxa{#1: #2}%
  \ifdim \wd\@tempboxa >\hsize
    #1: #2\par
  \else
    \global \@minipagefalse
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}

\AtBeginDocument{\@ifpackageloaded{hyperref}
  {\def\@linkcolor{blue}
   \def\@anchorcolor{blue}
   \def\@citecolor{blue}
   \def\@filecolor{blue}
   \def\@urlcolor{blue}
   \def\@menucolor{blue}
   \def\@pagecolor{blue}
\begingroup
  \@makeother\`%
  \@makeother\=%
  \edef\x{%
    \edef\noexpand\x{%
      \endgroup
      \noexpand\toks@{%
        \catcode 96=\noexpand\the\catcode`\noexpand\`\relax
        \catcode 61=\noexpand\the\catcode`\noexpand\=\relax
      }%
    }%
    \noexpand\x
  }%
\x
\@makeother\`
\@makeother\=
}{}}
%%
\def\appendixname{Appendix }
\renewcommand\appendix{\par
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \setcounter{equation}{0}
  \gdef\thefigure{\@Alph\c@section.\arabic{figure}}%
  \gdef\thetable{\@Alph\c@section.\arabic{table}}%
  \gdef\thesection{\appendixname~\@Alph\c@section}%
  \@addtoreset{equation}{section}%
  \gdef\theequation{\@Alph\c@section.\arabic{equation}}%
  \addtocontents{toc}{\string\let\string\numberline\string\tmptocnumberline}{}{}
}

%%%% \numberline width calculation for appendix.
\newdimen\appnamewidth
\def\tmptocnumberline#1{%
   \setbox0=\hbox{\appendixname}
   \appnamewidth=\wd0
   \addtolength\appnamewidth{2.5pc}
   \hb@xt@\appnamewidth{#1\hfill}
}

%% Added for work with amsrefs.sty

\@ifpackageloaded{amsrefs}%
  {}
  {%\let\bibsection\relax%
  \AtBeginDocument{\def\cites@b#1#2,#3{%
    \begingroup[%
        \toks@{\InnerCite{#2}#1}%
        \ifx\@empty#3\@xp\@gobble\fi
        \cites@c#3%
}}}
%%
%% Added for avoiding clash with cleveref.sty
\@ifpackageloaded{cleveref}%
 {}
 {\def\tnotetext[#1]#2{\g@addto@macro\@tnotes{%
    \refstepcounter{tnote}%
    \immediate\write\@auxout{\string\Newlabel{#1}{\thetnote}}
    \def\thefootnote{\ifcase\c@tnote\or$\star$\or$\star\star$\fi}%
    \footnotetext{#2}}}
%%%
  \def\fntext[#1]#2{\g@addto@macro\@fnotes{%
    \refstepcounter{fnote}%
    \immediate\write\@auxout{\string\Newlabel{#1}{\thefnote}}
    \def\thefootnote{\thefnote}%
    \global\setcounter{footnote}{\c@fnote}%
    \footnotetext{#2}}}
%%%
  \def\cortext[#1]#2{\g@addto@macro\@cornotes{%
    \refstepcounter{cnote}%
    \immediate\write\@auxout{\string\Newlabel{#1}{\thecnote}}
    \def\thefootnote{\ifcase\c@cnote\or$\ast$\or
    $\ast\ast$\fi}%
    \footnotetext{#2}}}
}

\def\textmarker#1#2{\textcolor{#1}{#2}}%*%
\endinput
%%
%% End of file `elsarticle.cls'.


==> sections/01_introduction.tex <==
\section{Introduction}
Shamir's Secret Sharing (SSS) \cite{shamir1979share} provides a method of integrating distributed trust into a system, while supporting Byzantine resilience. For this we can enhance our trust by distributing a private key across a number of nodes, and then enabling a distributed signing process - this is often known as Distributed Key Generation (DKG). One method of achieving this is to use the Asynchronous Verifiable Secret Sharing and Proactive \cite{cachin2002asynchronous} method, but this has several problems, including:

\begin{enumerate}
\item Dealer has access to all keys as they are the ones generating the keys. These steps ought to be distributed and made more secure.
\item The regeneration of lost shares, triggered by a node going offline or leaving the network, lacks automation, leading to operational inefficiencies. 
\item The absence of a proactive system that affords for downtimes and ensures the deletion of shares from an existing node once the share regeneration is done.
\end{enumerate}



\subsection{Shamir Secret Shares}

With secret sharing, we take a secret value and then share it with others. For example, we might have a share for Bob, Alice, Carol and Dave and then for three of them to come together to bring their shares together. First, we generate a polynomial, and which has a secret value. In the following example, we have a quadratic equation of $f(x)=2x^2 -2x + 5$ (Figure \ref{fig:quad}). The secret could be stored at $f(0)$ (the red line), and where we give Bob their y value for $x=1$ ($f(1)$ — the purple line), Carol the value at $x=2$ ($f(2)$ — the blue line), Dave the value at $x=3$ ($f(3)$ — the green line) and Alice the value at $x=4$ ($f(4)$ — the outer blue line). With the values of their own, they cannot recover $f(0)$, but if we have three of the values, we can recover it.

\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/quad01.png}
\caption{Example quadratic equation)}
\label{fig:quad}
\end{center}
\end{figure}

For an any 3-from-4, we can use a quadratic equation, such as $f(x)=20x^2-2x+10$, and where the value of 10 is the secret. Bob then gets the value of $f(x)$ when $x=1$. This can be defined as $f(1)$. Carol gets $f(2)$, Dave gets $f(3)$ and Alice gets $f(4)$. The secret value is thus $f(0)$. They then each know a point on the quadratic equation, and three of them can bring them back to recover the secret. In this case, we will generate a random polynomial of $ax^2+bx+secret$, and then distribute the shares to Bob, Alice, Carol and Dave.

\subsubsection{Shamir Secret Shares and Kryptology}

We can use the Kryptology library \cite{Kryptology} developed by Coinbase to implement Shamir Secret Shares. In this case, at \cite{asecuritysite_13378}, we will define $t$ for the threshold and $n$ for the number of shares.


\subsection{ECDSA and EdDSA}
A digital signature involves taking a hash of the message, and then using a private key to create a signature. The public key is then used to prove the signature and verify the contents of the message. The two main methods that are used as ECDSA (using the secp256k1 curve) and EdDSA (using the Curve 25519). An overview of these methods are:

\begin{itemize}
\item Ed25519 was proposed in 2011 by Daniel J. Bernstein, Niels Duif, Tanja Lange, Peter Schwabe, and Bo-Yin Yang \cite{bernstein2012high}, while ECDSA was proposed around 2001 by Don Johnson, Alfred Menezes, and Scott Vanstone \cite{johnson2001elliptic}.
\item ECDSA and EdDSA typically have equivalent performance and security levels.
\item ECDSA has a random nonce value created within the signature creation, whereas EdDSA does not. In ECDSA, we need to be careful in making sure that we do not reuse this nonce value and that it is random.
\item EdDSA uses the Schnorr signature method, and which is now out of patent. It supports the aggregation of keys in the signature and also the aggregation of the signature for multiple parties.
\item For improved security, ECDSA supports a 521-bit curve (P521), while EdDSA supports X448.
\item ECDSA signatures change each time based on the nonce used, whereas EdDSA signatures do not change for the same set of keys and the same message.
\item ECDSA is often used to keep compatibility with Bitcoin and Ethereum.
\item ECDSA public keys are (x,y) coordinates and thus have 512 bits (for secp256k1), while Ed25519 uses just the y coordinate value for the point, and thus has 256 bits.
\item It is possible to recover the public key from an ECDSA signature.
\end{itemize}


\subsubsection{ECDSA}
With ECDSA, Alice will sign a message with her private key, and then Bob will use her public key to verify that she signed the message (and that the message has now changed). Alice signs the message with the following:

\begin{itemize}
\item     Create a hash of the message $e=\textrm{HASH}(m)$.
\item     Let $h$ be the $L_{n}$ be the leftmost bits of $e$, $L_{n}$ has a  bit length of the group order $N$.
\item     Create a random number $k$ which is between 1 and $N-1$.
\item     Calculate a point on the curve as $(x_{1},y_{1})=k\times G$.
\item     Calculate $ r=x_{1} \pmod N $. If $r=0$, go back to Step 3.
\item     Calculate $s=k^{-1}(h+rd_{A}) \pmod N$. If $s=0$, go back to Step 3.
\item     The signature is the pair $(r,s)$.
\end{itemize}


Bob will check with:

\begin{itemize}
\item     Create a hash of the message $e=\textrm{HASH}(m)$.
\item     Let $h$ be the $L_{n}$ leftmost bits of $e$.
\item     Calculate $c=s^{-1} \pmod N$
\item     Calculate $u_{1}=h \cdot c \pmod N$ and $u_{2}=r \cdot c \pmod N$.
\item     Calculate the curve point ($x_{1},y_{1})=u_{1}\times G+u_{2}\times Q_{A}$. If $(x_{1},y_{1})=O$ then the signature is invalid.
\item     The signature is valid if $r\equiv x_{1}{\pmod {n}}$, invalid otherwise.
\end{itemize}

\begin{equation}
\begin{aligned}
(x_{1},y_{1}) &=u_{1}\times G+u_{2}\times Q_{A}\\ 
&= h \cdot c \cdot G + r \cdot c \cdot Q_A\\
&= c (hG + rQ_A) = \frac{hG + rQ_A} {k^{-1}(h+rd_A) } \\
&= \frac{hG + rd_A G} {k^{-1}(h+rd_A) } \\
&= \frac{(h + rd_A) G} {k^{-1}(h+rd_A) } =  kG 
\end{aligned}
\end{equation}

Within \cite{asecuritysite_55802}, we take a message and generate a private key and then generate a public key and a message signature. In this, we see that we have a 256-bit private key, and a public key which is a point on the secp256k1 curve. The output is two values: R and S. Once we use the message, the public key points, and the values of R and S, we should be able to determine the validity of the signature.


\subsubsection{EdDSA}
The Edwards-curve Digital Signature Algorithm (EdDSA) is used to create a digital signature using an enhancement of the Schnorr signature with Twisted Edwards curves. Overall it is faster that many other digital signature methods, and is strong for security. One example of EdDSA is Ed25519, and which is based on Curve 25519. It generates a 64-byte signature value of (R,s), and has 32-byte values for the public and the private keys.

With Ed25519, Bob first generates a 256-bit random number for the private key ($priv$) and then create the public key with:

\begin{equation}
pub =  H(priv)[\colon 32] \cdot B
\end{equation}

and where $B$ is the base point on the curve, and and where $H()$ is a hash function (SHA-512). In this case we take the lower 32 bytes of the SHA-512 hash. Normally we just define this as the $y$ co-ordinate of the point. The public key is this 32 bytes long (256 bits). To compute the signature, we generate:

\begin{equation}
r = H_{int}( H(priv)[32\colon] \: || \: M) \pmod l
\end{equation}

and where $H_{int}()$ is a hash function (SHA-512) and converted to an integer value. In this case we take the upper 32 bytes for the calculation. Then $M$ is the byte value of the message. With "||" we append the bytes together. We then convert this to a point on the curve with:

\begin{equation}
R=r \cdot B
\end{equation}

Next, we compute:
\begin{equation}
h=H_{int}(R \: || \: pub \: || \: M) \pmod l
\end{equation}
and:
\begin{equation}
s=H_{int}(priv))[\colon 32]\\
S=(r+h \cdot s) \pmod l
\end{equation}

The signature is then $(R,S$). Bob sends $M$, $R$, $S$ and $pub$ to Alice. Alice then computes:

\begin{equation}
k=H(R \: || \: pub \: || \: M) \pmod l\\
P_1=S \cdot B\\
P_2=R + k \cdot pub
\end{equation}

and if $P_1$ is equal to $P_2$, the signature verifies. This works because:

$P_1=S \cdot B = (r + h \cdot s \pmod l) \cdot B = r \cdot B + h \cdot s \cdot B = R + h \cdot pub = P_2$
Note that $l$ is the order of the curve ($l= 2^{252} + 27742317777372353535851937790883648493$).
The great advantage of using Ed25519 over ECDSA is that we can aggregate signatures and public keys. Within \cite{asecuritysite_24414}, we produce a signature that is 64 bytes long, made up of 32 bytes for the $R$ value, and 32 bytes for the $s$ value. The public key is also 32 bytes long, and the private key is 32 bytes. Overall Ed25519 produces one of the smallest signature sizes and has a small size of the public and private key.



==> sections/02_verifiable_share.tex <==




\section{Verifiable Secret Shares}
Within secret-sharing models, we can have three main categories:

\begin{itemize}
\item Synchronous model. This is implemented in systems that use a global clock to synchonise messages, and where there will be well-defined delays in processing. 
\item Asynchronous model. This is where there is no synchonisation of messages, and where delays can vary depending on workloads. One of the key issues is that it is difficult to differentiate a slow response from a participating party from a corrupt sender who refuses to send back messages. This leads to more complexity in the methods used by asynchonous methods. 
\item Hybrid. This is a mixture of synchonous and asynchronous models, and where there may be a few rounds of synchonization followed by asynchonous operations.
\end{itemize}

In a typical secret sharing method, the dealer defines a polynomial of $p(x)=a_0+a_1x+a_2x^2+...$ and where $a_0$ defines the secret. The dealer then sends out points on the polynomial, such for $x=1$ and where we have the $y$ value of $p(x=1)$. We can also create a commitment from the dealer, so that each participant can check that their share is valid. Within an asynchonous environment, the dealer may not wait around before all the shares have been acknowledged. AVSS supports a participating party in reconstructing its share using a distributed protocol that does not require the dealer to be present. This requires $f+1$ participants.
    
In asynchronous settings in which participants might fail, a dealer can wait for at most $n$ participants to acknowledge receiving a valid share, before it inevitably may walk away. The asynchronous VSS problem requires that if the dealer (or any participant) completes the sharing protocol, then every correct participant can eventually reconstruct its share using  a distributed protocol involving $f + 1$ participants.
    
The Coinbase Kryptology Golang library \cite{Kryptology} supports the Pedersen Verifiable Secret Shares, and which allows players in the secret shares to verify their shares, without revealing the secret. This involves a blinding process to allow the entities who receive the shares to check their validity.


\subsection{Pedersen Verifiable Shamir Shares}

With the Pedersen Verifiable Secret Sharing Scheme (PVSS) \cite{pedersen1991non}, we create a blinding factor (b), and then split this value into coefficients:
\begin{equation} 
g(x)=b+b_1 x+b_2 x^2 ...
\end{equation} \label{eqn}

The dealer (who is distributing the shares), initially privately sends out each share. For Bob:

\begin{equation} 
S_1=(p(1),g(1)) 
\end{equation} 

and for Alice:

\begin{equation} 
S2=(p(2),g(2)) 
\end{equation} 

and where the $p()$ is the secret share and $g()$ will be used to verify the share. The dealer also creates a number of commitments for elliptic curve point additions:

\begin{equation} 
C_1=p(1)+g(1)
\end{equation} 
\begin{equation} 
C_2=p(2)+g(2)
\end{equation} 

and so on. These are then passed to the entities involved. It will not be possible for any other player to reveal the secret share from the commitments, as the blinding factor has been applied. Figure \ref{fig:pvss} outlines the commitments.

\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/pvss.png}
\caption{PVSS)}
\label{fig:pvss}
\end{center}
\end{figure}

Each player receives a share and then checks the commitment against the share elements. If they do not match, the player will tell the other players that they have a complaint against the dealer. They will then reveal their commitment and their share. The dealer will also reveal its commitment. Next, the players will then check who is right against the commitments. If the commitment does not match the share, they will remove the dealer from the game; if not, they will remove the accusing entity from the game.

We can use the Kryptology library developed by Coinbase to implement PVSS. In this case, at \cite{asecuritysite_14012}, we will define $t$ for the threshold and $n$ for the number of shares.


\subsection{Asynchronous Verifiable Secret Sharing (AVSS)}
In 2002, Cachin et. al \cite{cachin2002asynchronous} defined Asynchronous Verifiable Secret Sharing (AVSS) method and which uses bi-variate polynomials. In most secret sharing schemes we have a polynomial with one variable, such as $p(x)=a_0+a_1x+a_2x^2+...$. With Shamir's Secret Shares, we store the secret share at $a_0$, and where we distribute points on the polynomial and then rebuild them back into a polynomial, and which should then reveal the secret. With AVSS we use bi-variate polynomials and which have two variables ($x$ and $y$). Bi-variate polynomials are in the form of $f(x,y)  =a_{00} + a_{10}x + a_{01} y + a_{11} xy +  a_{21} x^2y + +  a_{12} xy^2 + a_{22} x^2y^2 + ... $. In this case, the secret is kept at $a_{00}$. With the Shamir method, we define a threshold ($t$) from a number of shares ($n$), and then aim to recover a polynomial $f(x,y$) and where the secret share is at $f(0,0$).

In AVSS, we start with a bi-variate polynomial ($m \times n$):

\begin{equation}
f(x,y) = \sum_{k=0}^{n-1}\sum_{j=0}^{m-1} a_{jk}x^ky^j
\end{equation}

For $n=3$ and $m=3$, we have:

\begin{equation}
f(x,y)  =a_{00} + a_{10}x + a_{01} y + a_{11} xy +  a_{21} x^2y + +  a_{12} xy^2 + a_{22} x^2y^2
\end{equation}

In a secret sharing system, we aim to find the solution at $p(0,0)$.
We can represent the factors in a matrix form of:

\begin{equation}
    v_{m,n} =
    \begin{pmatrix}
    a_{0,0} & a_{0,1} & \cdots & a_{0,n-1} \\
    a_{1,0} & a_{1,1} & \cdots & a_{1,n-1} \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    a_{m-1,1} & a_{m-1,1} & \cdots & a_{m-1,n-1}
    \end{pmatrix}
\end{equation}

In AVSS, we place the secret at $a_{0,0}$ and random values in the other positions: 

 \begin{equation}
    f_{m,n} =
    \begin{pmatrix}
    s & r_{0,1} & \cdots & r_{0,n-1} \\
    r_{1,0} & r_{1,1} & \cdots & r_{1,n-1} \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    r_{m-1,1} & r_{m-1,1} & \cdots & r_{m-1,n-1}
    \end{pmatrix}
\end{equation}

We then generate a random matrix:

\begin{equation}
    f'_{m,n} =
    \begin{pmatrix}
    v_{0,0} & v_{0,1} & \cdots & v_{0,n-1} \\
    v_{1,0} & v_{1,1} & \cdots & v_{1,n-1} \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    v_{m-1,1} & v_{m-1,1} & \cdots & v_{m-1,n-1}
    \end{pmatrix}
\end{equation}

We then take a base point on the secp256k1 curve ($G$) and then scale with $f_(m,n)$, and then add this to $f'(m,n)$ to another base point ($H$). This then gives a number of secp256k1 points for the commitments from the dealer:

\begin{equation}
    C_{m,n} =
    \begin{pmatrix}
    sG + r_{0,0}H & r_{0,1}G+ r_{0,1}H & \cdots & r_{0,n-1}G + r_{0,n-1}H \\
    r_{1,0}G + r_{1,0}H & r_{1,1}G + r_{1,1}H & \cdots & r_{1,n-1}G + r_{1,n-1}H \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    r_{m-1,1}G + r_{m-1,1}H & r_{m-1,1}G + r_{m-1,1}H & \cdots & r_{m-1,n-1}G + r_{m-1,n-1}H
    \end{pmatrix}
\end{equation}

Each of the nodes $i$ then get:
\begin{align}
C\\
a_i(y) = f(i,y)\\
a_i'(y) = f'(i,y)\\
b_i(x) = f(x,i)\\
b_i'(x) = f'(x,i)\\
\end{align}

Thus Node 1 ($x=1$) gets the polynomial factors of:
\begin{equation}
a_1(y) = sG+ v_{0,0}H, r_{0,1}G + v_{0,1}H, \cdots r_{0,n-1}G + v_{0,n-1}H 
\end{equation}

Thus Node 2 ($x=2$) gets the polynomial factors of:
\begin{equation}
a_2(y) = sG+ v_{0,0}H, r_{0,1}G + v_{0,1}H \times 4,  \cdots  r_{0,n-1}G +  v_{0,n-1}H \times 2^{n-1}
\end{equation}

Thus Node 3 ($x=3$) gets the polynomial factors of:
\begin{equation}
a_3(y) = sG+ v_{0,0}H, r_{0,1}G + v_{0,1}H \times 9,  \cdots  r_{0,n-1}G + v_{0,n-1}H \times 3^{n-1}
\end{equation}

Every node $i$ will receive $C$, the share polynomial of $a_i(y)$ and $a_i'(y)$, and the sub-share polynomials are $b_i(y)$ and $b_i'(y)$ 
Each node can then check their shares against the commitment from the dealer. The sequence is then:

1. The Dealer creates a bi-variate polynomial and puts the secret at $f(0,0)$ and with random values at all the other other places in the matrix:

\begin{verbatim}
f := GenerateRandomBivariatePolynomial(secret, threshold)
\end{verbatim}

2. Create random bitvariate polynomial:

\begin{verbatim}
fprime := GenerateRandomBivariatePolynomial(*RandomBigInt(), threshold)
\end{verbatim}

3. Create commitment matrix, and which is the point assigns the $f$ as scalar values to the $G$ base point, and $fprime$ with the $H$ based point, and then adds these together, to get the form $a_{ij}G + a'_{ij}H$. 

\begin{verbatim}
	C := GetCommitmentMatrix(f, fprime)
\end{verbatim}

These are points on the secp256k1 curve. When a node receives a share, it can then check that the share is valid. In the following, we will take the first share for its validity:
\begin{lstlisting}[language=golang]
sigma := polyEval(EvaluateBivarPolyAtX(f, *big.NewInt(int64(threshold))), 0)
sigmaprime := polyEval(EvaluateBivarPolyAtX(fprime, *big.NewInt(int64(threshold))), 0)
fmt.Printf("\n1st share: Sigma=%s, Sigma_p=%s", sigma, sigmaprime)
rtn := AVSSVerifyShare(C, *big.NewInt(int64(threshold)), *sigma, *sigmaprime)
fmt.Printf("\nVerified share: %v ", rtn)
\end{lstlisting}

On completion of this process, each node has a polynomial share to a master polynomial, and where the master is a sum of all the polynomials given to the nodes.

Proactive Secret Sharing (PSS) is used to migrate keys. With this, the system creates polynomial shares of the existing shares and these are then added to the master polynomial.

A demonstrator is defined at \cite{asecuritysite_33918}.

\subsection{Feldman Verifiable Secret Sharing Scheme}
With secret sharing, we take a secret value and then share it with others. For example, we might have a share for Bob, Alice, Carol and Dave and then for three of them to come together to bring their shares together. For an \emph{any 3-from-4} scheme, we can use a quadratic equation, such as $f(x)=20 x - 2 x + 10$, and where the value of 10 is the secret. Bob then gets the value of $f(x)$ when $x=0$. This can be defined as $f(1)$. Carol gets $f(2)$, Dave gets $f(3)$ and Alice gets $f(4)$. The secret value is thus $f(0)$. They then each know a point on the quadratic equation, and three of them can bring them back to recover the secret. In this case, we will generate a random polynomial of $a x^2 + b x + secret$, and then distribute the shares to Bob, Alice, Carol and Dave. Finally, we will recover the secret from three of these shares (Bob, Carol and Dave). In 1987, Paul Feldman published a paper which proposed using the homomorphic encryption properties of exponation to create verifiable shares, and where a dealer creates the secret shares and distributes them to the players. They also publish an overall commitment to the shares and where each player can check that their share is valid, without revealing any information about the secret share, and any other player's secret share.

How do we cope with a dishonest dealer? How do the entities who receive the shares verify that they are valid? Well, one of the best ways was developed by Paul Feldman and is defined as a Verifiable Secret Sharing (VSS) method \cite{feldman1987practical}. The great advantage of this method is that we can use any homomorphic encryption approach.
For this we create a group $G$ using a prime number $p$ and a generator $g$ (typically a value of $g=2$ or $g=5$ is used). Overall the dealer creates a secret ($s$) and a random polynomial ($f(x)$), and where $f(0)=s$. For example:

\begin{equation*}
f(x) = 5 + 2x + 4x^2
\end{equation*}

in this case, the secret is 5, and $f(1)$ is 7, f(2) is 25, $f(3)$ is 47 and $f(4)$ is 77. For any 3-from-4 we can distribute points (1,7), (2,25), (3,47) and (4,77) to each of the players. Each player gets one point on the curve. With three points the players will then be able to discover the quadradic equation, and reveal the secret. With just one or two points, it will be impossible to do this. This is at the core of the Shamir method. But how do the players know they are getting a valid share of the secret, without revealing the secret? Well we have:
\begin{equation*}
f(x) = s + a_1 x + a_2 x^2 + ...
\end{equation*}We can then create commitments as:

\begin{itemize}
\item $c_0 = g^s \pmod p$
\item $c_1 = g^{a_1} \pmod p$
\item $c_2 = g^{a_2} \pmod p$
\end{itemize}

It is then possible for every player $i$ to verify that:
\begin{equation*}
v = f(i) \pmod p
\end{equation*}

and check:
\begin{equation*}
\displaystyle g^{v}=c_{0}c_{1}^{i}c_{2}^{i^{2}}\cdots c_{t}^{i^{t}}=\prod _{j=0}^{t}c_{j}^{i^{j}}=\prod _{j=0}^{t}g^{a_{j}i^{j}}=g^{\sum _{j=0}^{t}a_{j}i^{j}}=g^{f(i)}
\end{equation*}

This operation is also done using $\pmod p$.

We can use the Kryptology library developed by Coinbase to implement Felman Verifiable Shamir Secret (VSS) Shares. In this case, at \cite{asecuritysite_18994}, we will define $t$ for the threshold and $n$ for the number of shares.






==> sections/03_proactive.tex <==
\section{Proactive sharing}

Eldefrawy et al \cite{eldefrawy2021regenerating} define two core contributions. One is a Proactive Secret Sharing (PSS) that supports randomization and for the shares to be repaired of shares given information from other shares. They also use Regenerating Codes (RC) for disk storage and which use Reed Solomon error correcting (or erasure handling) codes. This supports distributed storage across cloud-based storage areas. In the paper the authors show that a PSS method can be converted into RC, and vice-versa. These are defined as a Generalized-decoding Regenerating Code (GRC).

\subsection{Local repairing}
Fu et al \cite{fu2017introduction} defined the concept of repairing locality as a key feature of distributed storage. This relates to the repair of a damaged or lost share, and where perfect sharing cannot be achieved with the integration of repairing for most of the existing secret share methods. The simplest way to regenerate corrupted shares is to regenerate it, but this requires at least the number of threshold nodes to come together to generate it. To overcome this issue, we can implement:

\begin{itemize}
\item Enrollment protocols.  Enrollment protocols \cite{dong2005non} are used to repair a secret share by only using coded versions of other shares, so the shares and the secret themselves are not revealed. However, these enrollment protocols can only be applied to speciﬁc SS schemes so the generality is lost. With social sharings \cite{nojoumian2010unconditionally}. 
\item Regeneration codes. In 2010, Dimakis \cite{dimakis2010network} first outlined the concept of using erase codes in order to fragment data across nodes. With this, some fragments on nodes will require to be replaced over time. We then use  regenerating codes to allow new nodes to receive data from surviving nodes, and which heal the storage infrastructure. 
\end{itemize}

Within repairable schemes, we define the conception of requiring $d$ participants to get together to repair a share. This is defined as the repairing degree. Guang et al \cite{guang2014repairable} defined their GLF scheme. This uses the linearized polynomials and regenerating codes that are used in distributed storage systems. They also apply  minimum bandwidth regenerating (MBR) codes to optimize the balance of optimal repairing and associated information rates. Rawat et al defined two operating points: Minimum storage multi-node regeneration (MSMR); and minimum bandwidth multi-node regeneration (MBMR) \cite{rawat2018centralized, rawat2016centralized}. They use a centralized multi-node repair (CMR) model with a single-node failure. 

\subsection{MDS codes}
Ye et al \cite{ye2018cooperative} outlined two main repair models: centralized report and co-operative. They propose that the co-operative approach is better for reducing the bandwidth consumed in the repair, and use maximum distance separable (MDS) code. Their repair method needs two rounds where a failed node uses helper nodes to download information, and the second round involves the failed node downloading information from other failed nodes. To implement an MDS code, the source file gets divided into $k$ blocks. There are then $r = n-k$ parity blocks, and where the codeword of a code is of length $n$. These codewords are stored in $n$ different storage areas.


\subsection{Reed-Solomon recovery}
% https://mortendahl.github.io/2017/08/13/secret-sharing-part3/
McEliece and Sarwate \cite{mceliece1981sharing} defined that the Shamir Secret Sharing method had a similar structure to Reed-Solomon coding. If we have elements of:

\begin{equation}
a = (a_0, a_1, .... a_{k-1})    
\end{equation}

and which is encoded into a codeword of:

\begin{equation}
D = (D_1, D_2, .... D_{r-1})    
\end{equation}

and where:

\begin{equation}
D_i = \sum_{i=0}^{k-1} a_j \alpha_i^j    
\end{equation}

The shares are then all of the $D_i$ values, and the secret is:

\begin{equation}
a_0=-\sum_{i=1}^{r-1} D_i    
\end{equation}

If we have $s$ shares of which $t$ are in error, it is possible to recover $\textbf{D}$ and $\textbf{a}$ when $s-2t \geq k$. Shamir's secret share system can then be defined as a special case of this, and where $r$ is a prime number, $k=0$, and $\alpha_i=i$.

Hineman et al \cite{hineman2021efficient} define that an MDS is required for Shamir secret sharing, of which Reed-Solomon is the most commonly used. They use a way of identifying possible symbols to be shared, and then using XOR operations rather than RS codes.

\subsubsection{Implementation}
Within Reed-Solomon codes, we define a vector for a message $M$ as $[m_0, m_1 ... + m_D]$ of which we derive a polynomial of:
\begin{equation}
F(X) = (m_0) + (m_1 . X) + ... + (m_D . X^D) 
\end{equation}

we then evaluate $F(X)$ for a fixed set of points, in order to generate the code word. Sugiyama et al \cite{sugiyama1975method} and \cite{gao2003new} defined an approach for reconstruction. This takes a potentially faulty polynomial $H$ from the shares and then runs an extended Euclidean algorithm to determine the original polynomial $G$. 


If there are $m+t$ shares and, at most $\lfloor t/2\rfloor$ are in error, the Reed-Solomon decoding algorithm can successfully recover them. Overall, we do not need to know which shares are in error. We can also determine which of the $m+t$ shares have an error. When there are more than $\lfloor t/2\rfloor$ shares in error, it is unlikely we will be able to reconstruct the secret \cite{Sarwate}. 



\subsection{Paillier key proof}
Kryptology uses the Pailler method to perform homomorphic encryption on the tokens. In order to prove the robustness of the Paillier keys they perform a zero-knowledge check on this. The work is documented in \cite{goldberg2019efficient}. The focus of the paper is to prove that a suitable private key has been created so that the public key has all the possible values within the given field, and without leaking anything about the private key. In Paillier, we pick two large prime numbers ($p$ and $q$). We then calculate a modulus ($N=pq$) and $\phi(N)=(p-1)(q-1)$. We then make sure that $gcd(pq,\phi(N))=1$. 

One of the key properties is to prove that the value of N is square-free (that is, it does not have a factor that is a square). Overall, Victor - the verifier - will not be able to factorize the modulus ($N$), so they will have to trust Peggy in the creation of a secure modulus. For example, Peggy could cheat, and rather than creating $N=p.q$, she could create $N=p.p$, and which is p squared ($N=p^2$). This will produce a weak key. 

In Paillier, Peggy picks two large prime numbers ($p$ and $q$). She then calculates a modulus ($N=pq$) and $\phi(N)=(p-1)(q-1)$. Now Victor wants Peggy to prove that the modulus is square-free. For the proof Peggy computes:

\begin{equation}
M=N^{-1} \pmod {\phi(N)}
\end{equation}

In an interactive proof, Victor (the verifier) then generates a number of random values as challenges ($x_i$), and passes these to Peggy. She then computes:

\begin{equation}
y_i = x_i^{M} \pmod N 
\end{equation}

Peggy passes these back to Victor and Victor then checks that:
\begin{equation}
x_i=y_i^N \mod N 
\end{equation}
for all values of $i$. If these are all true, Peggy has proven that the modulus is square-free, as she should not be able to generate the proofs if she has cheated. Overall, we can make this non-interactive (NI), by allowing Peggy the chance to create her own challenges, and then present these with the proofs.

The outline coding using the library from the Krytology library \cite{asecuritysite_38104}.

==> sections/04_consensus.tex <==
\section{Consensus in DKG}
A DKG (Distributed Key Generation) protocol allows for a public key to be generated from a shared secret that is stored by a number of parties ($n$). For this, we typically define a threshold ($t$) which is the number of nodes that must come together to rebuild the secret. Overall, there is no trusted dealer involved, and where we use threshold encryption and distributed signatures. A DKG transcript is used to define the correct information required to decrypt the secret share. This can be \emph{publicly verifiable} so that any party can validate their correctness \cite{gurkan2021aggregatable}. The main approaches to this include consensus algorithms and blockchain methods. A key focus is here there is more than one valid DKG transcript, and where parties must agree on the one to use. Overall, no DKG can have just one round for secrecy, as it is open to the \emph{rushing adversary} - which is the adversary that contributes last to the final distribution.


\subsection{Aggregatable and Publicly verifiable transcripts}
Gurkan et al \cite{gurkan2021aggregatable} define an Aggregatable DKG protocol and where transcripts contain all the information required for decrypting secret is publicly verifiable. Only valid transcripts should be aggregated.
With this all the parties can obtain secret shares – even when offline. There is also no need for a \emph{complaint} round, and which leads to fewer rounds. Overall, the secret key is a \emph{group element}, rather than a finite element. Instead of normal cryptography they use verifiable unpredictable function (VUF). VUF is a hard function that leads to a non-random looking output. The VUF is a group element and which is proved within the random oracle model and uses 10 pairings and six group elements. Threshold VUF can be used for verifiable random beacons.

The paper uses  Scrape \cite{\cite{cascudo2017scrape} } for Publicly Verifiable Secret Share (PVSS) – and where there is no need for complaint round.




\subsection{Leaderless}
Abraham et al \cite{abraham2021reaching} defines a protocol of Asynchronous Distributed Key Generation (A-DKG) that is resilient for $n/3$ dishonest or badly performing nodes. It has a constant number of rounds and has a $O(n^3 log(n))$ communication complexity. It requires a PKI infrastructure, and the following building blocks:

\begin{itemize}
\item Proposal Election (PE) protocol. This allows parties to agree on a valid proposal, after assessing a number of proposals.
\item Verifiable Gather protocol. This defines the proposals that have been seen by a party, and the ones they have not seen. 
\item Validated Asynchronous Byzantine Agreement (VABA) protocol. This creates a protocol which does not require leaders or an asynchronous DKG setup. 
\end{itemize}




==> sections/05_frost.tex <==
\section{Theshold DKG}


\subsection{FROST threshold Schnorr signature protocol}
One of the most important challenges within cybersecurity is key management. This is a way that organisations store encryption keys and can recall them when required. We also need a way to back up these keys, in case we lose them. One method of achieving this is to centralise our key management into a trusted server. This, though, can centralise our infrastructure, and it can become a target for attack.

An alternative is to use a Distributed Key Generation (DKG) infrastructure, and where we split the keys into a number of Shamir shares and then distribute these to a number of stored key stores. This is more secure and also resilient, and where we can create $n$ shares and with a $t$ threshold and where we can rebuild our data with at least $t$ shares. It should not be possible to reconstruct the key without gathering $t$ shares. In this way, we can either cope with a malicious key store or can cope with an outage on one or more of these.

In this case, we will use the FROST method defined by Komlo and Goldberg \cite{komlo2020frost}. With this, we use a share of a Schnorr signature across trusted parties, and where each of the key shares can be signed by each of the parties and where the validation signature can only be rebuilt when a given threshold is reached. Essentially, there are two core elements to the FROST method. The first is that n parties run a distributed key generation (DKG) service, and then agree on a verification key, and where each party has their own secret key. Then, any one of the parties involved can collaboratively generate a Schnorr signature. In Figure \ref{fig:fost}, we see that Bob, Alice and Carol have their own secret key. They then create a round where they create a verification key which is the aggregation of their public keys. This uses the Schnorr signature method, and where we can easily aggregate public keys together. The verification key will then be used to verify signatures. Each party will then hold a secret key ($i,sk_i$) and which is their long-term secret key, and also a verification key ($vk_i=sk_i G$). This verification key ($vk_i$) is then used to define the correctness of their signature signing shares, whereas the main verification ($vk$) checks the signed message for the group.

Next, we decide the signing threshold and how many signers are allowed to verify a message. In this case, we will do an any 2-from-3, and where Bob and Carol can come together and sign for a message (Figure \ref{fig:fost}).


\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/frost01.png}
\caption{FROST)}
\label{fig:fost}
\end{center}
\end{figure}

For a Schnorr signature, we first perform a key generation phase. Each party ($i$) create a random secret key ($sk$) and generators a validation key of:
\begin{equation*}
vk = sk \cdot G
\end{equation*}

For the signing process, we take the secret key ($sk$) and a message ($M$). Each party select a random nonce ($r$), and then computes:

\begin{equation*}
R = r \cdot G
c = H(M,R)
z= r + sk \cdot c \pmod p
Sig = (z,c)
\end{equation*}

To check the signature:

\begin{equation*}
R' = z \cdot G - c \cdot vk
c' = H(M,R')
\end{equation*}

We then check that $c'$ is equal to $c$. This works because:

\begin{equation}
\begin{aligned}
c' = H(M,R') &= H(M,z \cdot G - c \cdot vk) \\
&= H(M,(r + sk \cdot c) \cdot G - c \cdot vk)\\ 
&= H(M, r \cdot G + c \cdot sk \cdot G - c \cdot vk) \\
&= H(M,r \cdot G + c \cdot vk - c \cdot vk) \\
&= H(M,R) = c
\end{aligned}
\end{equation}


and where $H()$ is a hash on the content, $G$ is the base point on the curve, $sk$ is the secret key as a scalar value, and $vk$ is the public verifier point. 
In the following, we will add two new participants to a share: p1 (ID=1) and p2 (ID=2), and where we define an additional participant for p1 as p2 (ID-2), and vice verse. The first argument of NewDkgParticipant is the ID. This is followed by the threshold required to rebuild the shares. The next is the context of the message, and which avoids a replay attack. Finally, we have the curve type (Ed25519), and the last argument is the ID of the other share participant:

\begin{lstlisting}[language=golang]
Ctx := "Stop reply attack"
testCurve := curves.ED25519()
p1, _ := frost.NewDkgParticipant(1, 2, Ctx, testCurve, 2)
p2, _ := frost.NewDkgParticipant(2, 2, Ctx, testCurve, 1)
\end{lstlisting}

After the first round, we have a broadcast value, and a p2p share:

\begin{lstlisting}[language=golang]
bcast1, p2psend1, _ := p1.Round1(nil)
bcast2, p2psend2, _ := p2.Round1(nil)
\end{lstlisting}
The ID value of p2psend1 will contain the share (p2psend1 and p2psend2) for the given ID. For example, p2psend1[2] will contain the share for ID=2, and p2psend2[1] will contain the share for ID=1. We can then pass the shares:
\begin{lstlisting}[language=golang]
bcast := make(map[uint32]*frost.Round1Bcast)
p2p1 := make(map[uint32]*sharing.ShamirShare)
p2p2 := make(map[uint32]*sharing.ShamirShare)
bcast[1] = bcast1
bcast[2] = bcast2
p2p1[2] = p2psend2[1]
p2p2[1] = p2psend1[2]
\end{lstlisting}
For this, we exchange the shares, and where the first participant receives the share the second participant:
\begin{lstlisting}[language=golang]
p1.Round2(bcast, p2p1)
p2.Round2(bcast, p2p2)
fmt.Printf("\nSkShare P1: %x\n", p1.SkShare.Bytes())
fmt.Printf("SkShare P2: %x\n", p2.SkShare.Bytes())
fmt.Printf("\nVerification key P1: %x\n", p1.VerificationKey.ToAffineCompressed())
fmt.Printf("Verification key P2: %x\n", p2.VerificationKey.ToAffineCompressed())
\end{lstlisting}
P1 will have a secret key (p1.SkShare), and P2 will also have its own secret key (p2.SkShare). We will now have two verification keys on P1 and P2. These should be the same for each participant. Next, we will split the verification key into any two from three shares:
\begin{lstlisting}[language=golang]
s, _ := sharing.NewShamir(2, 3, myCurve)
\end{lstlisting}
These shares can then be distributed to participants. When we need to rebuild them we:

\begin{lstlisting}[language=golang]
sk, _ := s.Combine(&sharing.ShamirShare{Id: p1.Id, Value: p1.SkShare.Bytes()},&sharing.ShamirShare{Id: p2.Id, Value: p2.SkShare.Bytes()})
\end{lstlisting}

The value of sk will rebuild the secret back. We can then recreate the verification key with:
\begin{lstlisting}[language=golang]
vk := myCurve.ScalarBaseMult(sk)
rtn := vk.Equal(p1.VerificationKey)
if rtn {
 fmt.Printf("Verification keys are the same.\n")
 fmt.Printf("Verification key Round 2: %x\n", vk.ToAffineCompressed())
}
\end{lstlisting}

The outline coding using the library from the Krytology library is defined at \cite{asecuritysite_19437}.



\subsection{Threshold ECDSA}
With threshold ECDSA we can split the shares over a number of parties and then get each of these parties to sign a part of the signature, and then rebuild these.

\subsection{DKLS}
The DKLS [Doerner, Kondi, Lee, and Shelat) method \cite{doerner2019threshold} implements an ECDSA signing algorithm using threshold protocols. In this case, Bob and Alice will communicate using a DKG method, and then Bob will be able to create a valid signature. We can use the Kryptology library developed by Coinbase to implement 2-of-2 threshold ECDSA signing algorithm of the DKLS method. Once Bob and Alice have communicated, Bob will hold a signature for the message. We will then check this signature for its validity. 

 In \cite{asecuritysite_30932}, we can use the Kryptology library developed by Coinbase to implement 2-of-2 threshold ECDSA signing algorithm of the DKLS method. Once Bob and Alice have communicated, Bob will hold a signature for the message. We will then check this signature for its validity.

Initially, we split the secret key into two shares and distribute these to Bob and Alice, and which are stored as bob.SkA and alice.SkB. These will be used to generate a public key that Bob and Alice can use (bob.Pk and alice.Pk). This public key can be used to verify the generated digital signature. The following displays the secret shares and the public key:

\begin{lstlisting}[language=golang]
fmt.Printf("Message to sign: %s\n", msg)
fmt.Printf("\nAlice Secret Key: %x\n", alice.SkA.Bytes())
fmt.Printf("Alice Public Key: %x\n", alice.Pk.Bytes())
fmt.Printf("\nBob Secret Key: %x\n", bob.SkB.Bytes())
fmt.Printf("Bob Public Key: %x\n", bob.Pk.Bytes())
\end{lstlisting}

Bob generates a signature by communicating with Alice through DKG, and where the generated signature has two values: R and S. This is displayed as:

\begin{lstlisting}[language=golang]
fmt.Printf("Bob Signature: R:%x S:%x\n", bob.Sig.R, bob.Sig.S)
\end{lstlisting}

We can then take Bob's public key (bob.Pk.X and bob.Pk.Y), and then check that this signature is the valid against the public key.

\subsection{GG20}
The GG20 method \cite{gennaro2020one} method implements an ECDSA signing algorithm using threshold protocols. In this case, Bob and Alice will communicate using a DKG method, and then Bob will be able to create a valid signature. We can use the Kryptology library developed by Coinbase to implement 2-of-2 threshold ECDSA signing algorithm of the GG20 method. Once Bob and Alice have communicated, Bob will hold a signature for the message. We will then check this signature for its validity. We will thus split a private key up into two secret shares and then will be able to sign with the shares of the key. 

The focus of the paper [1] is to create an ECDSA signature using secret shares of a private key. In this way, we can create an ECDSA signature using multiple Shamir shares, and where the private is never actually revealed but split over two or more parties.

So, let's use the Coinbase Kryptology library to implement a 2-from-2 threshold ECDSA scheme using GG20 \cite{gennaro2020one}. Initially, we will use the secp256k1 curve and then generate a new private key (ikm).

This private key will not be stored on the parties which receive the shares, and can be deleted after the shares have been distributed. We can then generate the associated public key (pk) and split the key into a number of shares (sharesMap).

This public key will be used to check the signature that the parties create. We also create public shares which can be used to verify the shares created:

\begin{lstlisting}[language=golang]
pubSharesMap, _ := dealer.PreparePublicShares(sharesMap)
\end{lstlisting}

We then create Paillier keys which will be used to distribute the key signing.

The dealer of the shares is now setup. What we need now is for two parties to receive the shares, and for them to sign for a message (msg).

Next, we will create two participants (p1 and p2), and where p1 gets the first set of shares (sharesMap1), and the ID for these, and p2 gets the second set of shares (sharesMap2), and the required ID for these.

And then set them up for split the share. These will be run of either of the parties.

We then go into a number of rounds, and where s1 is run on one party, and s2 on another party.

Now each party can generate the shared signature.



We can then check the signature that has been generated against the public key. 



A 2-from-2 share is \href{https://asecuritysite.com/kryptology/sss_gg02}{here} and an any t-from-n share is \href{https://asecuritysite.com/kryptology/sss_gg03}{here}.


% Parking for now

\subsection{EthDKG: An Ethereum-based Distributed Key Generation Protocol}
EthDKG is defined in \cite{schindler2019ethdkg}, and allocates key pairs (public and private key) to trusted nodes. These can then be brought together to define a group public key. A signature is then generated by each node signing with their private key, and then the overall signature is generated by aggregating these signatures. The control of this is defined with a smart contract performing the operation of registering, sharing a subkey, disputing a subkey, saving a group key, and verifying a signature. The main events covered are registration received, subkey shared, and dispute successfully. 

\begin{itemize}
\item Registration. BLS key pairs are used to perform the key sharing, and where each client node can generate its own key pair. The public key from each node is then submitted along with a zero-knowledge proof against their identity.  A smart contract is then used to check the identity of the node and its rights to register.
\item Key sharing.  This runs a VSS and sends out encrypted shares, and associated verifications. The smart contract checks each of the shares and takes a hash of the transaction.
\item Dispute. Each client node checks the distributed shares, and posts a dispute for all the ones it thinks are incorrect. The smart contract checks whether the dispute is correct or not. If the dispute is correct, it will withdraw the shares from the specified node.
\item Finalisation. One node will then compute the overall public key, and where the smart contract will verify the generated key.
\end{itemize}

A demo of the system is given at \cite{Schindler}. 


\subsection{Aggregatable Distributed Key Generation}

Gurkan et al \cite{gurkan2021aggregatable} use an aggregable method for DKG and which can be publicly verified. The Rust implementation can be integrated from \cite{Kobigurk}. The code is currently experimental and should not be used in production.








==> sections/background.tex <==
\chapter{Research}



\section{Outline of use case}
In a basic use case, a file is encrypted with a unique encryption key, and then this key is split into a number of secret shares. When the key is regenerated, the key is rebuilt from the shares. The first part of the applied cryptography work has investigated: the application of Shamir Secret Shares (SSS), their performance; and the methods which can be integrated.

In the current implementation, we have three main stages:

\begin{itemize}
\item Key creation: Bob has a private key ($x$) and a public key ($Q=xG$). 
\item Encrypting document: When we want to encrypt a document (A) and we create 256-bit random key value, and then encrypt with an ECIES public key. At present this is encrypted with 256-bit AES CBC, but it would be an enhancement to use AES GCM. We then split the key into a number of shares and distribute it to trusted key stores.
\item Decrypting document: Bob will request a document, and which is recovered from the document storage network. We then match it to the required symmetric key, and call back the shares of the key. These are then reconstructed to reveal the original encryption key. Bob's private key is used for this.
\end{itemize}

With ECIES, we use a hybrid encryption method. Initially Bob has a private key ($x$) and a public key ($Q=xG$). To generate the encryption key, we create a random value ($r$) and compute:

\begin{equation}
R=rG
\end{equation}
and:
\begin{equation}
S=rQ
\end{equation}

The value of $S$ is then created as a symmetric key ($K$) and we encrypt the document with this key. To decrypt, Bob uses his private key ($x$) to recreate $S$:

\begin{equation}
S=xR
\end{equation}

In the product, the value of $R$ as an encryption key will be split into secret shares. The curve used in the existing implement is secp256k1, and which is used in Bitcoin and Ethereum. This curve supports the integration of digital signatures using ECDSA or EdDSA.

\section{Evaluation of SSS Methods}
This work has involved gathering a range of Shamir Secret Share methods, and experiments are currently being undertaken on their performance. There are a number of Shamir share implementations. These include:

\begin{itemize}
\item dsprenkels - \href{https://github.com/dsprenkels/sss-go}{here}.
\item SSSaas - \href{https://github.com/SSSaaS/sssa-golang}{here}.
\item codahale - \href{https://github.com/codahale/sss}{here}.
\item kryptology - \href{https://github.com/coinbase/kryptology}{here}.
\end{itemize}

Table \ref{table_1} outlines the result for creating 4,999,995 shares for a simple test. There will be more extensive tests undertaken.

\begin{center}
\begin{table}
\caption{Outline test for SSS}
\begin{tabular}{ | l | l | l |}
\hline
 Method & Time to split (s) & Time to reconstruct (s) \\ 
\hline
 Codahale & 112.1s & 13.9s \\ 
 Dsprenkels & 4.4s & 5.8s \\  
 SSSaaS & 64.1ms & 1.7s \\
 Kryptology & 11.2s & 214.4s \\
 \hline
\end{tabular}
\label{table_1}
\end{table}
\end{center}

It can be seen that SSSasS is the fastest in this simple evaluation.

\section{Kryptology}
The Coinbase Kryptology Golang library \cite{Kryptology} supports privacy-preserving crypto tokens, and integrates Shamir Secret Shares, EDCDSA threshold splitting, and partially homomorphic ElGamal encryption and the usage of hybrid encryption. The library is worthy to be investigated as it integrates some of the methods that are used within the Arcana product, and could be applied into areas of privacy-preserving techniques. For example, the library integrates Pedersen Verifiable Secret Shares, and which allows players in the secret shares to verify their shares, without revealing the secret. This involves a blinding process to allow the entities who receive the shares to check their validity. 

Over the past week, I have integrated six main demonstrators of the code:

\begin{itemize}
\item Simple curve integration. This integrates the generation of a private key scalar, and then determining the public key point value for a range of supported curves. Demo: [\href{https://asecuritysite.com/kryptology/ecc_simple}{here}].
\item BBS signing messages. Signing multiple messages with BBS. Demo: [\href{https://asecuritysite.com/kryptology/bbs_sign}{here}]: 
\item Accumulators. Accumulator. An accumulator can be used for zero-knowledge proof of knowledge. In this case we will use the BLS curve and create an accumulator and data a proof onto it, and then remove the proof. Demo: [\href{https://asecuritysite.com/kryptology/accumulator}{here}]: 
\item Authenticated ElGamal Encryption using Kryptology. Authenticated ElGamal. This implements a public key encryption method with authenticated ciphertext. Demo: [\href{https://asecuritysite.com/kryptology/elgamal01}{here}].
\item Shamir Secret Shares. Implementing SSS. With this we have a threshold of $t$ from $n$ shares. Demo: [\href{https://asecuritysite.com/kryptology/sss01}{here}].
\item Pedersen Verifiable Secret Sharing Scheme (PVSS) using Kryptology. With this we have a threshold of $t$ from $n$ shares and where the players can verify the shares they have. Demo: [\href{https://asecuritysite.com/kryptology/sss02}{here}].
\item Homomorphic Encryption. Homomorphic. This implements partial homomorphic encryption of adding and subtraction with ElGamal. Demo: [\href{https://asecuritysite.com/kryptology/hom}{here}].
\end{itemize}


\subsection{Curves supported}
Within elliptic curves, we can have a scalar value ($a$) and a base point on the curve ($G$). We then perform an add operation to produce another point on the curve as $aG$. This is the equivalent operation of adding the point $G$ for $a$ times. Normally we would define $aG$ as a public key point, and $a$ as a private key scalar value. Typically these operations are done within a finite field defined by prime number ($p$). In the case of Curve 25519, this prime number is $2^{255}-19$.

A sample example of using the Ed25519 curve, and with a private key of $x$ and a public key of $xG$. In the following case we will use $x=10$ and determine $10G$:

\begin{lstlisting}[language=golang]
package main

import (
	"fmt"

	"github.com/coinbase/kryptology/pkg/core/curves"
)

func main() {

	curve := curves.ED25519()

	x := curve.Scalar.New(10)
	xG := curve.Point.Generator().Mul(x)

	fmt.Printf("x=%x\n", x.Bytes())
	fmt.Printf("xG=%x", xG.ToAffineCompressed())

}

\end{lstlisting}

A sample run gives us:

\begin{lstlisting}
x=0a00000000000000000000000000000000000000000000000000000000000000

xG=2c7be86ab07488ba43e8e03d85a67625cfbf98c8544de4c877241b7aaafc7fe3
\end{lstlisting}

With the Ed25519 curve, we only need one of the co-ordinate points, and so the public key point is the same length as the private key scalar value. Normally, though, we only need to store the y co-ordinate value, as we can determine the x-cordinate from the y co-ordinate.

The Kryptology library supports a wide range of curves, including BLS (such as BLS 12377), Ed25519, P256, K256 (secp256k1 - as used in Bitcoin and Ethereum) and Pallas. The Boneh–Lynn–Shacham (BLS) signature method produces short signatures and use elliptic curve pairing (and which are also known as bilinear maps). These are particularly useful for Zero-Knowledge Proofs (ZKPs). Ed25519 uses Curve 25519 and is known to be a fast and efficient method for processing elliptic curves operations. A demo of the differing curves is given \href{https://asecuritysite.com/kryptology/ecc_simple}{here}.

\subsection{Shamir Secret Sharing method}
A core part of the Arcana product is the splitting of encryption keys into secret shares.  In 1979, Adi Shamir (the ‘S” in RSA) published a classic paper in the Communications of the ACM \cite{shamir1979share}. While a fairly old method, it is now being used to split up encryption keys, so let’s have a look at a basic implementation.

\subsubsection{Byzantine Fault Tolerance}
We need to start building systems which are fault-tolerant, and where we assume that sometimes our systems give us errors, or can be faulty, or that they have been taken over by a malicious agent. This will give us Byzantine Fault Tolerance (BFT) in our processing and decision-making. For example, let’s say we are processing a transaction, and have four checkers for the validity of the transaction. If we had one checker, then it may have an error or could be compromised by a hacker. But if we have four, then if three of the checkers were good, we would have an election, and take the majority vote. A checker which loses these elections may then be faulty or is compromised.

A perfect way of keeping things secure and creating resilience is to use Shamir Secret Sharing (SSS), and where we can distribute a secret, and then allow any n-from-m to recover the secret. In this way, Bob, Alice, Carol and Dave can share a secret, and then any three of them can come together and recreate the share. 

\subsubsection{Outline of method}

With secret sharing, we take a secret value and then share it with others. For example, we might have a share for Bob, Alice, Carol and Dave and then for three of them to come together to bring their shares together. First, we generate a polynomial, and which has a secret value. In the following example, we have a quadratic equation of $f(x)=2x^2 -2x + 5$ (Figure \ref{fig:quad}). The secret could be stored at $f(0)$ (the red line), and where we give Bob their y value for $x=1$ ($f(1)$ — the purple line), Carol the value at $x=2$ ($f(2)$ — the blue line), Dave the value at $x=3$ ($f(3)$ — the green line) and Alice the value at $x=4$ ($f(4)$ — the outer blue line). With the values of their own, they cannot recover $f(0)$, but if we have three of the values, we can recover it.

\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/quad01.png}
\caption{Example quadratic equation)}
\label{fig:quad}
\end{center}
\end{figure}

For an any 3-from-4, we can use a quadratic equation, such as $f(x)=20x^2-2x+10$, and where the value of 10 is the secret. Bob then gets the value of $f(x)$ when $x=1$. This can be defined as $f(1)$. Carol gets $f(2)$, Dave gets $f(3)$ and Alice gets $f(4)$. The secret value is thus $f(0)$. They then each know a point on the quadratic equation, and three of them can bring them back to recover the secret. In this case, we will generate a random polynomial of $ax^2+bx+secret$, and then distribute the shares to Bob, Alice, Carol and Dave.

\subsubsection{Shamir Secret Shares and Kryptology}

We can use the Kryptology library \cite{Kryptology} developed by Coinbase to implement Shamir Secret Shares. In this case, we will define $t$ for the threshold and $n$ for the number of shares \cite{asecuritysite_19437}.



\subsubsection{Pedersen Verifiable Shamir Shares}

With the Pedersen Verifiable Secret Sharing Scheme (PVSS) \cite{pedersen1991non}, we create a blinding factor (b), and then split this value into coefficients:
\begin{equation} 
g(x)=b+b_1 x+b_2 x^2 ...
\end{equation} \label{eqn}

The dealer (who is distributing the shares), initially privately sends out each share. For Bob:

\begin{equation} 
S_1=(p(1),g(1)) 
\end{equation} 

and for Alice:

\begin{equation} 
S2=(p(2),g(2)) 
\end{equation} 

and where the $p()$ is the secret share and $g()$ will be used to verify the share. The dealer also creates a number of commitments for elliptic curve point additions:

\begin{equation} 
C_1=p(1)+g(1)
\end{equation} 
\begin{equation} 
C_2=p(2)+g(2)
\end{equation} 

and so on. These are then passed to the entities involved. It will not be possible for any other player to reveal the secret share from the commitments, as the blinding factor has been applied. Figure \ref{fig:pvss} outlines the commitments.

\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/pvss.png}
\caption{PVSS)}
\label{fig:pvss}
\end{center}
\end{figure}

Each player receives a share then checks the commitment against the share elements. If they do not match, the player will tell the other players that they have a complaint against the dealer. They will then reveal their commitment and their share. The dealer will also reveal its commitment. Next, the players will then check who is right against the commitments. If the commitment does not match the share, they will remove the dealer from the game, if not, they will remove the accusing entity from the game.

We can use the Kryptology library developed by Coinbase to implement PVSS. In this case, we will define t for the threshold and n for the number of shares [\href{https://asecuritysite.com/kryptology/sss02}{here}]:

\begin{lstlisting}[language=golang]
package main

import (
	crand "crypto/rand"
	"fmt"
	"os"
	"strconv"

	"github.com/coinbase/kryptology/pkg/core/curves"
	"github.com/coinbase/kryptology/pkg/sharing"
)

func main() {

	msg := "Hello"
	var t uint32 = uint32(3)
	var n uint32 = uint32(4)
	argCount := len(os.Args[1:])

	if argCount > 0 {
		msg = os.Args[1]
	}
	if argCount > 1 {
		val, err := strconv.Atoi(os.Args[2])
		if err == nil {
			t = uint32(val)
		}
	}
	if argCount > 2 {
		val, err := strconv.Atoi(os.Args[3])
		if err == nil {
			n = uint32(val)
		}
	}

	curve := curves.ED25519()
	secret := curve.NewScalar().Hash([]byte(msg))

	pt := curve.ScalarBaseMult(secret)

	pedersen, _ := sharing.NewPedersen(t, n, pt)

	shares, _ := pedersen.Split(secret, crand.Reader)

	fmt.Printf("== Secret shares == %d from %d ===\n", t, n)
	for _, s := range shares.SecretShares {
		fmt.Printf("Share: %x\n", s.Bytes())
	}
	fmt.Printf("=================\n")

	fmt.Printf("== Blinding shares == %d from %d ===\n", t, n)
	for _, s := range shares.BlindingShares {
		fmt.Printf("Blinding shares: %x\n", s.Bytes())
	}
	fmt.Printf("=================\n")

	//	recovered, _ := pedersen.Combine(shares.SecretShares...)
	sG, _ := pedersen.Combine(shares.SecretShares...)
	bH, _ := pedersen.Combine(shares.BlindingShares...)

	fmt.Printf("Secret: %x\n", secret.Bytes())
	fmt.Printf("Recovered: %x\n", sG.Bytes())

	fmt.Printf("\nBlinding: %x\n", shares.Blinding.Bytes())
	fmt.Printf("Blinding Recovered: %x\n", bH.Bytes())

	err := shares.PedersenVerifier.Verify(shares.SecretShares[0], shares.BlindingShares[0])
	if err == nil {
		fmt.Printf("\nShare 1 verified\n")
	}
	err = shares.PedersenVerifier.Verify(shares.SecretShares[1], shares.BlindingShares[1])
	if err == nil {
		fmt.Printf("\nShare 2 verified\n")
	}

}
\end{lstlisting}

A sample run [\href{https://asecuritysite.com/kryptology/sss02}{here}]:

\begin{lstlisting}[language=script]
== Secret shares == 3 from 4 ===
Share: 0000000150eb0b9e5d50954c83bcec58a4a6b491b75849655ee955dcdc4c4c6a7767e092
Share: 000000024524c932a2cbbf2f800ef261e69decb27a3bc7d7eabda4f6706f28fe14ffed79
Share: 000000032baccdd2026ace45f92bd2de7763bffdb6700b4cf42bc90e83eaea3d34d4979d
Share: 000000040483197c7c2dc28fef138dce56f82e736bf513c47b33c22516bf9027d6e5defe
=================
== Secret shares == 3 from 4 ===
Blinding shares: 0000000108eeaf5d770301e932bb209c8d7d8c3a0d46cc86fba56ec5ccbfdf8c8a76350e
Blinding shares: 000000025a631f20f73bb0aa2c25dd42e55c758c7ceedc5b21f50df8eed5b8dcea3f8010
Blinding shares: 0000000317314991e644e98f89bb355bbf8683e324bcdc271d2b5df583c0be0983a5d528
Blinding shares: 0000000427347d569759a729b1eed8f72f3f6748ac2c13f0ed4516b98b80ef1056a93458
=================
Secret: 4eff951531f9509d0435c0c2b17e179b6dc58ff550aedbc1c78254825c0c70e8
Recovered: 4eff951531f9509d0435c0c2b17e179b6dc58ff550aedbc1c78254825c0c70e8Blinding: 0aaf48edb8d5d7dd03eeaf78cb2d77f67d3ff4b0aa39385a1d7f32166449f424
Blinding Recovered: 0aaf48edb8d5d7dd03eeaf78cb2d77f67d3ff4b0aa39385a1d7f32166449f424
Share 1 verified
Share 2 verified
\end{lstlisting}

\subsubsection{Paillier Homomorphic encryption}
With ElGamal we can implement homomorphic addition, and Kryptology uses this to preserve the privacy of the tokens created. Initially we have a private key of $x$ and a public key of:
\begin{equation} 
Y=xG
\end{equation} 

A cipher is made up of:
\begin{equation} 
C_1 = rG
\end{equation} 

and:
\begin{equation} 
C_2 = rY+M
\end{equation} 
 
The value of $M$ is then:

\begin{equation} 
M=vG
\end{equation} 

and where $v$ is the integer value that we want to operate on. To decrypt we basically take the private key (x) and compute:

\begin{equation} 
S = x C_1
\end{equation} 

and then recover the message with:

\begin{equation} 
M = C_2-S
\end{equation} 

If we add two ciphertext values (created from two random numbers of $r_1$ and $r_2$), we get:

\begin{equation} 
C_1=r_1 G + r_2 G = (r_1+r_2) G
\end{equation} 

and:
\begin{equation} 
C_2 = r_1 Y+r_2 Y+ M_1 + M_2 = (r_1+r_2)Y + (M_1 + M_2) 
\end{equation} 

When we decrypt, we create:
\begin{equation} 
S=x C_1 = x (r_1+r_2) G = (r_1+r_2) xG = (r_1+r_2)Y
\end{equation} 

and
\begin{equation} 
M=C_2-S =(r_1 +r_2) Y + M_1 + M_2 =  M_1 + M_2  - ((r_1+r_2)Y) = M_1 + M_2 
\end{equation} 

We then get a point on elliptic curve that relates to our result ($res.G$), and need to find $res$. We must search for the point to recover the result. The problem we have is:
\begin{equation} 
R=res.G
\end{equation} 

and we need to recover $m$ to find the result. This can be done by brute force if the result is relative small, but we can also solve for:
\begin{equation} 
res=log_G(R)
\end{equation} 

\begin{lstlisting}[language=golang]
package main

import (
	"fmt"
	"os"
	"strconv"

	"github.com/coinbase/kryptology/pkg/core/curves"
	"github.com/coinbase/kryptology/pkg/verenc/elgamal"
)

func main() {

	val1 := 5
	val2 := 4
	argCount := len(os.Args[1:])

	if argCount > 0 {
		val1, _ = strconv.Atoi(os.Args[1])

	}
	if argCount > 1 {
		val2, _ = strconv.Atoi(os.Args[2])
	}

	curve := curves.ED25519()
	pk, sk, _ := elgamal.NewKeys(curve)

	x1 := curve.Scalar.New(val1)

	x2 := curve.Scalar.New(val2)

	res1, _ := pk.HomomorphicEncrypt(x1)

	res2, _ := pk.HomomorphicEncrypt(x2)

	res1 = res1.Add(res2)

	dec, _ := res1.Decrypt(sk)

	pk_bytes, _ := pk.MarshalBinary()
	fmt.Printf("Public Key: %x\n", pk_bytes)
	sk_bytes, _ := sk.MarshalBinary()
	fmt.Printf("Private Key: %x\n", sk_bytes)

	fmt.Printf("Val1: %d\n", val1)
	val1_bytes, _ := res1.MarshalBinary()
	fmt.Printf(" Homomorphic encrypted: %x\n", val1_bytes)
	fmt.Printf("Val2: %d\n", val2)
	val2_bytes, _ := res2.MarshalBinary()
	fmt.Printf(" Homomorphic encrypted: %x\n", val2_bytes)

	fmt.Printf("Result (Homomorphic encrypted): %x\n", dec.ToAffineCompressed())

	for i := -1000; i < 1000; i++ {
		val := curve.Scalar.New(i)
		Val := curve.Point.Generator().Mul(val)

		rtn := Val.Equal(dec)
		if rtn == true {
			fmt.Printf("Result is %d \n", i)
			break
		}

	}
}
\end{lstlisting}

For this we can use the Baby-step, giant-step method or the Pollard's $\rho$ method.

\subsubsection{Crypto pairing}
With key pairing we have two cyclic groups ($G_1$ and $G_2$), and which are of an order of a prime number ($n$). A pairing on $(G_1,G_2,G_T)$ defines the function $e:G_1 \times G_2 \rightarrow G_T$, and where $g_1$ is the generator for $G_1$ and $g_2$ is the generator for $G_2$. If we have the points of $U_1$ and $U_2$ on $G_1$ and $V_1$ and $V_2$ on $G_2$, we get the bi-linear mapping of:

\begin{equation} 
e(U_1+U_2,V_1) =e(U_1,V_1) \times e(U_2,V_1) \\
e(U_1,V_1+V_2) =e(U_1,V_1) \times e(U_1,V_2)
\end{equation} 

If $U$ is a point on $G_1$, and $V$ is a point on $G_2$, we get:
\begin{equation} 
e(aU,bV) =e(U,V)^{ab}
\end{equation} 

If $G_1$ and $G_2$ are the same group, we get a symmetric grouping ($G_1 = G_2 = G$), and the following commutative property will apply:

\begin{equation} 
e(U^a,V^b) = e(U^b,V^a) = e(U,V)^{ab} = = e(V,U)^{ab}
\end{equation} 

The computation of $e$ should be efficient in computation time. The outline coding using the library from the Kryptology library is [\href{https://asecuritysite.com/kryptology/pairing}{here}]:

\begin{lstlisting}[language=golang]
package main

import (
	"fmt"
	"math/big"
	"os"
	"strconv"

	bls12381 "github.com/coinbase/kryptology/pkg/core/curves/native/bls12-381"
)

func main() {

	val1 := int64(10)
	val2 := int64(100)

	argCount := len(os.Args[1:])

	if argCount > 0 {
		val1, _ = strconv.ParseInt(os.Args[1], 10, 64)
	}
	if argCount > 1 {
		val2, _ = strconv.ParseInt(os.Args[2], 10, 64)
	}

	bls := bls12381.NewEngine()
	g1, g2 := bls.G1, bls.G2
	gt := bls.GT()

	// e(a*G1, b*G2) = e(b*G1, a*G2)
	{
		a, b := big.NewInt(val1), big.NewInt(val2)
		G1, G2 := g1.One(), g2.One()

		P1 := g1.New()
		g1.MulScalar(P1, G1, a)

		P2 := g2.New()
		g2.MulScalar(P2, G2, b)

		e0, _ := bls.AddPair(P1, P2).Result()

		P1 = g1.New()
		g1.MulScalar(P1, G1, b)

		P2 = g2.New()
		g2.MulScalar(P2, G2, a)

		e1, _ := bls.AddPair(P1, P2).Result()

		if e0.Equal(e1) {
			fmt.Printf("Pairing: e(%d G1,%d G2)=e(%d G1, %d G2)\n", val1, val2, val2, val1)
		}

	}

	// e(a*G1, b*G2) = e(a*b*G1, G2)
	{
		a, b := big.NewInt(val1), big.NewInt(val2)
		G1, G2 := g1.One(), g2.One()

		P1 := g1.New()
		g1.MulScalar(P1, G1, a)

		P2 := g2.New()
		g2.MulScalar(P2, G2, b)

		e0, _ := bls.AddPair(P1, P2).Result()

		P1 = g1.New()
		g1.MulScalar(P1, G1, new(big.Int).Mul(a, b))

		P2 = G2

		e1, _ := bls.AddPair(P1, P2).Result()

		if e0.Equal(e1) {
			fmt.Printf("Pairing: e(%d G1, %d G2)=e(%d G1,  G2)\n", val1, val2, val1*val2)
		}

	}

	// e(a*G1, b*G2) = e(G1, G2)^c
	{
		a, b := big.NewInt(val1), big.NewInt(val2)
		c := new(big.Int).Mul(a, b)
		G1, G2 := g1.One(), g2.One()
		e0, _ := bls.AddPair(G1, G2).Result()

		P1, P2 := g1.New(), g2.New()
		g1.MulScalar(P1, G1, a)
		g2.MulScalar(P2, G2, b)
		e1, _ := bls.AddPair(P1, P2).Result()

		gt.Exp(e0, e0, c)

		if e0.Equal(e1) {
			fmt.Printf("Pairing: e(%d G1,%d G2)=e(G1,G2)^ %d\n", val1, val2, val1+val2)
		}

	}

}
\end{lstlisting}




A sample run:

\begin{lstlisting}[language=script]
a=10
b=100
Pairing confirmed: e(10 G1,100 G2)=e(100 G1, 10 G2)
Pairing confirmed: e(10 G1, 100 G2)=e(1000 G1,  G2)
Pairing confirmed: e(10 G1,100 G2)=e(G1,G2)^ 110
\end{lstlisting}

\subsubsection{Paillier key proof}
Kryptology uses the Pailler method to perform homomorphic encryption on the tokens. In order to prove the robustness of the Paillier keys they perform a zero-knowledge check on this. The work is documented in \cite{goldberg2019efficient}. The focus of the paper is to prove that a suitable private key has been created, so that the public key has all the possible values within the given field, and without leaking anything about the private key. In Paillier, we pick two large prime numbers ($p$ and $q$). We then calculate a modulus ($N=pq$) and $\phi(N)=(p-1)(q-1)$. We then make sure that $gcd(pq,\phi(N))=1$. 

One of the key properties is to prove that the value of N is square free (that is, it does not have a factor that is a square). Overall, Victor - the verifier - will not be able to factorize the modulus ($N$), so will have to trust Peggy in the creation of a secure modulus. For example, Peggy could cheat, and rather than creating $N=p.q$, she could create $N=p.p$, and which is p squared ($N=p^2$). This will produce a weak key. 

In Paillier, Peggy picks two large prime numbers ($p$ and $q$). She then calculates a modulus ($N=pq$) and $\phi(N)=(p-1)(q-1)$. Now Victor wants Peggy to prove that the modulus is square-free. For the proof Peggy computes:

\begin{equation}
M=N^{-1} \pmod {\phi(N)}
\end{equation}

In an interactive proof, Victor (the verifier) then generates a number of random values as challenges ($x_i$), and passes these to Peggy. She then computes:

\begin{equation}
y_i = x_i^{M} \pmod N 
\end{equation}

Peggy passes these back to Victor and Victor then checks that:
\begin{equation}
x_i=y_i^N \mod N 
\end{equation}
for all values of $i$. If these are all true, Peggy has proven that the modulus is square-free, as she should not be able to generate the proofs if she has cheated. Overall, we can make this non-interactive (NI), by allowing Peggy the chance to create her own challenges, and then present these with the proofs.

The outline coding using the library from the Krytology library [\href{https://asecuritysite.com/kryptology/zkpal}{here}]::

\begin{lstlisting}[language=golang]
package main

import (
	"crypto/rand"
	"fmt"
	"math"
	"math/big"

	crypto "github.com/coinbase/kryptology/pkg/core"
)

func main() {

	p, _ := rand.Prime(rand.Reader, 128)
	q, _ := rand.Prime(rand.Reader, 128)
	N := new(big.Int).Mul(p, q)
	PHI := new(big.Int).Mul(new(big.Int).Sub(p, big.NewInt(1)), new(big.Int).Sub(q, big.NewInt(1)))

	PsfProofLength := 5

	// 1. M = N^{-1} mod \phi(N)
	M, _ := crypto.Inv(N, PHI)

	// 2. Generate challenges
	x := make([]*big.Int, PsfProofLength)
	for i := 0; i < PsfProofLength; i++ {
		x[i], _ = rand.Int(rand.Reader, new(big.Int).SetUint64(uint64(math.Pow(2, 64))))
	}

	proof := make([]*big.Int, PsfProofLength)
	// 3. Create proofs y_i = x_i^M mod N
	for i, xj := range x {

		yi, _ := crypto.Exp(xj, M, N)
		proof[i] = yi
	}

	fmt.Printf("p=%s\n", p)
	fmt.Printf("q=%s\n", q)
	fmt.Printf("N=%s\n", N)
	fmt.Printf("PHI=%s\n", PHI)
	fmt.Printf("\nChallenges:\t%v\n", x)
	fmt.Printf("Proof:\t%v\n", proof)

	proven := true
	for j, xj := range x {
		// 4. Proof: yj^N == x mod N return false

		lhs, _ := crypto.Exp(proof[j], N, N)

		if lhs.Cmp(xj) != 0 {
			fmt.Printf("Failed at %d\n", j)
			proven = false
		}
	}
	if proven == true {
		fmt.Printf("\nZero knowledge proof of safe Paillier\n")
	} else {
		fmt.Printf("\nNo Zero knowledge proof of safe Paillier\n")
	}

	fmt.Printf("\n\n== Now trying with an incorrect value of N=p^2 ==\n")

	N = new(big.Int).Mul(p, p)
	PHI = new(big.Int).Mul(new(big.Int).Sub(p, big.NewInt(1)), new(big.Int).Sub(p, big.NewInt(1)))

	proof = make([]*big.Int, PsfProofLength)
	// 3. Create proofs y_i = x_i^M mod N
	for i, xj := range x {

		yi, _ := crypto.Exp(xj, M, N)
		proof[i] = yi
	}

	fmt.Printf("p=%s\n", p)
	fmt.Printf("N=%s\n", N)
	fmt.Printf("PHI=%s\n", PHI)
	fmt.Printf("\nChallenges:\t%v\n", x)
	fmt.Printf("Proof:\t%v\n", proof)

	proven = true
	for j, xj := range x {
		// 4. Proof: yj^N == x mod N return false

		lhs, _ := crypto.Exp(proof[j], N, N)

		if lhs.Cmp(xj) != 0 {
			fmt.Printf("[Failed at %d]", j)
			proven = false
		}
	}
	if proven == true {
		fmt.Printf("\nZero knowledge proof of safe Paillier\n")
	} else {
		fmt.Printf("\nNo Zero knowledge proof of safe Paillier\n")
	}

}
\end{lstlisting}


A sample run is:
\begin{lstlisting}[language=script]
p=272607875711507234568172267871128963309
q=295946972516113719350378532078127656991
N=80677475500869576284216027503952826078439882763776608467923415825330976343219
PHI=80677475500869576284216027503952826077871327915548987514004865025381719722920

Challenges: [6175083952328541262 8170758500240932032 690144035803220448 5251383100325791414 7491250541467116415]
Proof:  [11964768429949674995906973048072290410298740842351249440155864963629295066643 2404036667536209695550094652200905842055096939969209457294393748537640760745 40213555573116455989223390360860064550186560820959033554469884782324844562896 52274994561541289937830320424416180467927177634778522999370893526641867564866 48843463049104864058386473913402375195965387767392969916582915710419561820741]

Zero knowledge proof of safe Paillier


== Now trying with an incorrect value of N=p^2 ==
p=272607875711507234568172267871128963309
N=74315053899940576031754513999406594897046717010370080236134373721813068229481
PHI=74315053899940576031754513999406594896501501258947065766998029186070810302864

Challenges: [6175083952328541262 8170758500240932032 690144035803220448 5251383100325791414 7491250541467116415]
Proof:  [48347497314044952093421350958061044670781973850949883675536730894971919557470 10658399863087440754746008212552663340496243739712655818209208097999235794672 32586614850160003802408771853260820571836860873070529326104339164882528234538 57983605267606520649471600773805506019743872785122299504104128122615372714735 2095494264165920873205461901730045396708273073195597895993911748465314990906]
[Failed at 0][Failed at 1][Failed at 2][Failed at 3][Failed at 4]
No Zero knowledge proof of safe Paillier
\end{lstlisting}

\subsection{Accumulators}
In this case, we will look at an accumulator method using Bilinear Maps, as first proposed by Lan Nyugen \cite{nguyen2005accumulators}. An accumulator allows Bob to add values onto a fixed-length digest, and to provide proof of the values added, without revealing them within the accumulated value. In this case, we will add a message onto an accumulator for a given message, and then we will remove it to show that the accumulator goes back to its original state. In this was Bob can prove that he knows something without actually revealing it to Alice, and where Bob can provide proof to it. In this case, we will use the Kyptography library from Coinbase, and add a message onto an accumulator, to prove that we know the message without actually revealing it. After we generate the proof, we will remove the message from the accumulator, and prove that it has gone back to its original value. Overall, we can add and remove any number of elements, and prove multiple proofs in a single round.
\subsubsection{Creating an accumulator}

We can create an accumulator with the BLS curve (BLS 12381). For this we generate a random nonce and generated a shared secret key for the proof:
\begin{lstlisting}[language=golang]
curve := curves.BLS12381(&curves.PointBls12381G1{})
	var seed [32]byte
	key, _ := new(accumulator.SecretKey).New(curve, seed[:])
\end{lstlisting}

We are not generating a random seed here, but, in practice, it would be a random value. Next, we can create the new accumulator with this secret key:
\begin{lstlisting}[language=golang]
acc, _ := new(accumulator.Accumulator).New(curve)
\end{lstlisting}
Now we can add a message as an element onto the accumulator:
\begin{lstlisting}[language=golang]
element := curve.Scalar.Hash([]byte(msg))
	_, _ = acc.Add(key, element)
\end{lstlisting}	

We can then share the accumulator value to show that we know the message. If we want, we can now remove the message from the accmulator with:
\begin{lstlisting}[language=golang]
_, _ = acc.Remove(key, element)
\end{lstlisting}

In this case we will use the BLS curve to provide our accumulator [here]:
\begin{lstlisting}[language=golang]
package mainimport (
	"fmt"
	"os"	"github.com/coinbase/kryptology/pkg/accumulator"
	"github.com/coinbase/kryptology/pkg/core/curves"
)func main() {	msg := "Hello"
	argCount := len(os.Args[1:])	if argCount > 0 {
		msg = os.Args[1]
	}	curve := curves.BLS12381(&curves.PointBls12381G1{})
	var seed [32]byte
	key, _ := new(accumulator.SecretKey).New(curve, seed[:])	acc, _ := new(accumulator.Accumulator).New(curve)	element := curve.Scalar.Hash([]byte(msg))	rtn, _ := acc.MarshalBinary()	fmt.Printf("Before add: %x\n", rtn)	_, _ = acc.Add(key, element)	rtn, _ = acc.MarshalBinary()	fmt.Printf("\nAfter add: %x\n", rtn)	_, _ = acc.Remove(key, element)
	rtn, _ = acc.MarshalBinary()	fmt.Printf("\nAfter remove: %x\n", rtn)}
\end{lstlisting}

A sample run:

\begin{lstlisting}[language=script]
Message to prove: Hello
Nonce: 0000000000000000000000000000000000000000000000000000000000000000
Key: 2007ec86a2ab79613fc0294e058151ddc74db38b0cde95a4678eb91f1258f31b400a424c5331323338314731
Before add: 3097f1d3a73197d7942695638c4fa9ac0fc3688c4f9774b905a14e3a3f171bac586c55e83ff97a1aeffb3af00adb22c6bb0a424c5331323338314731After add: 30a2ad98cb32af3afdaedac08e48e61c67929578f78d2a0985f5f55bfbe8ede8747b5f917ce2be90477bae72c4ae7734430a424c5331323338314731After remove: 3097f1d3a73197d7942695638c4fa9ac0fc3688c4f9774b905a14e3a3f171bac586c55e83ff97a1aeffb3af00adb22c6bb0a424c5331323338314731
\end{lstlisting}

A demo of accumulators is given \href{https://asecuritysite.com/kryptology/accumulator}{here}.

\subsection{Feldman Verifiable Secret Sharing Scheme }
With secret sharing, we take a secret value and then share it with others. For example we might have a share for Bob, Alice, Carol and Dave and then for three of them to come together to bring their shares together. For an any 3-from-4, we can use a quadratic equation, such as $f(x)=20 x - 2 x + 10$, and where the value of 10 is the secret. Bob then gets the value of $f(x)$ when $x=0$. This can be defined as $f(1)$. Carol gets $f(2)$, Dave gets $f(3)$ and Alice gets $f(4)$. The secret value is thus $f(0)$. They then each know a point on the quadratic equation, and three of them can bring then back to recover the secret. In this case we will generate a random polynomial of $a x^2 + b x + secret$, and then distribute the shares to Bob, Alice, Carol and Dave. Finally we will recover the secret from three of these shares (Bob, Carol and Dave). In 1987, Paul Feldman published a paper which proposed using the homomorphic encryption properties of exponation to create verifiable shares, and where a dealer creates the secret shares and distributed them to the players. They also publish an overall commitment to the shares and where each player can check that their share is valid, without revealing any information about the secret share, and any other player's secret share.

How do we cope with a dishonest dealer? How do the entities who receive the shares verify that they are valid? Well one of the best ways was developed by Paul Feldman and is defined as a Verifiable Secret Sharing (VSS) method \cite{feldman1987practical}. The great advantage of this method is that we can use any homomorphic encryption approach.
For this we create a group $G$ using a prime number $p$ and a generator $g$ (typically a value of $g=2$ or $g=5$ is used). Overall the dealer creates a secret ($s$) and a random polynomial ($f(x)$), and where $f(0)=s$. For example:

\begin{equation*}
f(x) = 5 + 2x + 4x^2
\end{equation*}

in this case, the secret is 5, and $f(1)$ is 7, f(2) is 25, $f(3)$ is 47 and $f(4)$ is 77. For any 3-from-4 we can distribute points (1,7), (2,25), (3,47) and (4,77) to each of the players. Each player gets one point on the curve. With three points the players will then be able to discover the quadradic equation, and reveal the secret. With just one or two points, it will be impossible to do this. This is at the core of the Shamir method. But how do the players know they are getting a valid share of the secret, without revealing the secret? Well we have:
\begin{equation*}
f(x) = s + a_1 x + a_2 x^2 + ...
\end{equation*}We can then create commitments as:

\begin{itemize}
\item $c_0 = g^s \pmod p$
\item $c_1 = g^{a_1} \pmod p$
\item $c_2 = g^{a_2} \pmod p$
\end{itemize}

It is then possible for every player $i$ to verify that:
\begin{equation*}
v = f(i) \pmod p
\end{equation*}

and check:
\begin{equation*}
\displaystyle g^{v}=c_{0}c_{1}^{i}c_{2}^{i^{2}}\cdots c_{t}^{i^{t}}=\prod _{j=0}^{t}c_{j}^{i^{j}}=\prod _{j=0}^{t}g^{a_{j}i^{j}}=g^{\sum _{j=0}^{t}a_{j}i^{j}}=g^{f(i)}
\end{equation*}

This operation is also done using $\pmod p$.

We can use the Kryptology library developed by Coinbase to implement Felman Verifiable Shamir Secret (VSS) Shares. In this case we will define $t$ for the threshold and $n$ for the number of shares:


\begin{lstlisting}[language=golang]
package main

import (
	crand "crypto/rand"
	"fmt"
	"os"
	"strconv"

	"github.com/coinbase/kryptology/pkg/core/curves"
	"github.com/coinbase/kryptology/pkg/sharing"
)

func main() {

	msg := "Hello"
	var t uint32 = uint32(3)
	var n uint32 = uint32(5)
	argCount := len(os.Args[1:])

	if argCount > 0 {
		msg = os.Args[1]
	}
	if argCount > 1 {
		val, err := strconv.Atoi(os.Args[2])
		if err == nil {
			t = uint32(val)
		}
	}
	if argCount > 2 {
		val, err := strconv.Atoi(os.Args[3])
		if err == nil {
			n = uint32(val)
		}
	}

	testCurve := curves.ED25519()
	scheme, _ := sharing.NewFeldman(t, n, testCurve)

	secret := testCurve.Scalar.Hash([]byte(msg))

	fmt.Printf("=== Feldman Verifiable Secret Shares === ")
	fmt.Printf("\nMessage: %s\nScheme: %d from %d\nOriginal secret: %x\n", msg, t, n, secret.Bytes())

	fmt.Printf("\nSplitting shares:\n")
	verifiers, shares, _ := scheme.Split(secret, crand.Reader)

	for _, s := range shares {
		rtn := verifiers.Verify(s)
		if rtn == nil {
			fmt.Printf(" Share %d: %x [Valid]\n", s.Id, s.Value)
		}

	}

	fmt.Printf("\nNow combining with all the shares ...\n")

	rSecret, err := scheme.Combine(shares...)

	if err == nil {
		fmt.Printf("Recovered secret: %x\n", rSecret.Bytes())
	} else {
		fmt.Printf("Cannot recover from all shares\n")
	}

	fmt.Printf("\nNow combining with two shares ...\n")
	rSecret, err = scheme.Combine(shares[0],shares[1])

	if err == nil {
		fmt.Printf("Recovered secret: %x\n", rSecret.Bytes())
		fmt.Printf("\nNow combining with two shares ...\n")
	} else {
		fmt.Printf("Cannot recover from two shares\n")
	}

	fmt.Printf("\nNow combining with three shares ...\n")
	rSecret, err = scheme.Combine(shares[0],shares[1],shares[2])

	if err == nil {
		fmt.Printf("Recovered secret: %x\n", rSecret.Bytes())
	} else {
		fmt.Printf("Cannot recover from three shares\n")
	}

}

\end{lstlisting}


A sample run:

\begin{lstlisting}[language=golang]
=== Feldman Verifiable Secret Shares === 
Message: hello
Scheme: 3 from 5
Original secret: b586c3423482ab97d876ce24cab8bd8ab84e22ac3a52a8dfbb330bbe92a3260f

Splitting shares:
 Share 1: 5e3fb175d1e82cddb5613c7682d544efeb5cf7ddb2cf92eb47613c96ad5dc10a [Valid]
 Share 2: f3649e7834e513292e70fef2889c1f6ffaac38a0b4cd5466fe45b790a5f7fe09 [Valid]
 Share 3: 74f78a4b5d77607b41a2149bdd0d4e0ae43ee6f23f4cee4fdfe17bad7a71df0c [Valid]
 Share 4: f4228191313c007c195b87cba12ff1aba81200d6544b5fa8ea348aec2ccb6203 [Valid]
 Share 5: 4d8f6c04e6f917db62d445ca92f5c67d48288649f3caa76f203fe24dbc04890d [Valid]

Now combining with all the shares ...
Recovered secret: b586c3423482ab97d876ce24cab8bd8ab84e22ac3a52a8dfbb330bbe92a3260f

Now combining with two shares ...
Cannot recover from two shares

Now combining with three shares ...
Recovered secret: b586c3423482ab97d876ce24cab8bd8ab84e22ac3a52a8dfbb330bbe92a3260f
\end{lstlisting}

The running code is \href{https://asecuritysite.com/kryptology/sss_fel}{here}.

\subsection{Distributed key generation (DKG) using FROST threshold Schnorr signature protocol}
One of the most important challenges within cybersecurity is key management. This is a way that organisations store encryption keys and can recall them when required. We also need a way to back up these keys, in case we lose them. One method of achieving this is to centralise our key management into a trusted server. This, though, can centralise our infrastructure, and it can become a target for attack.

An alternative is to use a Distributed Key Generation (DKG) infrastructure, and where we split the keys into a number of Shamir shares, and then distribute these to a number of stored key stores. This is more secure and also resilient, and where we can create $n$ shares and with a $t$ threshold, and where we can rebuild our data with at least $t$ shares. It should not be possible to reconstruct the key without gathering $t$ shares. In this way, we can either cope with a malicious key store or can cope with an outage on one or more of these.

In this case, we will use the FROST method defined by Komlo and Goldberg \cite{komlo2020frost}. With this, we use a share of a Schnorr signature across trusted parties, and where each of the key shares can be signed by each of the parties, and where the validation signature can only be rebuilt when a given threshold is reached. Essentially there are two core elements to the FROST method. The first is that n parties run a distributed key generation (DKG) service, and then agree on a verification key, and where each party has their own secret key. Then any one of the parties involved can collaboratively generate a Schnorr signature. In the following diagram we see that Bob, Alice and Carol have their own secret key. They then create a round where the create a verification key which is the aggregation of their public keys. This uses the Schnorr signature method, and where we can easily agreegate public keys together. The verification key will then be used to verify signatures. Each party will tehn hold a secret key ($i,sk_i$) and which is there long term secret key, and also a verification key ($vk_i=sk_i G$). This verification key ($vk_i$) is then used to define the correctness of their signature signing shares, whereas the main verification ($vk$) checks the signed message for the group.

Next we decide the signing threshold, and how many signers are allowed to verify a message. In this case, we will do an any 2-from-3, and where Bob and Carol can come together and sign for a message (Figure \ref{fig:fost}).


\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/frost01.png}
\caption{FROST)}
\label{fig:fost}
\end{center}
\end{figure}

For a Schnorr signature we first perform a key generation phase. Each party ($i$) create a random secret key ($sk$) and generators a validation key of:
\begin{equation*}
vk = sk \cdot G
\end{equation*}

For the signing process we take the secret key ($sk$) and a message ($M$). Each party select a random nonce ($r$), and then computes:

\begin{equation*}
R = r \cdot G
c = H(M,R)
z= r + sk \cdot c \pmod p
Sig = (z,c)
\end{equation*}

To check the signature:

\begin{equation*}
R' = z \cdot G - c \cdot vk
c' = H(M,R')
\end{equation*}

We then check that $c'$ is equal to $c$. This works because:

\begin{equation}
\begin{aligned}
c' = H(M,R') &= H(M,z \cdot G - c \cdot vk) \\
&= H(M,(r + sk \cdot c) \cdot G - c \cdot vk)\\ 
&= H(M, r \cdot G + c \cdot sk \cdot G - c \cdot vk) \\
&= H(M,r \cdot G + c \cdot vk - c \cdot vk) \\
&= H(M,R) = c
\end{aligned}
\end{equation}


and where $H()$ is a hash on the content, $G$ is the base point on the curve, $sk$ is the secret key as a scalar value, and $vk$ is the public verifier point. 
In the following, we will add two new participants to a share: p1 (ID=1) and p2 (ID=2), and where we define an additional participant for p1 as p2 (ID-2), and vice verse. The first argument of NewDkgParticipant is the ID. This is followed by the threshold required to rebuild the shares. The next is the context of the message, and which avoids a replay attack. Finally, we have the curve type (Ed25519), and the last argument is the ID of the other share participant:

\begin{lstlisting}[language=golang]
Ctx := "Stop reply attack"
testCurve := curves.ED25519()
p1, _ := frost.NewDkgParticipant(1, 2, Ctx, testCurve, 2)
p2, _ := frost.NewDkgParticipant(2, 2, Ctx, testCurve, 1)
\end{lstlisting}

After the first round, we have a broadcast value, and a p2p share:

\begin{lstlisting}[language=golang]
bcast1, p2psend1, _ := p1.Round1(nil)
bcast2, p2psend2, _ := p2.Round1(nil)
\end{lstlisting}
The ID value of p2psend1 will contain the share (p2psend1 and p2psend2) for the given ID. For example, p2psend1[2] will contain the share for ID=2, and p2psend2[1] will contain the share for ID=1. We can then pass the shares:
\begin{lstlisting}[language=golang]
bcast := make(map[uint32]*frost.Round1Bcast)
p2p1 := make(map[uint32]*sharing.ShamirShare)
p2p2 := make(map[uint32]*sharing.ShamirShare)
bcast[1] = bcast1
bcast[2] = bcast2
p2p1[2] = p2psend2[1]
p2p2[1] = p2psend1[2]
\end{lstlisting}
For this, we exchange the shares, and where the first participant receives the share the second participant:
\begin{lstlisting}[language=golang]
p1.Round2(bcast, p2p1)
p2.Round2(bcast, p2p2)
fmt.Printf("\nSkShare P1: %x\n", p1.SkShare.Bytes())
fmt.Printf("SkShare P2: %x\n", p2.SkShare.Bytes())
fmt.Printf("\nVerification key P1: %x\n", p1.VerificationKey.ToAffineCompressed())
fmt.Printf("Verification key P2: %x\n", p2.VerificationKey.ToAffineCompressed())
\end{lstlisting}
P1 will have a secret key (p1.SkShare), and P2 will also have its own secret key (p2.SkShare). We will now have two verification keys on P1 and P2. These should be the same for each participant. Next, we will split the verification key into any two from three shares:
\begin{lstlisting}[language=golang]
s, _ := sharing.NewShamir(2, 3, myCurve)
\end{lstlisting}
These shares can then be distributed to participants. When we need to rebuilt them we:
\begin{lstlisting}[language=golang]
sk, _ := s.Combine(&sharing.ShamirShare{Id: p1.Id, Value: p1.SkShare.Bytes()},&sharing.ShamirShare{Id: p2.Id, Value: p2.SkShare.Bytes()})
\end{lstlisting}
The value of sk will rebuild the secret back. We can then recreate the verification key with:
\begin{lstlisting}[language=golang]
vk := myCurve.ScalarBaseMult(sk)
rtn := vk.Equal(p1.VerificationKey)
if rtn {
 fmt.Printf("Verification keys are the same.\n")
 fmt.Printf("Verification key Round 2: %x\n", vk.ToAffineCompressed())
}
\end{lstlisting}

The outline coding using the library from the Krytology library:

\begin{lstlisting}[language=golang]
package main

import (
	"fmt"

	"github.com/coinbase/kryptology/pkg/core/curves"
	"github.com/coinbase/kryptology/pkg/dkg/frost"
	"github.com/coinbase/kryptology/pkg/sharing"
)

// Test dkg round1 works for 2 participants
func main() {

	// Round 1

	Ctx := "string to prevent replay attack"
	myCurve := curves.ED25519()

	fmt.Printf("=== Round 1 let's generate secret keys ===\n")

	p1, _ := frost.NewDkgParticipant(1, 2, Ctx, myCurve, 2)


	p2, _ := frost.NewDkgParticipant(2, 2, Ctx, myCurve, 1)

	bcast1, p2psend1, _ := p1.Round1(nil)
	bcast2, p2psend2, _ := p2.Round1(nil)

	fmt.Printf("\n=== Round 2 let's generate the verification key ===\n")
	bcast := make(map[uint32]*frost.Round1Bcast)
	p2p1 := make(map[uint32]*sharing.ShamirShare)
	p2p2 := make(map[uint32]*sharing.ShamirShare)
	bcast[1] = bcast1
	bcast[2] = bcast2
	p2p1[2] = p2psend2[1]
	p2p2[1] = p2psend1[2]

	// Running round 2
	p1.Round2(bcast, p2p1)
	p2.Round2(bcast, p2p2)
	fmt.Printf("\nSkShare P1: %x\n", p1.SkShare.Bytes())
	fmt.Printf("SkShare P2: %x\n", p2.SkShare.Bytes())
	fmt.Printf("\nVerification key P1: %x\n", p1.VerificationKey.ToAffineCompressed())
	fmt.Printf("Verification key P2: %x\n", p2.VerificationKey.ToAffineCompressed())

	fmt.Printf("\n=== Round 3 split those secret keys and rebuild verification key ===\n")

	s, _ := sharing.NewShamir(2, 3, myCurve)
	sk, _ := s.Combine(&sharing.ShamirShare{Id: p1.Id, Value: p1.SkShare.Bytes()},
		&sharing.ShamirShare{Id: p2.Id, Value: p2.SkShare.Bytes()})

	vk := myCurve.ScalarBaseMult(sk)
	rtn := vk.Equal(p1.VerificationKey)

	if rtn {
		fmt.Printf("Verification keys are the same.\n")
		fmt.Printf("Verification key Round 2: %x\n", vk.ToAffineCompressed())
	}
}

\end{lstlisting}
A sample run is:
\begin{lstlisting}[language=golang]
=== Round 1 let's generate secret keys ===

=== Round 2 let's generate the verification key ===

SkShare P1: ce265892e28d85248a2b84e5d0f8d8cb1d913ff2b56c2bb10abf773db5d71806
SkShare P2: edf456335be5535a58cb20ac91ef953890d8fab07e1adac48a273a4ecc96470d

Verification key P1: 041a152cb05f02ebb1573bae9d1ff9d0909f787f05c5a825d8560ce6d9f463db
Verification key P2: 041a152cb05f02ebb1573bae9d1ff9d0909f787f05c5a825d8560ce6d9f463db

=== Round 3 split those secret keys and rebuild verification key ===
Verification keys are the same.
Verification key Round 2: 041a152cb05f02ebb1573bae9d1ff9d0909f787f05c5a825d8560ce6d9f463db
\end{lstlisting}

The running code is \href{https://asecuritysite.com/kryptology/dkg}{here}.

\subsection{Paillier}
The Paillier cryptosystem supports homomorphic encryption, where two encrypted values can be added or one value casn be scalar multiplied, and the decryption of the result gives the result. In this case we will use 1,024 bit prime numbers for $p$ and $q$ and thus produce a modulus with 2,048 bits ($n=pq$).

First we select two large prime numbers ($p$ and $q$) and compute:
\begin{equation*}
n=pq
PHI=(p-1)(q-1)
\end{equation*}

$ \lambda =\operatorname {lcm} {(p-1,q-1)} $
and where lcm is the least common multiple. We then select random integer $g$ for:
$ \displaystyle g \in \mathbb {Z} _{n^{2}}^{*} $
We must make sure that $n$ divides the order of $g$ by checking the following: 
$ \mu =(L(g^{\lambda }{\bmod {n}}^{2}))^{-1}{\bmod {n}}$

and where $L$ is defined as $L(x)=\frac {x-1}{n}$. The public key is $(n ,g)$ and the private key is $(\lambda ,\mu )$.
To encrypt a message ($M$), we select a random $r$ value and compute the ciphertext of:

$c=g^{m}\cdot r^{n} \pmod {n^{2}}$

and then to decrypt:

\begin{equation*}
m=L(c^{\lambda }{\bmod n}^{2})\cdot \mu {\pmod n} 
\end{equation*}

\subsubsection{Adding and scalar multiply}

If we take two ciphers ($C_1$ and $C_2$), we get:
$C_1 = g^{m_1}\cdot r_1^{n} \pmod {n^{2}} $
$C_2 = g^{m_2}\cdot r_2^{n} \pmod {n^{2}} $
If we now multiply them we get:
$C_1 \cdot C_2 = g^{m_1}\cdot r_1^{n} \cdot g^{m_2}\cdot r_2^{n} \pmod {n^{2}}$
$C_1 \cdot C_2 = g^{m_1+m_2}\cdot r_1^{n} \cdot r_2^{n} \pmod {n^{2}}$
And we adding two values requires a multiplication of the ciphers.

The outline coding using the library from the Kryptology library. We have manually added the public and secret key, but in real-life we would generate with:
\begin{lstlisting}[language=golang]
pub, sec, _ := paillier.NewKeys()
\end{lstlisting}
The code is:
\begin{lstlisting}[language=golang]
package main

import (
	"fmt"
	"math/big"
	"os"

	"github.com/coinbase/kryptology/pkg/paillier"
)

func main() {

	var sec paillier.SecretKey
	var pub paillier.PublicKey

	//	pub, sec, _ := paillier.NewKeys()

	pub.N, _ = new(big.Int).SetString("22203902867524505059996239340306362808852805402888214954381553003002718752808306965243974655390219346481612755387890570991182385566928749760445875916800573782909761881261515602762049819293013811136510263722491329215251675663091154175860620927146517652389408089110716148633480085801107700968384078929774277970426932561081560231010426294975678729992804063220974701278229766883426991469078323539488917623430196595127834729964807458110080684240115196595760172158113810254192728271785178985307185853395355962836026777351498860874006114137632167254987479651229489157192247478252351962954320801263428208801271515398015887801", 10)
	pub.N2 = new(big.Int).Mul(pub.N, pub.N)

	sec.N = pub.N
	sec.N2 = pub.N2
	sec.Lambda, _ = new(big.Int).SetString("11101951433762252529998119670153181404426402701444107477190776501501359376404153482621987327695109673240806377693945285495591192783464374880222937958400286891454880940630757801381024909646506905568255131861245664607625837831545577087930310463573258826194704044555358074316740042900553850484192039464887138985064438949068643503538028104882092520753872226183177268421975002892541203962036580811698912148170624870917841537346985483337432253649017635885024033744586145456966646545432316660152135614842196027111652507352356170725302821683928442675667004336523805058723372589095589316741830468728743532156406225121890756346", 10)
	sec.Totient, _ = new(big.Int).SetString("22203902867524505059996239340306362808852805402888214954381553003002718752808306965243974655390219346481612755387890570991182385566928749760445875916800573782909761881261515602762049819293013811136510263722491329215251675663091154175860620927146517652389408089110716148633480085801107700968384078929774277970128877898137287007076056209764185041507744452366354536843950005785082407924073161623397824296341249741835683074693970966674864507298035271770048067489172290913933293090864633320304271229684392054223305014704712341450605643367856885351334008673047610117446745178191178633483660937457487064312812450243781512692", 10)
	sec.U, _ = new(big.Int).SetString("11108720355657041776647490476262423100273444107890028034525926371450220865341816894255404548947647952186614924131107824022774134150177636593890919577479093776330856863330832621779073688637362125712752218152358601679371477743308049274665882845748928958872854339383876978533793119837835146167726752137945969833510158025058440018805812646143848801020667307117190186323497007267362203459968413761903710129427082211518450427328378521338965975284389455704146581178957343955351641425309976491396722227064973929033480821132777267246266490713852090985090755453080857556125803448778856380844874040092451545474091429770838805", 10)
	//	fmt.Printf("Pub N: %v\n", pub.N)
	//	fmt.Printf("Pub N2: %v\n", pub.N2)
	//	fmt.Printf("Sec: Lambda: %v\n", sec.Lambda)
	//	fmt.Printf("Sec: Totient: %v\n", sec.Totient)
	//	fmt.Printf("U: %v\n", sec.U)

	v1 := "111"
	v2 := "123"
	argCount := len(os.Args[1:])

	if argCount > 0 {
		v1 = os.Args[1]
	}
	if argCount > 1 {
		v2 = os.Args[2]
	}

	val1, _ := new(big.Int).SetString(v1, 10)
	val2, _ := new(big.Int).SetString(v2, 10)

	cipher1, c1, _ := pub.Encrypt(val1)

	cipher2, c2, _ := pub.Encrypt(val2)

	cipher3, _ := pub.Add(cipher1, cipher2)
	cipher4, _ := pub.Mul(val1, cipher2)

	decrypted1, _ := sec.Decrypt(cipher3)
	decrypted2, _ := sec.Decrypt(cipher4)

	fmt.Printf("\na=%s, b=%s\n", val1, val2)

	fmt.Printf("\nEnc(a)=%v, Enc(b)=%v\n", c1, c2)

	fmt.Printf("%s + %s = %s\n", val1, val2, decrypted1)
	fmt.Printf("%s * %s = %s\n", val1, val2, decrypted2)

}


\end{lstlisting}
A sample run is:
\begin{lstlisting}[language=golang]
a=99, b=101

Enc(a)=3194871588628358748966290700084048039504351559895566068649699226686196823202719691848442538154334259086870718517154309238960535353238124681826437650609974756182111331187136550288888243913621355453394195988893907331662212619099956597214048344379155251813838360379613014234504733115070813852665958338054399570730908960729062476752496268730534679455242536966348295264398620170743424134258798655234402342376007577814664497900979829030250365742441838215291615628708192832598514895136556284052555200143916946043349922329083954234944551751946938497382693177826236713968527218819113690486875483513214352456619925368986523829, Enc(b)=13589527499232325752634778817851281121651040055415530301574438693923234689704613260352777781803577016195096649735936270615387802707921560074089079322940073435224175548073476004757540792879509712875530692314042199000397816797600039616264877447516437328780537103533071545942061490755982844224226236302168781174648600938374827556758739664948513788576346004713439291103166197919603791687898854044026637077370502518171971262488604799791153729247987748432317839412374043015668538315916284242023004655533679040068212527422566840965831377168708156964822692509744524741001528815590877128498757010895632375885634162380520158219
99 + 101 = 200
99 * 101 = 9999

\end{lstlisting}

The running code is \href{https://asecuritysite.com/kryptology/pail01}{here}.

\subsubsection{Paillier Subtraction}
 The Paillier cryptosystem supports homomorphic encryption, where two encrypted values can be added, subtracted and scalar multiplied and the decryption of the result gives the result. In this case we will use 1,024 bit prime numbers for $p$ and $q$ and thus produce a modulus with 2,048 bits ($n=pq$).
 
First we select two large prime numbers ($p$ and $q$) and compute:
\begin{equation*}
n=pq
PHI=(p-1)(q-1)
\end{equation*}

$ \lambda =\operatorname {lcm} {(p-1,q-1)} $
and where lcm is the least common multiple. We then select random integer $g$ for:
$ \displaystyle g \in \mathbb {Z} _{n^{2}}^{*} $
We must make sure that $n$ divides the order of $g$ by checking the following: 
$ \mu =(L(g^{\lambda }{\bmod {n}}^{2}))^{-1}{\bmod {n}}$

and where $L$ is defined as $L(x)=\frac {x-1}{n}$. The public key is $(n ,g)$ and the private key is $(\lambda ,\mu )$.
To encrypt a message ($M$), we select a random $r$ value and compute the ciphertext of:
\begin{equation*}
c=g^{m}\cdot r^{n} \pmod {n^{2}}
\end{equation*}
and then to decrypt:
\begin{equation*}
m=L(c^{\lambda }{\bmod n}^{2})\cdot \mu {\pmod n} 
\end{equation*}
\subsubsection{Adding and scalar multiply}
If we take two ciphers ($C_1$ and $C_2$), we get:
\begin{equation*}
C_1 = g^{m_1}\cdot r_1^{n} \pmod {n^{2}} 
C_2 = g^{m_2}\cdot r_2^{n} \pmod {n^{2}} 
\end{equation*}

If we now multiply them we get:
\begin{equation*}
C_1 \cdot C_2 = g^{m_1}\cdot r_1^{n} \cdot g^{m_2}\cdot r_2^{n} \pmod {n^{2}}
C_1 \cdot C_2 = g^{m_1+m_2}\cdot r_1^{n} \cdot r_2^{n} \pmod {n^{2}}
\end{equation*}

And we adding two values requires a multiplication of the ciphers.
\subsubsection{Subtract}
If we take two ciphers ($C_1$ and $C_2$), we get:
$C_1 = g^{m_1}\cdot r_1^{n} \pmod {n^{2}} $
$C_2 = g^{m_2}\cdot r_2^{n} \pmod {n^{2}} $

If we now divide them we get:
\begin{equation*}
\frac{C_1}  {C_2} = \frac{ g^{m_1}\cdot r_1^{n}}{g^{m_2}\cdot r_2^{n}} \pmod {n^{2}}   
\frac{C_1}  {C_2} =  g^{m_1-m_2} \frac{r_1^{n}}{r_2^{n}} \pmod {n^{2}}  
\end{equation*}

And thus a subtraction is equivalent to a divide operation. For this we perform a modular divide operation.
\begin{lstlisting}[language=golang]
inv_cipher2, _ := crypto.Inv(cipher2, pub.N2)
\end{lstlisting}
and which is:
$C_2^{-1} = \textrm{InverseMod}(C_2,n^2)$
What we also need to do, is perform this operation when the result is greater than a given threshold:
$m = m - n$
<h2>Code</h2>
The basic data structures for the secret key, public key and ciphertext is:
\begin{lstlisting}[language=golang]
type (
	PublicKey struct {
		N  *big.Int
		N2 *big.Int
	}

	SecretKey struct {
		PublicKey
		Lambda  *big.Int
		Totient *big.Int
		U       *big.Int
	}
	Ciphertext *big.Int
)
\end{lstlisting}
The adding of ciphertext values is achieved through a multiplication of our big integer ciphertext values $c=a \cdot b \pmod {n^2}$:
\begin{lstlisting}[language=golang]
func add(pk PublicKey, a Ciphertext, b Ciphertext) Ciphertext {

	c := new(big.Int).Mul(a, b)
	return (new(big.Int).Mod(c, pk.N2))

}
\end{lstlisting}
When we multiply two Paillier ciphertext's, we actually use an exponenent function, and where $Enc(a)^k  -> Enc(k.a) \mod n$  
\begin{lstlisting}[language=golang]
func mul(a, c, m *big.Int) *big.Int {

	z := new(big.Int).Exp(c, a, m)
	return (z)
}
\end{lstlisting}
When we need to multiply two big integers we do it using a mod operator:
\begin{lstlisting}[language=golang]
func Mul(x, y, m *big.Int) *big.Int {

	z := new(big.Int).Mul(x, y)

	return z.Mod(z, m)
}
\end{lstlisting}
The inverse mod is used in the subtraction operation, and is implemented as:
\begin{lstlisting}[language=golang]
func Inv(x, m *big.Int) *big.Int {

	z := new(big.Int).ModInverse(x, m)
	return (z)
}
\end{lstlisting}


To encrypt the values, we create a random nonce ($r$) and then compute: 
$ \mu =(L(g^{\lambda }{\bmod {n}}^{2}))^{-1}{\bmod {n}}$

and where $L$ is defined as $L(x)=\frac {x-1}{n}$. The public key is $(n ,g)$ and the private key is $(\lambda ,\mu )$.
To encrypt a message ($M$), we select a random $r$ value and compute the ciphertext of:
$c=g^{m}\cdot r^{n} \pmod {n^{2}}$
This is implemented as:
\begin{lstlisting}[language=golang]
func encrypt(pk PublicKey, msg *big.Int) *big.Int {

	r, _ := core.Rand(pk.N)

	a := new(big.Int).Add(pk.N, core.One)
	a.Exp(a, msg, pk.N2)
	b := new(big.Int).Exp(r, pk.N, pk.N2) // b = r^N (mod N^2)

	// ciphertext = a*b = (N+1)^m * r^N  (mod N^2)
	c := Mul(a, b, pk.N2)

	return c
}
func L(n, x *big.Int) *big.Int {
	// (x - 1) / n
	b := new(big.Int).Sub(x, big.NewInt(1))
	return b.Div(b, n)
}
\end{lstlisting}
To decrypt:


\begin{lstlisting}[language=golang]
func decrypt(sk SecretKey, c *big.Int) *big.Int {

	// a = c^{lambda(N)}		mod N^2
	a := new(big.Int).Exp(c, sk.Lambda, sk.N2)

	// l = L(a, N)
	ell := L(sk.N, a)

	// m = lu = L(a)*u = L(c^{lambda(N)})*u	mod N
	m := Mul(ell, sk.U, sk.N)

	return m
}
\end{lstlisting}


<h2>Coding</h2>

The outline coding using the library from the Kryptology library. We have manually added the public and secret key, but in real-life we would generate with:
\begin{lstlisting}[language=golang]
pub, sec, _ := paillier.NewKeys()
\end{lstlisting}
The code is:
\begin{lstlisting}[language=golang]
package main

import (
	"fmt"
	"math/big"
	"os"

	"github.com/coinbase/kryptology/pkg/core"
)

type (
	PublicKey struct {
		N  *big.Int
		N2 *big.Int
	}

	SecretKey struct {
		PublicKey
		Lambda  *big.Int
		Totient *big.Int
		U       *big.Int
	}
	Ciphertext *big.Int
)

func add(pk PublicKey, a Ciphertext, b Ciphertext) Ciphertext {

	c := new(big.Int).Mul(a, b)
	return (new(big.Int).Mod(c, pk.N2))

}
func encrypt(pk PublicKey, msg *big.Int) *big.Int {

	r, _ := core.Rand(pk.N)

	a := new(big.Int).Add(pk.N, core.One)
	a.Exp(a, msg, pk.N2)
	b := new(big.Int).Exp(r, pk.N, pk.N2) // b = r^N (mod N^2)

	// ciphertext = a*b = (N+1)^m * r^N  (mod N^2)
	c := Mul(a, b, pk.N2)

	return c
}
func L(n, x *big.Int) *big.Int {
	// (x - 1) / n
	b := new(big.Int).Sub(x, big.NewInt(1))
	return b.Div(b, n)
}

func decrypt(sk SecretKey, c *big.Int) *big.Int {

	// a = c^{lambda(N)}		mod N^2
	a := new(big.Int).Exp(c, sk.Lambda, sk.N2)

	// l = L(a, N)
	ell := L(sk.N, a)

	// m = lu = L(a)*u = L(c^{lambda(N)})*u	mod N
	m := Mul(ell, sk.U, sk.N)

	return m
}

func Mul(x, y, m *big.Int) *big.Int {

	z := new(big.Int).Mul(x, y)

	return z.Mod(z, m)
}
func Inv(x, m *big.Int) *big.Int {

	z := new(big.Int).ModInverse(x, m)
	return (z)
}
func mul(a, c, m *big.Int) *big.Int {

	z := new(big.Int).Exp(c, a, m)
	return (z)
}
func setupKeys(sec *SecretKey, pub *PublicKey) {
	pub.N, _ = new(big.Int).SetString("22203902867524505059996239340306362808852805402888214954381553003002718752808306965243974655390219346481612755387890570991182385566928749760445875916800573782909761881261515602762049819293013811136510263722491329215251675663091154175860620927146517652389408089110716148633480085801107700968384078929774277970426932561081560231010426294975678729992804063220974701278229766883426991469078323539488917623430196595127834729964807458110080684240115196595760172158113810254192728271785178985307185853395355962836026777351498860874006114137632167254987479651229489157192247478252351962954320801263428208801271515398015887801", 10)
	pub.N2 = new(big.Int).Mul(pub.N, pub.N)

	sec.N = pub.N
	sec.N2 = pub.N2
	sec.Lambda, _ = new(big.Int).SetString("11101951433762252529998119670153181404426402701444107477190776501501359376404153482621987327695109673240806377693945285495591192783464374880222937958400286891454880940630757801381024909646506905568255131861245664607625837831545577087930310463573258826194704044555358074316740042900553850484192039464887138985064438949068643503538028104882092520753872226183177268421975002892541203962036580811698912148170624870917841537346985483337432253649017635885024033744586145456966646545432316660152135614842196027111652507352356170725302821683928442675667004336523805058723372589095589316741830468728743532156406225121890756346", 10)
	sec.Totient, _ = new(big.Int).SetString("22203902867524505059996239340306362808852805402888214954381553003002718752808306965243974655390219346481612755387890570991182385566928749760445875916800573782909761881261515602762049819293013811136510263722491329215251675663091154175860620927146517652389408089110716148633480085801107700968384078929774277970128877898137287007076056209764185041507744452366354536843950005785082407924073161623397824296341249741835683074693970966674864507298035271770048067489172290913933293090864633320304271229684392054223305014704712341450605643367856885351334008673047610117446745178191178633483660937457487064312812450243781512692", 10)
	sec.U, _ = new(big.Int).SetString("11108720355657041776647490476262423100273444107890028034525926371450220865341816894255404548947647952186614924131107824022774134150177636593890919577479093776330856863330832621779073688637362125712752218152358601679371477743308049274665882845748928958872854339383876978533793119837835146167726752137945969833510158025058440018805812646143848801020667307117190186323497007267362203459968413761903710129427082211518450427328378521338965975284389455704146581178957343955351641425309976491396722227064973929033480821132777267246266490713852090985090755453080857556125803448778856380844874040092451545474091429770838805", 10)

}
func main() {

	var sec SecretKey
	var pub PublicKey

	//	pub, sec, _ := paillier.NewKeys()
	setupKeys(&sec, &pub)

	v1 := "223"
	v2 := "224"
	argCount := len(os.Args[1:])

	if argCount > 0 {
		v1 = os.Args[1]
	}
	if argCount > 1 {
		v2 = os.Args[2]
	}

	val1, _ := new(big.Int).SetString(v1, 10)
	val2, _ := new(big.Int).SetString(v2, 10)

	cipher1 := encrypt(pub, val1)

	cipher2 := encrypt(pub, val2)

	// Adding
	cipher3 := add(pub, cipher1, cipher2)

	decrypted1 := decrypt(sec, cipher3)

	// Subtraction
	inv_cipher2 := Inv(cipher2, pub.N2)

	cipher4 := add(pub, cipher1, inv_cipher2)

	decrypted2 := decrypt(sec, cipher4)

	// Multiply
	cipher5 := mul(val1, cipher2, pub.N2)

	decrypted3 := decrypt(sec, cipher5)

	fmt.Printf("\na=%s, b=%s\n", val1, val2)

	fmt.Printf("\nEnc(a)=%v, Enc(b)=%v\n", cipher1, cipher2)

	fmt.Printf("\n%s + %s = %s\n", val1, val2, decrypted1)
	fmt.Printf("\n%s * %s = %s\n", val1, val2, decrypted3)

	if decrypted2.Cmp(new(big.Int).Div(pub.N, big.NewInt(2))) > 0 {
		// m = m - n
		fmt.Printf("%s - %s = %s\n", val1, val2, new(big.Int).Sub(decrypted2, pub.N))
	} else {
		fmt.Printf("%s - %s = %s\n", val1, val2, decrypted2)
	}

}



\end{lstlisting}
A sample run is:
\begin{lstlisting}[language=golang]
a=222, b=111

Enc(a)=480255181920800962319428195982635686810088385894694335732539232950598802361655578994299473947015823706085641632265918920177271050935899445772018657379409917340875585795573456622928011108763896998310685496049348635361148476665982292583742521662892246510134496910480985230953608457374596556061690681311372035369557473453948571498287540563940498719457037028423196712497593060402292462158152772365096268526544613966053669489002176306136618535389523393860906046429497082997574262450762786531668654114069457095304276136300381237935928488169886100022455673772985830484439920173220489954345908504730126607166660669616837735331132127595030555268828556190724381620586303349525363142824926041003132666363188063124075469384544768925327914082583686275806308821004655253016048332888033533857446684327464728753575758198032289396001937677420421304213675660776816637709884428865855227219223951888611467829806312828381700124791746116297756951418091223465584531827315766709832802225806892686198418948109322860207792492578901690557854559299736849385819889486069503912193322571436752435739403077721769655830857694261861731325926243758449255964430155072325622086559490250784450951299715352393589113643733050357885271539548238790965835016548892755681491217, Enc(b)=398205057005000805455412925833532994717615194020655376461633849479054914228469584412356182413073212222229225897995778310285802001620224215672510848280476816560246933598044438129822536195476471730535502177390452652250248208595245774868663210615963412562038409604119717517734532923327183494024965696228498538639558086901827119637452112502647978827481995866363495625837621647623546620410500086811780489366824575093690909960314240825269897595801111438023076383121529088191656996666295497574395828609506976835480393272407009883660101408839186236877371208967820363921744294119034984338166756418022949781351180172422781584254651807677632253283134440525408418041260953938375203226980802190306068235344987804712672397597944426532987481662630428128948672757884566423914969203583167323575075335034411157347418887682930435526342638719818198078786738032388166189020743344542420574023931557754426969505264962187883070184429059626960626546411313341199020568060067512561944206262699174908858448584688032887324374515251373912574173526824962194722293602736606882903604170107467326730803713106312324982828292317687693528819441737056014833346488071437353342607272253728630007825092500186949850603988095382717600780136544280866381494593592289423116839401

222 + 111 = 333

222 * 111 = 24642
222 - 111 = 111

\end{lstlisting}

The running code is \href{https://asecuritysite.com/kryptology/pail03}{here}.


\subsection{Encrypted searching}
With pair-based cryptography we have two cyclic groups ($G_1$ and $G_2$), and which are of an order of a prime number ($n$). A pairing on $(G_1,G_2,G_T)$ defines the function $e:G_1 \times G_2 \rightarrow G_T$, and where $g_1$ is a generator for $G_1$ and $g_2$ is a generator for $G_2$. If $U$ is a point on $G_1$, and $V$ is a point on $G_2$, we have following rules:

\begin{equation*}
\hat{e}(aU,bV) = \hat{e}(U,V)^{ab} = \hat{e}(abU, V) = \hat{e}(U, abV ) = \hat{e}(bU,aV)
\end{equation*}

In this case we will encrypt a string, and then use crypto pairing to search for it. It uses the Kryptology library.
                

With crypto pairing we have two elliptic curves: G1 and G2, and then map onto a third curve: Gt. The pairing of the points on G1 (P) and G2 (Q) is defined as a pairing function, and where we determine $\hat{e}(Q,P)$. For the points of $P$ and $Q$, this has special mappings of: 

\begin{equation*}
\hat{e}(sQ,rP) = \hat{e}(rQ,sP) = \hat{e}(rsQ,P) = \hat{e}(Q,rsP) =  \hat{e}(sQ,P)^r =  \hat{e}(Q,P)^{rs} 
\end{equation*}

and:
\begin{equation*}
\hat{e}(R+Q,P) = \hat{e}(R,P) \times  \hat{e}(Q,P)  
\end{equation*}

First we have two curves ($G_1$ and $G_2$) and initially we define a large prime number ($q$). First Alice - who wants to search - selects a point on the $G_2$ curve ($P$), and generates a using a random number ($s$):
\begin{equation*}
sk=s
\end{equation*}
Alice then creates public key with:
\begin{equation*}
P_{s}=sP
\end{equation*}

Next Bob creates a random value ($r$) and creates:
\begin{equation*}
P_{r}=rP
\end{equation*}

Bob then hashes the word to search ($m$) to the G2 curve:
\begin{equation*}
Q_W=H_1(m)
\end{equation*}
Bob takes Alice's public key ($P_s$) and his private key ($r$) and creates the pairing of:
\begin{equation*}
\hat{e}{(Q_W,P_{s})}^r
\end{equation*}

If Alice wants to search for $W_2$, she matches to:
\begin{equation*}
\hat{e}(T_w,P_r)
\end{equation*}
and where $T_w=s H_1(W_2))$

This works because:
\begin{equation*}
\hat{e}(T_w,P_r) = \hat{e}(s H_1(W_2),rP) = \hat{e}(r H_1(W_2),sP)  = \hat{e}(Q_W,sP)^r =  \hat{e}(Q_W,P_s)^r
\end{equation*}

\begin{figure}
\begin{center}
\includegraphics[width=1.0\linewidth]{figures/pair11.png}
\caption{Example quadratic equation)}
\label{fig:pair}
\end{center}
\end{figure}

The outline coding using the library from the Kryptology library is
\begin{lstlisting}[language=golang]
package main

import (
	"crypto/rand"
	"fmt"
	"math/big"
	"os"

	"crypto/sha256"

	bls12381 "github.com/coinbase/kryptology/pkg/core/curves/native/bls12-381"
)

func main() {

	m := "hello"
	tof := "hello"

	argCount := len(os.Args[1:])

	if argCount > 0 {
		m = os.Args[1]
	}
	if argCount > 1 {
		tof = os.Args[2]
	}

	fmt.Printf("Encrypted word: %s\n\n", m)
	fmt.Printf("Word to find: %s\n\n", tof)

	bls := bls12381.NewEngine()
	g1, g2 := bls.G1, bls.G2
	gt := bls.GT()

	msg := []byte(m)
	tofind := []byte(tof)

	HW, _ := g1.HashToCurve(sha256.New, msg, []byte(""))
	ToF, _ := g1.HashToCurve(sha256.New, tofind, []byte(""))

	r := make([]byte, 32)
	rand.Read(r)
	rval := new(big.Int).SetBytes(r)

	s := make([]byte, 32)
	rand.Read(s)
	sval := new(big.Int).SetBytes(s)

	G2 := g2.One()
	sP := g2.New()
	rP := g2.New()

	sToF := g1.New()

	g2.MulScalar(sP, G2, sval)
	g2.MulScalar(rP, G2, rval)

	g1.MulScalar(sToF, ToF, sval)

	fmt.Printf("s = %x\n", s)
	fmt.Printf("r = %x\n\n", r)

	e0, _ := bls.AddPair(HW, sP).Result()
	gt.Exp(e0, e0, rval)

	e1, _ := bls.AddPair(sToF, rP).Result()

	fmt.Printf("First part of e0 pairing: %+v\n", e0[0][0][0])
	fmt.Printf("First part of e1 pairing: %+v\n", e1[0][0][0])

	if e0.Equal(e1) {
		fmt.Printf("We have found it...")
	} else {
		fmt.Printf("Cannot find!")
	}

}


\end{lstlisting}
A sample run is:
\begin{lstlisting}[language=golang]
Encrypted word: Hello

Word to find: Hello

s = 1229b2836a548cca3bc9ac238cd0c634635535f3a5b6f12aac78fd5fa096a77c
r = 2fce640d56121d278b20dedd00ecc442e3a1c536de98209f4f10f551b15072e9

First part of e0 pairing: [5509936851070022305 4957573568693525133 3532086020062769437 5031641048332977130 18248703594105518599 657243605775503017]
First part of e1 pairing: [5509936851070022305 4957573568693525133 3532086020062769437 5031641048332977130 18248703594105518599 657243605775503017]
We have found it...

\end{lstlisting}
and a false search:
\begin{lstlisting}[language=golang]
Encrypted word: Hello

Word to find: Hello123

s = 3398a4ecba24cc114291082613ed0f49a5e482ee72d829cdd33fefd404f91ca6
r = cf2c6448553df07deb10b4e70dd0e2e113a4d3318d87d1c08d735528f9754dde

First part of e0 pairing: [9433419437807457542 14827067878769968193 9757426493516444139 5593213596321565194 10129867375955106600 81638192315469051]
First part of e1 pairing: [9963009439914925460 13665328121908137426 1398638186177370014 5695327681334410247 16635414863332113065 1808470817875180072]
Cannot find!
\end{lstlisting}

The running code is \href{https://asecuritysite.com/kryptology/enc}{here}.

\section{Asynchronous Verifiable Secret Sharing}
 In 2002, Cachin et. al defined Asynchronous Verifiable Secret Sharing (AVSS) method and which uses bi-variate polynomials \cite{cachin2002asynchronous}\cite{cachin2005asynchronous}. In most secret sharing schemes we have a polynomial with one variable, such as $p(x)=a_0+a_1x+a_2x^2+...$. With Shamir's Secret Shares we store the secret share at $a_0$, and where we distribute points on the polynomial, and then rebuild them back into a polynomial, and which should then reveal the secret. With AVSS we use bi-variate polynomials and which has two variables ($x$ and $y$). Bi-variate polynomials are in the form of $f(x,y)  =a_{00} + a_{10}x + a_{01} y + a_{11} xy +  a_{21} x^2y + +  a_{12} xy^2 + a_{22} x^2y^2 + ... $. In this case, the secret is kept at $a_{00}$. With the Shamir method, we define a threshold ($t$) from a number of shares ($n$), and then aim to recover a polynomial $f(x,y$) and where the secret share is at $f(0,0$).
 
Within secret sharing models we can have three main categories:

\begin{itemize}
\item Synchronous model. This is implemented in systems that use a global clock to synchonise messages, and where there will be well-defined delays in processing. 
\item Asynchronous model. This is where there is no synchonisation of messages, and where delays can vary depending on workloads. One of the key issues is that it is difficult to differentiate a slow response from a participating party from a corrupt sender who refuses to send back messages. This leads to more complexity in the methods used by asynchonous methods. 
\item Hybrid. This is a mixture of synchonous and asynchronous models, and where there may be a few rounds of synchonization followed by asynchonous operations.
\end{itemize}

In a typical secret sharing method, the dealer defines a polynomial of $p(x)=a_0+a_1x+a_2x^2+...$ and where $a_0$ defines the secret. The dealer then sends out points on the polynomial, such for $x=1$ and where we have the $y$ value of $p(x=1)$. We can also create a commitment from the dealer, so that each participant can check that their share is valid. Within an asynchonous environment, the dealer may not wait around before all the shares have been acknowledged. AVSS supports a participating party to reconstruct its share using a distributed protocol that does not require the dealer to be present. This requires $f+1$ participants.

In asynchronous settings in which if participants might fail, a dealer can wait for at most n f participants to acknowledge receiving a valid share, before it inevitably may walk away. The asynchronous VSS problem requires that if the dealer (or any participant) completes the sharing protocol, then every correct participant can eventually reconstruct its share using  a distributed protocol involving $f + 1$ participants.

In AVSS, we start with a bi-variate polynomial ($m \times n$):

\begin{equation*}
f(x,y)  = \sum_{k=0}^{n-1}\sum_{j=0}^{m-1} a_{jk}x^ky^j
    \end{equation*}

For $n=3$ and $m=3$, we have:

\begin{equation*}
f(x,y)  =a_{00} + a_{10}x + a_{01} y + a_{11} xy +  a_{21} x^2y + +  a_{12} xy^2 + a_{22} x^2y^2
    \end{equation*}
    
In a secret sharing system, we aim to find the solution at $p(0,0)$.
We can represent the factors in a matrix form of:


    \begin{equation*}
    v_{m,n} =
    \begin{pmatrix}
    a_{0,0} & a_{0,1} & \cdots & a_{0,n-1} \\
    a_{1,0} & a_{1,1} & \cdots & a_{1,n-1} \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    a_{m-1,1} & a_{m-1,1} & \cdots & a_{m-1,n-1}
    \end{pmatrix}
    \end{equation*}


In AVSS, we place the secret at $a_{0,0}$ and random values in the other positions: 


    \begin{equation*}
    f_{m,n} =
    \begin{pmatrix}
    s & r_{0,1} & \cdots & r_{0,n-1} \\
    r_{1,0} & r_{1,1} & \cdots & r_{1,n-1} \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    r_{m-1,1} & r_{m-1,1} & \cdots & r_{m-1,n-1}
    \end{pmatrix}
    \end{equation*}


We then generate a random matrix:


    \begin{equation*}
    f'_{m,n} =
    \begin{pmatrix}
    v_{0,0} & v_{0,1} & \cdots & v_{0,n-1} \\
    v_{1,0} & v_{1,1} & \cdots & v_{1,n-1} \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    v_{m-1,1} & v_{m-1,1} & \cdots & v_{m-1,n-1}
    \end{pmatrix}
    \end{equation*}


We then take a base point on the secp256k1 curve ($G$) and then scale with $f_(m,n)$, and then add this to $f'(m,n)$ to another base point ($H$). This then gives  gives a number of secp256k1 points for the commitments from the dealer:


    \begin{equation*}
    C_{m,n} =
    \begin{pmatrix}
    sG + r_{0,0}H & r_{0,1}G+ r_{0,1}H & \cdots & r_{0,n-1}G + r_{0,n-1}H \\
    r_{1,0}G + r_{1,0}H & r_{1,1}G + r_{1,1}H & \cdots & r_{1,n-1}G + r_{1,n-1}H \\
    \vdots  & \vdots  & \ddots & \vdots  \\
    r_{m-1,1}G + r_{m-1,1}H & r_{m-1,1}G + r_{m-1,1}H & \cdots & r_{m-1,n-1}G + r_{m-1,n-1}H
    \end{pmatrix}
    \end{equation*}

Each of the nodes $i$ then get:

\begin{itemize}
\item $C$
\item $a_i(y) = f(i,y)$
\item $a_i'(y) = f'(i,y)$
\item $b_i(x) = f(x,i)$
\item $b_i'(x) = f'(x,i)$
\end{itemize}


Thus Node 1 ($x=1$) gets the polynomial factors of:
 \begin{equation*}
a_1(y) = sG+ v_{0,0}H, r_{0,1}G + v_{0,1}H, \cdots r_{0,n-1}G + v_{0,n-1}H 
 \end{equation*}

Thus Node 2 ($x=2$) gets the polynomial factors of:

 \begin{equation*}
a_2(y) = sG+ v_{0,0}H, r_{0,1}G + v_{0,1}H \times 4,  \cdots  r_{0,n-1}G +  v_{0,n-1}H \times 2^{n-1}
 \end{equation*}

Thus Node 3 ($x=3$) gets the polynomial factors of:

 \begin{equation*}
a_3(y) = sG+ v_{0,0}H, r_{0,1}G + v_{0,1}H \times 9,  \cdots  r_{0,n-1}G + v_{0,n-1}H \times 3^{n-1}
 \end{equation*}

Every node $i$ will receive $C$, the share polynomial of $a_i(y)$ and $a_i'(y)$, and the sub-share polynomials are $b_i(y)$ and $b_i'(y)$ 
Each node can then check their shares against the commitment from the dealer. The sequence is then:

1. The Dealer creates a bi-variate polynomial and puts the secret at $f(0,0)$ and with random values at all the other other places in the matrix:
\begin{lstlisting}[language=golang]
	f := GenerateRandomBivariatePolynomial(secret, threshold)
\end{lstlisting}
2. Create random bitvariate polynomial:
\begin{lstlisting}[language=golang]
	fprime := GenerateRandomBivariatePolynomial(*RandomBigInt(), threshold)
\end{lstlisting}
3. Create commitment matrix, and which is the point assigns the $f$ as scalar values to the $G$ base point, and $fprime$ with the $H$ based point, and then adds these together, to get the form $a_{ij}G + a'_{ij}H$. 
\begin{lstlisting}[language=golang]
	C := GetCommitmentMatrix(f, fprime)
\end{lstlisting}
These are points on the secp256k1 curve. When a node receives a share, it can then check that the share is valid. In the following, we will take the first share for its validity:
\begin{lstlisting}[language=golang]
	sigma := polyEval(EvaluateBivarPolyAtX(f, *big.NewInt(int64(threshold))), 0)
	sigmaprime := polyEval(EvaluateBivarPolyAtX(fprime, *big.NewInt(int64(threshold))), 0)
	fmt.Printf("\n1st share: Sigma=%s, Sigma_p=%s", sigma, sigmaprime)
	rtn := AVSSVerifyShare(C, *big.NewInt(int64(threshold)), *sigma, *sigmaprime)
	fmt.Printf("\nVerified share: %v ", rtn)
\end{lstlisting}
<h2>Coding</h2>

The following code is based on the Tor.us source. In this case we will define $t$ for the threshold and $n$ for the number of shares:


\begin{lstlisting}[language=golang]
// Based on https://github.com/torusresearch/torus-node
package main

import (
	"crypto/rand"
	"fmt"
	"main/secp256k1"
	"math/big"
	"os"
	"strconv"
)

func RandomBigInt() *big.Int {
	randomInt, _ := rand.Int(rand.Reader, secp256k1.GeneratorOrder)
	return randomInt
}
func AVSSVerifyShare(C [][]secp256k1.Point, m big.Int, sigma big.Int, sigmaprime big.Int) bool {
	sG := secp256k1.BigIntToPoint(secp256k1.Curve.ScalarBaseMult(sigma.Bytes()))
	rH := secp256k1.BigIntToPoint(secp256k1.Curve.ScalarMult(&secp256k1.H.X, &secp256k1.H.Y, sigmaprime.Bytes()))
	sGrH := secp256k1.BigIntToPoint(secp256k1.Curve.Add(&sG.X, &sG.Y, &rH.X, &rH.Y))
	pt := secp256k1.Point{X: *big.NewInt(int64(0)), Y: *big.NewInt(int64(0))}
	for j := range C {
		Cj0 := C[j][0]
		mj := new(big.Int).Exp(&m, big.NewInt(int64(j)), secp256k1.GeneratorOrder)
		Cj0mj := secp256k1.BigIntToPoint(secp256k1.Curve.ScalarMult(&Cj0.X, &Cj0.Y, mj.Bytes()))
		pt = secp256k1.BigIntToPoint(secp256k1.Curve.Add(&pt.X, &pt.Y, &Cj0mj.X, &Cj0mj.Y))
	}

	if sGrH.X.Cmp(&pt.X) != 0 || sGrH.Y.Cmp(&pt.Y) != 0 {
		return false
	}

	return true
}

func GenerateRandomBivariatePolynomial(secret big.Int, threshold int) [][]big.Int {
	bivarPolyCoeffs := make([][]big.Int, threshold)
	for j := range bivarPolyCoeffs {
		bivarPolyCoeffs[j] = make([]big.Int, threshold)
		for l := range bivarPolyCoeffs[j] {
			if j == 0 && l == 0 {
				bivarPolyCoeffs[j][l] = secret
			} else {
				bivarPolyCoeffs[j][l] = *RandomBigInt()
			}
		}
	}

	return bivarPolyCoeffs
}

func GetCommitmentMatrix(f [][]big.Int, fprime [][]big.Int) [][]secp256k1.Point {
	threshold := len(f)
	bivarPolyCommits := make([][]secp256k1.Point, threshold)
	for j := range bivarPolyCommits {
		bivarPolyCommits[j] = make([]secp256k1.Point, threshold)
		for l := range bivarPolyCommits[j] {
			gfjl := secp256k1.BigIntToPoint(secp256k1.Curve.ScalarBaseMult(f[j][l].Bytes()))
			hfprimejl := secp256k1.BigIntToPoint(secp256k1.Curve.ScalarMult(
				&secp256k1.H.X,
				&secp256k1.H.Y,
				fprime[j][l].Bytes(),
			))
			bivarPolyCommits[j][l] = secp256k1.BigIntToPoint(secp256k1.Curve.Add(&gfjl.X, &gfjl.Y, &hfprimejl.X, &hfprimejl.Y))
		}
	}
	return bivarPolyCommits
}

type PrimaryPolynomial struct {
	Coeff     []big.Int
	Threshold int
}

func PolyEval(polynomial PrimaryPolynomial, x big.Int) *big.Int {
	return polyEval(polynomial, int(x.Int64()))
}

func polyEval(polynomial PrimaryPolynomial, x int) *big.Int { // get private share
	xi := big.NewInt(int64(x))
	sum := new(big.Int)

	sum.Add(sum, &polynomial.Coeff[0])

	for i := 1; i < polynomial.Threshold; i++ {
		tmp := new(big.Int).Mul(xi, &polynomial.Coeff[i])
		sum.Add(sum, tmp)
		sum.Mod(sum, secp256k1.GeneratorOrder)
		xi.Mul(xi, big.NewInt(int64(x)))
		xi.Mod(xi, secp256k1.GeneratorOrder)
	}
	return sum
}
func EvaluateBivarPolyAtX(bivarPoly [][]big.Int, index big.Int) PrimaryPolynomial {
	fiY := PrimaryPolynomial{
		Coeff:     make([]big.Int, len(bivarPoly)),
		Threshold: len(bivarPoly),
	}
	for l := range bivarPoly[0] { // loop through horizontally first
		for j := range bivarPoly { // loop through vertically
			fiY.Coeff[l] = *new(big.Int).Add(
				&fiY.Coeff[l],
				new(big.Int).Mul(
					&bivarPoly[j][l],
					new(big.Int).Exp(&index, big.NewInt(int64(j)), secp256k1.GeneratorOrder),
				),
			)
		}
	}
	return fiY
}
func EvaluateBivarPolyAtY(bivarPoly [][]big.Int, index big.Int) PrimaryPolynomial {
	fiX := PrimaryPolynomial{
		Coeff:     make([]big.Int, len(bivarPoly)),
		Threshold: len(bivarPoly),
	}
	for j := range bivarPoly { // loop through vertically first
		for l := range bivarPoly[j] { // loop through horizontally
			fiX.Coeff[j] = *new(big.Int).Add(
				&fiX.Coeff[j],
				new(big.Int).Mul(
					&bivarPoly[j][l],
					new(big.Int).Exp(&index, big.NewInt(int64(l)), secp256k1.GeneratorOrder),
				),
			)
		}
	}
	return fiX
}

func showMatrix(msg string, m [][]big.Int, size int) {
	fmt.Printf("%s\n", msg)
	for i := 0; i < size; i++ {
		fmt.Printf("Row: ")
		for j := 0; j < size; j++ {
			fmt.Printf("%s ", m[i][j].String())
		}
		fmt.Printf("\n")
	}
	fmt.Printf("\n")
}
func showPoints(msg string, m [][]secp256k1.Point, size int) {
	fmt.Printf("%s\n", msg)
	for i := 0; i < size; i++ {
		fmt.Printf("Row: ")
		for j := 0; j < size; j++ {
			fmt.Printf("%s ", m[i][j].X.String())
		}
		fmt.Printf("\n")
	}
	fmt.Printf("\n")
}
func main() {

	threshold := 3
	s := 5
	nodes := 5
	//	secret := *RandomBigInt()

	argCount := len(os.Args[1:])

	if argCount > 0 {
		s, _ = strconv.Atoi(os.Args[1])
	}
	if argCount > 1 {
		threshold, _ = strconv.Atoi(os.Args[2])

	}
	if argCount > 2 {
		nodes, _ = strconv.Atoi(os.Args[3])

	}

	secret := *big.NewInt(int64(s))

	fmt.Printf("Secret=%d, threshold=%d, nodes=%d\n", s, threshold, nodes)

	f := GenerateRandomBivariatePolynomial(secret, threshold)
	showMatrix("=== Show f (share at f(0,0))===", f, threshold)
	fprime := GenerateRandomBivariatePolynomial(*RandomBigInt(), threshold)
	showMatrix("=== Show f' ===", fprime, threshold)

	C := GetCommitmentMatrix(f, fprime)
	showPoints("=== Show Commitments (C - X points) ===", C, threshold)
	sigma := polyEval(EvaluateBivarPolyAtX(f, *big.NewInt(int64(threshold))), 0)
	sigmaprime := polyEval(EvaluateBivarPolyAtX(fprime, *big.NewInt(int64(threshold))), 0)
	fmt.Printf("\n1st share: Sigma=%s, Sigma_p=%s", sigma, sigmaprime)
	rtn := AVSSVerifyShare(C, *big.NewInt(int64(threshold)), *sigma, *sigmaprime)
	fmt.Printf("\nVerified share: %v ", rtn)

	/*
		for node := 0; node < nodes; node++ {
			i := *big.NewInt(int64(node + 1))
			AIY := EvaluateBivarPolyAtX(f, i)
			AIprimeY := EvaluateBivarPolyAtX(fprime, i)
			BIX := EvaluateBivarPolyAtY(f, i)
			BIprimeX := EvaluateBivarPolyAtY(fprime, i)
			fmt.Printf("AIY=%v, AIprimeY=%v, BIX=%v, BIPrimeX=%v\n", AIY.Coeff, AIprimeY.Coeff, BIX.Coeff, BIprimeX.Coeff)
		} */
}


\end{lstlisting}


A sample run:
\begin{lstlisting}[language=golang]
Secret=5, threshold=3, nodes=5
=== Show f (share at f(0,0))===
Row: 5 9743195669945784265736128598508718513383431809992852931467201572222501709532 11921601245529184890572677981314550793638440277120977934507285858736284872764 
Row: 38914775169750618295866116389646254021539712841774945361261041297120280450770 39728712398652269566024872460140072549594041362028713476440569412633907719597 93804328507791152440549289202239599104421824368912194876844146484734559224879 
Row: 29699601562624258681390881187189276130152510632542564550139048371246796426949 20177829835342526168771993908034295528249900168488246059089443608353861373117 50725914710115279957671906851075719555745896639024880177910113896553695516565 

=== Show f' ===
Row: 115470196996176989345349889981956268662981937404082398634901967695935968192584 33044579844575268229918544233776696118670553243354949460102752276645043035280 94715233694196754547344213678075119784007634903399571068809848072191720921783 
Row: 4340250202862599175210727375498478088765750740690216946430308017593134758098 36851108627021186689738145561635749516393072041227168049762415989053802072740 85484825408312771819133941960259191534837442943831567555553302176157039053809 
Row: 92533102775313911545179309541127851019948561944739879791724032538117151496081 65933151131078972969485082821058756347303210836121412732507767307017160267569 86168717839084739660292482381227107627026797065820199045141906676115087565692 

=== Show Commitments (C) ===
Row: 115470196996176989345349889981956268662981937404082398634901967695935968192584 33044579844575268229918544233776696118670553243354949460102752276645043035280 94715233694196754547344213678075119784007634903399571068809848072191720921783 
Row: 4340250202862599175210727375498478088765750740690216946430308017593134758098 36851108627021186689738145561635749516393072041227168049762415989053802072740 85484825408312771819133941960259191534837442943831567555553302176157039053809 
Row: 92533102775313911545179309541127851019948561944739879791724032538117151496081 65933151131078972969485082821058756347303210836121412732507767307017160267569 86168717839084739660292482381227107627026797065820199045141906676115087565692 


Sigma=36664471860921596749403324827578523677479041380983203887219069808027524711845, Sigma_p=34952158684060427389027977909099099286115732896212732538867879459624443976911
Verified share: true 
\end{lstlisting}

The running code is \href{https://asecuritysite.com/sharing/avss}{here}.


\section{ECDSA and EdDSA}
A digital signature involves taking a hash of the message, and then using a private key to create a signature. The public key is then used to prove the signature, and verify the contents of the message. The two main methods that are used as ECDSA (using the secp256k1 curve) and EdDSA (using the Curve 25519). An overview of these methods are:

\begin{itemize}
\item Ed25519 was proposed in 2011 by Daniel J. Bernstein, Niels Duif, Tanja Lange, Peter Schwabe, and Bo-Yin Yang \cite{bernstein2012high}, while ECDSA was proposed around 2001 by Don Johnson, Alfred Menezes, and Scott Vanstone \cite{johnson2001elliptic}.
\item ECDSA and EdDSA typically have equivalent performance and security levels.
\item ECDSA has a random nonce value created within the signature creation, whereas EdDSA does not. In ECDSA, we need to be careful in making sure that we do not reuse this nonce value, and that it is random.
\item EdDSA uses the Schnorr signature method, and which is now out of patent. It supports the aggregation of keys in the signature, and also the aggregation of the signature for multiple parties.
\item For improved security, ECDSA supports a 521-bit curve (P521), while EdDSA supports X448.
\item ECDSA signatures change each time based on the nonce used, whereas EdDSA signatures do not change for the same set of keys and the same message.
\item ECDSA is often used to keep compatibility with Bitcoin and Ethereum.
\item ECDSA public keys are (x,y) coordinates and thus have 512 bits (for secp256k1), while Ed25519 uses just the y co-ordinate value for the point, and thus has 256 bits.
\item It is possible to recover the public key from an ECDSA signature.
\end{itemize}


\subsection{ECDSA}
With ECDSA, Alice will sign a message with her private key, and then Bob will use her public key to verify that she signed the message (and that the message has now changed). Alice signs the message with the following:

\begin{itemize}
\item     Create a hash of the message $e=\textrm{HASH}(m)$.
\item     Let $h$ be the $L_{n}$ be the leftmost bits of $e$, $L_{n}$ has a  bit length of the group order $N$.
\item     Create a random number $k$ which is between 1 and $N-1$.
\item     Calculate a point on the curve as $(x_{1},y_{1})=k\times G$.
\item     Calculate $ r=x_{1} \pmod N $. If $r=0$, go back to Step 3.
\item     Calculate $s=k^{-1}(h+rd_{A}) \pmod N$. If $s=0$, go back to Step 3.
\item     The signature is the pair $(r,s)$.
\end{itemize}


Bob will check with:

\begin{itemize}
\item     Create a hash of the message $e=\textrm{HASH}(m)$.
\item     Let $h$ be the $L_{n}$ leftmost bits of $e$.
\item     Calculate $c=s^{-1} \pmod N$
\item     Calculate $u_{1}=h \cdot c \pmod N$ and $u_{2}=r \cdot c \pmod N$.
\item     Calculate the curve point ($x_{1},y_{1})=u_{1}\times G+u_{2}\times Q_{A}$. If $(x_{1},y_{1})=O$ then the signature is invalid.
\item     The signature is valid if $r\equiv x_{1}{\pmod {n}}$, invalid otherwise.
\end{itemize}

\begin{equation}
\begin{aligned}
(x_{1},y_{1}) &=u_{1}\times G+u_{2}\times Q_{A}\\ 
&= h \cdot c \cdot G + r \cdot c \cdot Q_A\\
&= c (hG + rQ_A) = \frac{hG + rQ_A} {k^{-1}(h+rd_A) } \\
&= \frac{hG + rd_A G} {k^{-1}(h+rd_A) } \\
&= \frac{(h + rd_A) G} {k^{-1}(h+rd_A) } =  kG 
\end{aligned}
\end{equation}

In the following we take a message, and generate a private key and then generate a public key and a message signature:

The running code is \href{https://asecuritysite.com/signatures/ecdsa_rs2}{here}.


The result is:

\begin{lstlisting}[language=golang]
=== Message ===
Msg=Hello 123
Hash=859e38d581e214dc7c8c871c425642913363a829065cf4acddd120ed5391b04b

=== Private key ===
Private key=a1edc17864ccc57f322c37565bd57c362d26b2834eca4e7a67bb3418a5559bce
Curve=P-256k1
Bit size=256
Base point (G) =(55066263022277343669578718895168534326250603453777594175500187360389116729240, 32670510020758816978083085130507043184471273380659243275938904335757337482424)
Prime=115792089237316195423570985008687907853269984665640564039457584007908834671663, Order=115792089237316195423570985008687907852837564279074904382605163141518161494337
=== Public key (X,Y) ===
X=110581895814688467324911896802326037643108110087623152868491197405382354846363 Y=4616276638173468737374384061170336228946320530451436648770152914318200031985
  Hex: X=f47b22911aed2191e9bffe2288b6a0c4eb9d64a04b96cdc87ff7bd170f4ec29b Y=0a34b850fef1c8913e8fca3275b2610b0b9e5dce7fb0942b377b46978d2a4af1

=== Signature (R,S) ===
R=63035590451686162315501508447714319652376408329503273191996886726405900868402 S=15428273428652997041233197909518826116574060127483623302249411101801664504930
 Hex: R=8b5ce13e27f4997276e4aa710f92e86f9dc394458f9884e56f0f6720f81e1b32 S=221c17e2f5e15dfbdabf3744582981da99242347905f7305db5381b5cec06462
Signature verifies
\end{lstlisting}

In this, we see that we have a 256-bit private key, and a public key which is a point on the secp256k1 curve. The output is two values: R and S. Once we use the message, the public key points, and the values of R and S, we should be able to determine the validity of the signature.

Now, we can test these values for x,y, r and s: here. If we now change the y value to be “38a21f573ed9ad9c8dd9107d8954d24b10357beee5b9df470f289be9a28b96a0”: , we now get an invalid signature: 

Reference: \href{https://asecuritysite.com/signatures/ecdsa_rs?msg0=Hello\%20123&r0=8d855e3135408528319c48b9e77bff82dfdf18bf9c65011df8725ab5823ae40c&s0=b5df557f90fd5697986806186497392d9bdf29fb6dc198775a381d900c399ee&x0=316c6d59567275de266aa82a30ba3e1cd408246a988b431f13d244e34bc2efc1&y0=38a21f573ed9ad9c8dd9107d8954d24b10357beee5b9df470f289be9a28b96a0}{here}.

\subsection{EdDSA}
The Edwards-curve Digital Signature Algorithm (EdDSA) is used to create a digital signature using an enhancement of the Schnorr signature with Twisted Edwards curves. Overall it is faster that many other digital signature methods, and is strong for security. One example of EdDSA is Ed25519, and which is based on Curve 25519. It generates a 64-byte signature value of (R,s), and has 32-byte values for the public and the private keys.

With Ed25519, Bob first generate a 256-bit random number for the private key ($priv$) and then create the public key with:

\begin{equation}
pub =  H(priv)[\colon 32] \cdot B
\end{equation}

and where $B$ is the base point on the curve, and and where $H()$ is a hash function (SHA-512). In this case we take the lower 32 bytes of the SHA-512 hash. Normally we just define this as the $y$ co-ordinate of the point. The public key is this 32 bytes long (256 bits). To compute the signature, we generate:

\begin{equation}
r = H_{int}( H(priv)[32\colon] \: || \: M) \pmod l
\end{equation}

and where $H_{int}()$ is a hash function (SHA-512) and converted to an integer value. In this case we take the upper 32 bytes for the calculation. Then $M$ is the byte value of the message. With "||" we append the bytes together. We then convert this to a point on the curve with:

\begin{equation}
R=r \cdot B
\end{equation}

Next, we compute:
\begin{equation}
h=H_{int}(R \: || \: pub \: || \: M) \pmod l
\end{equation}
and:
\begin{equation}
s=H_{int}(priv))[\colon 32]\\
S=(r+h \cdot s) \pmod l
\end{equation}

The signature is then $(R,S$). Bob sends $M$, $R$, $S$ and $pub$ to Alice. Alice then computes:

\begin{equation}
k=H(R \: || \: pub \: || \: M) \pmod l\\
P_1=S \cdot B\\
P_2=R + k \cdot pub
\end{equation}

and if $P_1$ is equal to $P_2$, the signature verifies. This works because:

$P_1=S \cdot B = (r + h \cdot s \pmod l) \cdot B = r \cdot B + h \cdot s \cdot B = R + h \cdot pub = P_2$
Note that $l$ is the order of the curve ($l= 2^{252} + 27742317777372353535851937790883648493$).
The great advantage of using Ed25519 over ECDSA is that we can aggregate signatures and public keys.


The following is an outline of the code:
\begin{lstlisting}[language=golang]
package main

import (
	"crypto/ed25519"

	"encoding/base64"
	"fmt"
	"os"
)

func Base64Encode(message []byte) []byte {
	b := make([]byte, base64.StdEncoding.EncodedLen(len(message)))
	base64.StdEncoding.Encode(b, message)
	return b
}

func main() {

	msg := "Hello 123"

	argCount := len(os.Args[1:])
	if argCount > 0 {
		msg = os.Args[1]
	}

	publ, priv, _ := ed25519.GenerateKey((nil))

	m := []byte(msg)

	sig := ed25519.Sign(priv, m)

	fmt.Printf("=== Message ===\n")
	fmt.Printf("Msg: %s\nHash: %x\n", msg, m)
	fmt.Printf("\n=== Public key ===\n")
	fmt.Printf("Public key: %x\n", publ)
	fmt.Printf("   Public key (Base64): %s\n", Base64Encode(publ))
	fmt.Printf("\n=== Private key ===\n")
	fmt.Printf("Private key: %x\n", priv[0:32])
	fmt.Printf("   Private key (Base64): %s\n", Base64Encode(priv[0:32]))
	fmt.Printf("   Private key (Base64) Full key: %s\n", Base64Encode(priv))
	fmt.Printf("   Private key (Full key): %x\n", priv)
	fmt.Printf("\n=== Signature (R,s) ===\n")
	fmt.Printf("Signature: R=%x s=%x\n", sig[0:32], sig[32:64])
	fmt.Printf("   Signature (Base64)=%s\n\n", Base64Encode(sig))

	rtn := ed25519.Verify(publ, m, sig)

	if rtn {
		fmt.Printf("Signature verifies")
	} else {
		fmt.Printf("Signature does not verify")
	}
}

\end{lstlisting}

A sample run with the message of "Hello" is:

\begin{lstlisting}
=== Message ===
Msg: Hello
Hash: 48656c6c6f

=== Public key ===
Public key: c3903a26c73a433554325859c963056acd2d503fc36313ae21647f911e723fab
   Public key (Base64): w5A6Jsc6QzVUMlhZyWMFas0tUD/DYxOuIWR/kR5yP6s=

=== Private key ===
Private key: fc225cb6dd8969541e57754b4120b51e6a92673107c7c8e1dc25a7a3e6b1066b
   Private key (Base64): /CJctt2JaVQeV3VLQSC1HmqSZzEHx8jh3CWno+axBms=
   Private key (Base64) Full key: /CJctt2JaVQeV3VLQSC1HmqSZzEHx8jh3CWno+axBmvDkDomxzpDNVQyWFnJYwVqzS1QP8NjE64hZH+RHnI/qw==
   Private key (Full key): fc225cb6dd8969541e57754b4120b51e6a92673107c7c8e1dc25a7a3e6b1066bc3903a26c73a433554325859c963056acd2d503fc36313ae21647f911e723fab

=== Signature (R,s) ===
Signature: R=fbee75ddd533296a9ebacbe653a3335d1b9a99d6e6c7941d4651e04a6268ad2e s=086b3da235c4f4e426d1a2e76a731c0a81844d98fe59f412abd869fb3008d00d

   Signature (Base64)=++513dUzKWqeusvmU6MzXRuamdbmx5QdRlHgSmJorS4Iaz2iNcT05CbRoudqcxwKgYRNmP5Z9BKr2Gn7MAjQDQ==

Signature verifies
\end{lstlisting}

The signature is 64 bytes long, made up of 32 bytes for the $R$ value, and 32 bytes for the $s$ value. The public key is also 32 bytes long, and the private key as 32 bytes. Overall Ed25519 produces one of the smallest signature sizes, and has a small size of the public and private key.

\subsection{Threshold ECDSA}
With threshold ECDSA we can split the shares over a number of parties and then get each of these parties to sign a part of the signature, and then rebuild these.

\subsubsection{DKLS}
The DKLS [Doerner, Kondi, Lee, and Shelat) method \cite{doerner2019threshold} implements an ECDSA signing algorithm using threshold protocols. In this case, Bob and Alice will communicate using a DKG method, and then Bob will be able to create a valid signature. We can use the Kryptology library developed by Coinbase to implement 2-of-2 threshold ECDSA signing algorithm of the DKLS method. Once Bob and Alice have communicated, Bob will hold a signature for the message. We will then check this signature for its validity. 

 We can use the Kryptology library developed by Coinbase to implement 2-of-2 threshold ECDSA signing algorithm of the DKLS method. Once Bob and Alice have communicated, Bob will hold a signature for the message. We will then check this signature for its validity.

\begin{lstlisting}[language=golang]
package main

import (
	"crypto/ecdsa"
	"crypto/sha256"
	"fmt"
	"os"

	"github.com/btcsuite/btcd/btcec"
	"github.com/coinbase/kryptology/pkg/core/curves"
	"github.com/dustinxie/ecc"

	"github.com/coinbase/kryptology/pkg/tecdsa/dkls"
)

func main() {

	msg := "Hello 123"

	argCount := len(os.Args[1:])

	if argCount > 0 {
		msg = os.Args[1]
	}

	params, _ := dkls.NewParams(btcec.S256(), curves.NewK256Scalar())

	alice := dkls.NewAlice(params)
	bob := dkls.NewBob(params)

	m := []byte(msg)
	digest := sha256.Sum256(m)

	alicePipe, bobPipe := dkls.NewPipeWrappers()
	errors := make(chan error, 2)
	go func() {
		errors <- alice.DKG(alicePipe)
                }()
                go func() {
                errors <- bob.DKG(bobPipe)
	}()
	for i := 0; i < 2; i++ {
		if err := <-errors; err != nil {
			fmt.Printf("Here")
		}
	}

	fmt.Printf("Message to sign: %s\n", msg)
	fmt.Printf("\nAlice Secret Key: %x\n", alice.SkA.Bytes())
	fmt.Printf("Alice Public Key: %x\n", alice.Pk.Bytes())

	fmt.Printf("\nBob Secret Key: %x\n", bob.SkB.Bytes())
	fmt.Printf("Bob Public Key: %x\n", bob.Pk.Bytes())

	errors = make(chan error, 2)
	go func() {
		errors <- alice.Sign(digest[:], alicePipe)
	}()
	go func() {
		errors <- bob.Sign(digest[:], bobPipe)
	}()

	for i := 0; i < 2; i++ {
		if err := <-errors; err != nil {
			fmt.Printf("Signing failed!!!")
		}
	}

	fmt.Printf("Bob Signature: R:%x S:%x\n", bob.Sig.R, bob.Sig.S)

	fmt.Printf("\n=== Now checking with Bob's public key ===\n")
	publicKey := ecdsa.PublicKey{
		Curve: ecc.P256k1(), //secp256k1
		X:     bob.Pk.X,
		Y:     bob.Pk.Y,
	}

	rtn := ecdsa.Verify(&publicKey, digest[:], bob.Sig.R, bob.Sig.S)

	if rtn {
		fmt.Printf("Signature works. Yipee!")
	} else {
		fmt.Printf("Signature does not check out!!!")
	}

}
\end{lstlisting}

The running code is \href{https://asecuritysite.com/kryptology/tecdsa}{here}.

Initially, we split the secret key into two shares and distribute these to Bob and Alice., and which are stored as bob.SkA and alice.SkB. These will be used to generate a public key that Bob and Alice can use (bob.Pk and alice.Pk). This public key can be used to verify the generated digital signature. The following displays the secret shares and the public key:

\begin{lstlisting}[language=golang]
fmt.Printf("Message to sign: %s\n", msg)
fmt.Printf("\nAlice Secret Key: %x\n", alice.SkA.Bytes())
fmt.Printf("Alice Public Key: %x\n", alice.Pk.Bytes())
fmt.Printf("\nBob Secret Key: %x\n", bob.SkB.Bytes())
fmt.Printf("Bob Public Key: %x\n", bob.Pk.Bytes())
\end{lstlisting}

Bob generates a signature by communicating with Alice through DKG, and where the generated signature has two values: R and S. This is displayed as:

\begin{lstlisting}[language=golang]
fmt.Printf("Bob Signature: R:%x S:%x\n", bob.Sig.R, bob.Sig.S)
\end{lstlisting}

We can then take Bob's public key (bob.Pk.X and bob.Pk.Y), and then check that this signature is the valid against the public key:

\begin{lstlisting}
fmt.Printf("\n=== Now checking with Bob's public key ===\n")
	publicKey := ecdsa.PublicKey{
		Curve: ecc.P256k1(), //secp256k1
		X:     bob.Pk.X,
		Y:     bob.Pk.Y,
	}

	rtn := ecdsa.Verify(&publicKey, digest[:], bob.Sig.R, bob.Sig.S)

	if rtn {
		fmt.Printf("Signature works. Yipee!")
	} else {
		fmt.Printf("Signature does not check out!!!")
	}
\end{lstlisting}

A sample run:

\begin{lstlisting}
Message to sign: hello 123

Alice Secret Key: 4d8774e7588a7af7886f1d97216bd7cf97bcce0f3ed4b0cc1308eba19d7068ce
Alice Public Key: 8383eb0260d211043e190b4b8a79db1a95ac0f9b6b5e37946e4bf76f4ad733535ccf8a8e48632107b58f8311f1df1580cbfdd80db01ae952435b4897ecf586ef

Bob Secret Key: d099fd0419dc6afb58229ceece9308a89f35d574e6077ccdf41c50b0ce48c0d0
Bob Public Key: 8383eb0260d211043e190b4b8a79db1a95ac0f9b6b5e37946e4bf76f4ad733535ccf8a8e48632107b58f8311f1df1580cbfdd80db01ae952435b4897ecf586ef
Bob Signature: R:bb4c4b4fbba9da07687320e0c2bf95e5eef5471db1b819fd0188b14f4a60362c S:1efc7288269e613e05faaa29370f86b46cf57cb107e41ef3030a4d345dd0a911

=== Now checking with Bob's public key ===
Signature works. Yipee!
\end{lstlisting}

\subsubsection{GG20}
The GG20 (Gennaro, R., and Goldfeder, S. (2020) \cite{gennaro2020one}) method implements an ECDSA signing algorithm using threshold protocols. In this case, Bob and Alice will communicate using a DKG method, and then Bob will be able to create a valid signature. We can use the Kryptology library developed by Coinbase to implement 2-of-2 threshold ECDSA signing algorithm of the GG20 method. Once Bob and Alice have communicated, Bob will hold a signature for the message. We will then check this signature for its validity. We will thus split a private key up into two secret shares and then will be able to sign with the shares of the key. 

The focus of the paper [1] is to create an ECDSA signature using secret shares of a private key. In this way we can create an ECDSA signature using multiple Shamir shares, and where the private is never actually revealed, but split over two or more parties.

So, let's use the Coinbase Kryptology library to implement a 2-from-2 theshold ECDSA scheme using GG20 (Gennaro and Goldfeder, 2020). Initially we will use the secp256k1 curve and then generate a new private key (ikm):

\begin{lstlisting}[language=golang]
k256 := btcec.S256()ikm, _ := dealer.NewSecret(k256)
\end{lstlisting}

This private key will not be stored on the parties which receive the shares, and can be deleted afer the shares have been distributed. We can then generate the associated public key (pk) and split the key into a number of shares (sharesMap):

\begin{lstlisting}[language=golang]
pk, sharesMap, _ := dealer.NewDealerShares(k256, tshare, nshare, ikm)fmt.Printf("Message: %s\n", msg)fmt.Printf("Sharing scheme: Any %d from %d\n", tshare, nshare)fmt.Printf("Random secret: (%x)\n\n", ikm)fmt.Printf("Public key: (%s %s)\n\n", pk.X, pk.Y)
\end{lstlisting}

This public key will be used to check that the signature that the parties create. We also create public shares which can be used to verify the shares created:

\begin{lstlisting}[language=golang]
pubSharesMap, _ := dealer.PreparePublicShares(sharesMap)
\end{lstlisting}

We then create Paillier keys which will be used to distribute the key signing:

\begin{lstlisting}[language=golang]
keyPrimesArray := genPrimesArray(2)
paillier1, _ := paillier.NewSecretKey(keyPrimesArray[0].p, keyPrimesArray[0].q)

paillier2, _ := paillier.NewSecretKey(keyPrimesArray[1].p, keyPrimesArray[1].q)

	dealerSetup := &signingSetup{
		curve:        k256,
		pk:           pk,
		sharesMap:    sharesMap,
		pubSharesMap: pubSharesMap,
		pubkeys: map[uint32]*paillier.PublicKey{
			1: &paillier1.PublicKey,
			2: &paillier2.PublicKey,
		},
		privkeys: map[uint32]*paillier.SecretKey{
			1: paillier1,
			2: paillier2,
		},
		proofParams: &dealer.TrustedDealerKeyGenType{
			ProofParams: dealerParams,
		},
	}
\end{lstlisting}

The dealer of the shares is now setup. What we need now is two parties to receive the shares, and for them to sign for a message (msg). We can create a hash of the message with:

\begin{lstlisting}[language=golang]
m := []byte(msg)msgHash := sha256.Sum256(m)
\end{lstlisting}

Next we will create two participants (p1 and p2), and where p1 gets the first set of shares (sharesMap1), and the ID for these, and p2 gets the second set of shares (sharesMap2), and the required ID for these:

\begin{lstlisting}[language=golang]
p1 := Participant{*setup.sharesMap[1], setup.privkeys[1]}
p2 := Participant{*setup.sharesMap[2], setup.privkeys[2]}
\end{lstlisting}

And then set them up for split the share. These will be run of either of the parties:

\begin{lstlisting}[language=golang]
s1, _ := p1.PrepareToSign(setup.pk,k256Verifier,setup.curve,setup.proofParams,setup.pubSharesMap,setup.pubkeys)

s2, _ := p2.PrepareToSign(setup.pk,k256Verifier,setup.curve,setup.proofParams,setup.pubSharesMap,
setup.pubkeys)
\end{lstlisting}

We then go into a number of rounds, and where s1 is run on one party, and s2 on another party:

\begin{lstlisting}[language=golang]
r1_s1_bcast, r1_s1_p2p, _ := s1.SignRound1()

r1_s2_bcast, r1_s2_p2p, _ := s2.SignRound1()

r2_s1_p2p, _ := s1.SignRound2(map[uint32]*Round1Bcast{2: r1_s2_bcast},map[uint32]*Round1P2PSend{2: r1_s2_p2p[1]},)

r2_s2_p2p, _ := s2.SignRound2(map[uint32]*Round1Bcast{1: r1_s1_bcast},map[uint32]*Round1P2PSend{1: r1_s1_p2p[2]},)


r3_s1_bcast, _ := s1.SignRound3(map[uint32]*P2PSend{2: r2_s2_p2p[1]},)

r3_s2_bcast, _ := s2.SignRound3(map[uint32]*P2PSend{1: r2_s1_p2p[2]},)

r4_s1_bcast, _ := s1.SignRound4(map[uint32]*Round3Bcast{2: r3_s2_bcast})

r4_s2_bcast, _ := s2.SignRound4(map[uint32]*Round3Bcast{1: r3_s1_bcast})

r5_s1_bcast, r5_s1_p2p, _ := s1.SignRound5(map[uint32]*Round4Bcast{2: r4_s2_bcast},)r5_s2_bcast, r5_s2_p2p, _ := s2.SignRound5(map[uint32]*Round4Bcast{1: r4_s1_bcast},)

r6_s1_bcast, _ := s1.SignRound6Full(msgHash, map[uint32]*Round5Bcast{2: r5_s2_bcast},map[uint32]*Round5P2PSend{2: r5_s2_p2p[1]},)r6_s2_bcast, _ := s2.SignRound6Full(msgHash, map[uint32]*Round5Bcast{1: r5_s1_bcast}, map[uint32]*Round5P2PSend{1: r5_s1_p2p[2]},)
\end{lstlisting}

Now each party can generate the shared signature:

\begin{lstlisting}[language=golang]
s1_sig, _ := s1.SignOutput(
		map[uint32]*Round6FullBcast{2: r6_s2_bcast},
	)

s2_sig, _ := s2.SignOutput(
		map[uint32]*Round6FullBcast{1: r6_s1_bcast},
	)
\end{lstlisting}

We can then check the signature that has been generated against the public key:

\begin{lstlisting}[language=golang]
publicKey := ecdsa.PublicKey{
		Curve: ecc.P256k1(), //secp256k1
		X:     setup.pk.X,
		Y:     setup.pk.Y,
	}

fmt.Printf("Message: %s\n", msg)
fmt.Printf("Node 1 signature: (%d %d)\n", s1_sig.R, s1_sig.S)

fmt.Printf("Node 2 signature: (%d %d)\n", s2_sig.R, s2_sig.S)

rtn := ecdsa.Verify(&publicKey, msgHash, s1_sig.R, s1_sig.S)fmt.Printf("\nSignature Verified: %v", rtn)
\end{lstlisting}[language=golang]

A sample run is:

\begin{lstlisting}
Message: hello
Sharing scheme: Any 2 from 2
Random secret: (4ba8a796f32ec45a1197de6089fa236e50801928ad24fecac8c1ab09e531a166)Public key: (26312696491752052329024843181188922148239837748725137580407874797348180244367 15363854046934109047334192976294337901992160667810868208924200646181218876027)Node 1 signature: (58831626654799325138549587498198878137267315963404497589755928522155537172377 52424895795438944536339814184633346175739904425137488476336337801850504274550)
Node 2 signature: (58831626654799325138549587498198878137267315963404497589755928522155537172377 52424895795438944536339814184633346175739904425137488476336337801850504274550)Signature Verified: true
\end{lstlisting}

A 2-from-2 share is \href{https://asecuritysite.com/kryptology/sss_gg02}{here} and an any t-from-n share is \href{https://asecuritysite.com/kryptology/sss_gg03}{here}.

\subsection{Threshold Ed25519}
To be completed

A demo is \href{https://asecuritysite.com/signatures/ed25519}{here}.


\section{Verifiable Encryption}
\subsection{Camenisch-Shoup}
To be completed

A demo is \href{https://asecuritysite.com/kryptology/camshoup}{here}.

\subsection{ElGamal}
To be completed

A demo is \href{https://asecuritysite.com/kryptology/elgamal_ver}{here}.

















==> sections/blockchain.tex <==
\chapter{DKG on a Blockchain}
\section{Introduction}
\section{Share creation}
For node $P_i$ we create random polynomial values:
\begin{align}
c_{ij} = random(q)$ for $j = 1 ... n\\
c_{i0} = s_i\\
f_i(x)= c_{i0} + c_{i1} x + c_{i2} x^2 ... \pmod q
\end{align}


and where $x$ is the index value of the polynomial. We then generate $f(0), f(1) ... f(n-1)$Next we compute the commitments as:

$C_{ij}=G_1 \times c_{ij}$ for $j = 1 ... n$

and where $C_{ij}$ is the commitment of coefficient $j$ for  $P_i$.

We end up with commitments[] ($C_{i0} ... C_{it}$), shares[] ($c_{i0} ... c_{it}$), and where $c_0$ is the secret share.

![Screenshot 2022-08-04 at 10.44.13.png](https://s3-us-west-2.amazonaws.com/secure.notion-static.com/40c024c5-3435-4248-a3f5-793dfc00b83a/Screenshot_2022-08-04_at_10.44.13.png)

## Share distribution

The share sent from Node $i$  to Node $j$  is encrypted with a key of:

$k_{ij}=sk_i \times pk_j = sk_i \times sk_j \times G$

his is passed through Diffie Hellman key exchange. Each node then sends and encrypted version of $s_{i \rightarrow j}$ from $P_i$ to $P_j$:

$\overline{s_{i \rightarrow j}} =  Enc_{k_{ij}}( s_{i \rightarrow j})$

We thus encrypt share ($s_{ij}$) using the shared key $k_{ij}$. This is performed using and X-OR and Hash method. 

$h=Hash(k_{ij} || j)$

$\overline{s_{i \rightarrow j}} =   s_{i \rightarrow j} \oplus h$

and where Hash() is a Keccak256 hash.

The hash method will just be Keccak-256. In our smart contract, when 
we want to generate the decryption key (decryption_key); we can generate
 with:

```solidity
uint256 decryption_key = uint256(keccak256(abi.encodePacked(sij, j)));
```

and then decrypt with:

```solidity
sij ^= decryption_key;
```

Note that the “^” operation is XOR in Solidity. The Python code to implement these methods is [here](https://asecuritysite.com/ethereum/sym_key). The decryption key is used in the **dispute phase**.

![Screenshot 2022-08-04 at 10.41.02.png](https://s3-us-west-2.amazonaws.com/secure.notion-static.com/c2bb43cb-48f6-404d-88e5-354664749fb0/Screenshot_2022-08-04_at_10.41.02.png)

## Share verification

$C = G_1 \times s_{i \rightarrow j}$

$F_i(j) = \sum_k (c_{ik} \times j^{i+1})$ 

Check $C == F_i(j)$

## DLEQ

Proof ($c,r$) is generated from:

$c,r = DLEQ(G,pk_i,pk_j,k_{ij},sk_i)$ 

and where we create a proof based on $sk_i.G=pk_i$  and $k_{ij} = sk_i.pk_i$. The following is the code in Python [[here](https://asecuritysite.com/zero/dleq4)]:

```python
# Code extracted from https://github.com/PhilippSchindler/ethdkg
import web3
from typing import Tuple
import secrets

from py_ecc.optimized_bn128 import G1, G2
from py_ecc.optimized_bn128 import add, multiply, neg, normalize, pairing, is_on_curve
from py_ecc.optimized_bn128 import curve_order as CURVE_ORDER
from py_ecc.optimized_bn128 import field_modulus as FIELD_MODULUS

# from py_ecc.typing import Optimized_Point3D, Optimized_FQ, Optimized_FQ2
from py_ecc.typing import Optimized_Point3D
from py_ecc.fields import optimized_bn128_FQ, optimized_bn128_FQ2

keccak_256 = web3.Web3.solidityKeccak

PointG1 = Optimized_Point3D[optimized_bn128_FQ]
PointG2 = Optimized_Point3D[optimized_bn128_FQ2]

FQ = optimized_bn128_FQ
FQ2 = optimized_bn128_FQ2

H1 = (
    FQ(9727523064272218541460723335320998459488975639302513747055235660443850046724),
    FQ(5031696974169251245229961296941447383441169981934237515842977230762345915487),
    FQ(1),
)
H2 = (
    FQ2((9110522554455888802745409460679507850660709404525090688071718755658817738702, 14120302265976430476300156362541817133873389322564306174224598966336605751189)),
    FQ2((8015061597608194114184122605728732604411275728909990814600934336120589400179, 21550838471174089343030649382112381550278244756451022825185015902639198926789)),
    FQ2((1, 0))
)

def random_scalar() -> int:
    """ Returns a random exponent for the BN128 curve, i.e. a random element from Zq.
    """
    return secrets.randbelow(CURVE_ORDER)

def dleq(x1: PointG1, y1: PointG1, x2: PointG1, y2: PointG1, alpha: int) -> Tuple[int, int]:
    """ DLEQ... discrete logarithm equality
        Proofs that the caller knows alpha such that y1 = x1**alpha and y2 = x2**alpha
        without revealing alpha.
    """
    w = random_scalar()
    a1 = multiply(x1, w)
    a2 = multiply(x2, w)
    c = keccak_256(
        abi_types=["uint256"] * 12,
        values=[
            int(v)
            for v in normalize(a1)
            + normalize(a2)
            + normalize(x1)
            + normalize(y1)
            + normalize(x2)
            + normalize(y2)
        ],
    )
    c = int.from_bytes(c, "big")
    **r = (w - alpha * c) % CURVE_ORDER**
    return c, r

def dleq_verify(
    x1: PointG1, y1: PointG1, x2: PointG1, y2: PointG1, challenge: int, response: int) -> bool:
    a1 = add(multiply(x1, response), multiply(y1, challenge))
    a2 = add(multiply(x2, response), multiply(y2, challenge))
    c = keccak_256(  # pylint: disable=E1120
        abi_types=["uint256"] * 12,  # 12,
        values=[
            int(v)
            for v in normalize(a1)
            + normalize(a2)
            + normalize(x1)
            + normalize(y1)
            + normalize(x2)
            + normalize(y2)
        ],
    )
    c = int.from_bytes(c, "big")
    return c == challenge

x=random_scalar()

pub1=multiply(G1, x)
pub2=multiply(H1, x)

c,r = dleq(G1, pub1, H1, pub2,x)

rtn=dleq_verify(G1, pub1, H1,pub2, c, r)

print(f"Secret: {x}")
print(f"x.G: {pub1}")
print(f"x.H: {pub2}")
print (f"\nc={c}, r={r}")

print(f"Proven: {rtn}")
```

A sample run gives:

```
x: 10366729598460110564106835528331459549420144661779728900553421386151727683717

x.G: (19264659997498337231621849020324059839727633018344333818406571209706203133187, 12311200540645983074100160614979827101793507198593933504549623882564840726866, 20670726114001654463056991634829687089002941232072263069935333565317103573495)
x.H: (14945644336923121346342859944168545416458423597018613969345084948695366548579, 6287194924561282354354695364050405821231283221714798271249840862954991383974, 9769023299891292075968207384775446300063615377412681646013428758993263180405)

c=51608323136266335612692795096660702882832975771701719531287921368851758992301, 
r=5697936578451188395987467431508950282667773400761457095498679147707605201421
Proven: True
```

Overall the smart contract operates in the same way and uses the bn256Add() and bn256ScalarMul() to implement the add and scalar multiply functions. These are precompile contract functions at 0x06 and 0x07:

```solidity
/**
 *Submitted for verification at Etherscan.io on 2022-08-01
*/

pragma solidity ^0.8.0;

contract dleq {
    function dleq_verify(
        uint256[2] memory x1, uint256[2] memory y1,
        uint256[2] memory x2, uint256[2] memory y2,
        uint256[2] memory proof
    )
    public returns (bool proof_is_valid)
    {
        uint256[2] memory tmp1;
        uint256[2] memory tmp2;

        tmp1 = bn128_multiply([x1[0], x1[1], proof[1]]);
        tmp2 = bn128_multiply([y1[0], y1[1], proof[0]]);
        uint256[2] memory a1 = bn128_add([tmp1[0], tmp1[1], tmp2[0], tmp2[1]]);

        tmp1 = bn128_multiply([x2[0], x2[1], proof[1]]);
        tmp2 = bn128_multiply([y2[0], y2[1], proof[0]]);
        uint256[2] memory a2 = bn128_add([tmp1[0], tmp1[1], tmp2[0], tmp2[1]]);

        uint256 challenge = uint256(keccak256(abi.encodePacked(a1, a2, x1, y1, x2, y2)));
        proof_is_valid = challenge == proof[0];
  

    }
    function bn128_multiply(uint256[3] memory input)
    public returns (uint256[2] memory result) {
        // computes P*x
        // input: 3 values of 256 bit each
        //  *) x-coordinate of point P
        //  *) y-coordinate of point P
        //  *) scalar x

        bool success;
        assembly {
            // 0x07     id of precompiled bn256ScalarMul contract
            // 0        number of ether to transfer
            // 96       size of call parameters, i.e. 96 bytes total (256 bit for x, 256 bit for y, 256 bit for scalar)
            // 64       size of call return value, i.e. 64 bytes / 512 bit for a BN256 curve point
            success := call(not(0), 0x07, 0, input, 96, result, 64)
        }
        require(success, "elliptic curve multiplication failed");
    }
    function bn128_add(uint256[4] memory input)
    public returns (uint256[2] memory result) {
        // computes P + Q
        // input: 4 values of 256 bit each
        //  *) x-coordinate of point P
        //  *) y-coordinate of point P
        //  *) x-coordinate of point Q
        //  *) y-coordinate of point Q

        bool success;
        assembly {
            // 0x06     id of precompiled bn256Add contract
            // 0        number of ether to transfer
            // 128      size of call parameters, i.e. 128 bytes total
            // 64       size of call return value, i.e. 64 bytes / 512 bit for a BN256 curve point
            success := call(not(0), 0x06, 0, input, 128, result, 64)
        }
        require(success, "elliptic curve addition failed");
    }
}
```

## Load shares

We load the encrypted shares and decrypt them. We are then able to verify each share.  Shares which fail will be marked as INVALID within node.decryted[issuer]:

![Screenshot 2022-08-04 at 10.16.31.png](https://s3-us-west-2.amazonaws.com/secure.notion-static.com/719f1520-0c04-44d9-87b6-b26d79c4ac82/Screenshot_2022-08-04_at_10.16.31.png)

## Submit disputes

Each node will check if the nodes have provided invalid shares. For disputed shares, a node will use dleq() to create a shared_key_correctness_proof (c,r). This and the shared_key is passed to the mark contract. The smart contract uses dleq_verify() to verify, and if it shows that the share is incorrect the disrupter is marked as having invalid shares, with setting share_distribution_hashes[issuer] with a zero value.

![Screenshot 2022-08-04 at 10.34.14.png](https://s3-us-west-2.amazonaws.com/secure.notion-static.com/4ac3f302-dc59-4c36-b4b0-2224d419ca4c/Screenshot_2022-08-04_at_10.34.14.png)

## Load disputes

With this, a node loads the disputes and verifies them. It does this by reading the dispute event log from the smart contract. The node then verifies the dispute, and updates node.disputed_nodes[].

![Screenshot 2022-08-04 at 11.53.15.png](https://s3-us-west-2.amazonaws.com/secure.notion-static.com/bcdea977-bc1d-437f-8d30-e5eca42c52a8/Screenshot_2022-08-04_at_11.53.15.png)

